CS Educator challenges and their solutions : A systematic mapping study

Computer Science (CS) education is expanding rapidly, but educators continue to face persistent challenges in teaching and learning environments.Despite growing interest, limited systematic work exists to categorize and synthesize the specific challenges faced by CS educators and the remedies adopted in response.This is problematic because it remains unclear which areas have been thoroughly addressed and which still lack sufficient scholarly attention. In this study, we conducted a structured literature review of peer-reviewed research papers published over the last five years, focusing on challenges and remedies across ten categorized themes, including pedagogical, emotional, technological, and institutional dimensions.Our analysis revealed recurring issues in areas such as assessment practices, teacher training, classroom management, and emotional well-being, along with various strategies such as professional development programs and policy interventions adopted to mitigate them while also revealing several areas that have received insufficient attention.This review offers a consolidated understanding of the CS education landscape, providing valuable insights for researchers, curriculum designers, and policymakers aiming to improve teaching effectiveness and educator support.

==> ExtraContentToRefer.tex <==
pedagogical pointwise:

Pedagogical challenges faced by Computer Science (CS) teachers and educators refer to the multifaceted difficulties and obstacles that educators encounter in effectively designing, delivering, and adapting computer science instruction. These challenges stem from the inherent nature of computer science as a discipline, the rapid evolution of technology, the societal implications of computing, and the institutional contexts in which teaching occurs.



\subsubsection{Lack of Pedagogical Content Knowledge and Adaptability}
Educators frequently lack the pedagogical content knowledge required for effective CS instruction, needing to adapt continuously to diverse student needs and contexts \cite{Thigpen2024}. As a result, students often struggle to transfer knowledge between sessions and peers, which complicates collaborative learning \cite{Musaeus2024}.

\subsubsection{Preparation Gaps and Communication Barriers}
Preparation gaps among instructors and TAs hinder student motivation, often due to poor communication, unclear objectives, and social anxiety \cite{Farghally2024}. Instructors also face conflicting guidance on teaching style, especially with language-specific conventions \cite{Kirk2024}.

\subsubsection{Insufficient Industry Alignment and Teacher Shortage}
Integrating industry practices remains uneven, especially in theory-heavy courses like algorithms \cite{Valstar2020}. A shortage of qualified CS teachers continues, and pedagogical training is often inadequate \cite{Williams2020,Pieper2020}.

\subsubsection{Instructional Ineffectiveness and Lack of Training}
Student enthusiasm tends to drop when instructional methods or infrastructure are ineffective, and students often lack resilience \cite{Venn-Wycherley2020}. Many instructors lack formal training and are unfamiliar with evidence-based strategies \cite{Goncharow2021}, resulting in students struggling to transfer skills between programming languages \cite{Tshukudu2021}.

\subsubsection{Curricular Misalignment and Evolving Standards}
Defining the academic core of CS and aligning it with pedagogical practice is difficult as educational standards evolve \cite{Ni2021}. Technical content frequently overshadows pedagogical focus \cite{Vahid2024}, and teacher qualifications and professional development remain ongoing concerns \cite{Denny2024}.

\subsubsection{Standards-Based and Culturally Responsive Pedagogy}
Aligning lessons with standards such as the (Computer Science Teachers Association) CSTA remains challenging, particularly for novice teachers \cite{McGill2023}. Translating culturally responsive pedagogy into actionable practice, embedding cultural content, and supporting student-led learning are further complicated by rigid curriculum constraints \cite{Hwang2023}. Integrating social justice topics adds additional complexity \cite{Hwang2023}.

\subsubsection{Challenges of OER and AI Integration}
Open Educational Resource (OER) use presents issues related to coverage, quality, customization, and keeping content current in a rapidly evolving discipline \cite{Fowler2023}. Growing reliance on AI can impede foundational learning and demands new competencies in prompt engineering \cite{Lau2023}. CS1 and CS2 courses still emphasize syntax over conceptual understanding \cite{Lau2023}.

\subsubsection{Project-Based Learning and Resistance to Innovation}
Project-based learning in CS is hindered by the complexity of topics \cite{Samarasekara2023}. There is also resistance to centralized textbooks and digital technology integration \cite{Samarasekara2023}. Furthermore, incorporating abolitionist or justice-oriented content faces skepticism, contributing to techno-nihilism and a diminished sense of pedagogical imagination \cite{Rosenbloom2023}.

\subsubsection{Assessment Tools, Feedback, and TA Limitations}
Feedback systems can often confuse students, especially when relying on outdated or legacy platforms \cite{Forden2023}. The effectiveness of gamification tools in introductory courses like CS1 remains contested \cite{Forden2023}. Teaching assistants frequently lack deep content knowledge, which limits the quality of grading and instructional support \cite{Zaman2023}.

\subsubsection{Student Diversity, Debugging, and Learning Support}
Diverse levels of prerequisite knowledge among students complicate task selection and goal-setting for educators \cite{Sauerwein2023}. Debugging remains a persistent difficulty for both students and instructors \cite{Macann2023}. Additionally, many educators undervalue the importance of clear learning objectives and struggle to develop high-quality instructional materials. Reliance on log data without translating it into actionable pedagogical feedback, and insufficient support for isolated learners, further exacerbate teaching challenges \cite{Singh2020}.


\subsection{Pedagogical Challenges}
% Common themes of pedagogical challenges reported across various studies include lack of CS-specific teaching knowledge required for effective CS instruction, needing to adapt continuously to diverse student needs and contexts \cite{Thigpen2024}, preparation and knowledge gaps among instructors and TAs \cite{Zaman2023,Sauerwein2023}, conflicting guidance on teaching style, especially with language-specific conventions \cite{Kirk2024}, inadequacy of Open Educational Resource  (OERs) \cite{Fowler2023}, challenges of project-based learning \cite{Samarasekara2023} and curriculum gaps especially around cultural integration, ethics, and digital technology integration (DEI) content \cite{Hwang2023,Rosenbloom2023}. Instructors also often fail to craft effective objectives, design interactive material \cite{Singh2020, Kirk2022} or support collaborative learning \cite{Brandes2020}, especially in large classes \cite{Patel2024}. 

% Online learning brings a range of specific challenges ranging from student engagement and participation \cite{Wilde2024,Cook2022,Ju2020}, adapting existing material to online contexts keeping in mind diverse learning styles or equitable access \cite{Marshall2020,Hamouda2025,Izu2025}, offering feedback at scale \cite{Krause-Levy2023} to developing effective curricula blending practical skill development and theoretical knowledge \cite{VanDeGrift2023,Anyango2021} remain ongoing concerns. 

% promote asynchronous participation \cite{}, and scaffold difficult concepts \cite{Upadhyaya2020}. Timely feedback delivery \cite{Kalathas2022}, real-world learning transfer \cite{Nitta2022}, cultural competence \cite{Ishizue2024}, and the bridging of theory and practice \cite{Berry2022} are also emphasized. Furthermore, academic rigor in flexible formats \cite{Shrestha2022}, supporting diverse learner needs \cite{Mason2024}, encouraging self-regulated learning \cite{Luxton-Reilly2023}, blended learning \cite{Lau2022}, and gamification strategies \cite{Tsan2022} are pursued alongside balancing synchronous and asynchronous activities \cite{Su2021}, personalized pathways \cite{Lee2022}, deep learning strategies \cite{Yadav2022}, learning analytics \cite{Tsan2022}, and future-ready learning approaches \cite{Wilde2024}.Recent studies have highlighted core pedagogical difficulties in teaching CS algorithms courses, such as students' insufficient background knowledge, lack of mathematical and proof-writing skills, and lack of programming experience. Educators also face challenges helping students apply algorithm design techniques to novel problems and struggle to illustrate the real-world relevance of abstract concepts \cite{Luu2023,Mahoney2023}.

\subsection{Classroom Management Challenges}

Classroom management in CS education encompasses the effective organization of instruction, scaling of resources, and sustaining student engagement. 

\subsubsection{Instructional Constraints and Equity}
Instructors face ongoing pedagogical and logistical hurdles, such as adapting practices to diverse classroom contexts and ensuring equitable participation \cite{Thigpen2024,Musaeus2024,Farghally2024}. Large class sizes further exacerbate difficulties in maintaining instructional quality and attending to individual student needs \cite{Valstar2020,Goncharow2021,Pieper2020}.

\subsubsection{Student Engagement and Resource Limitations}
Engaging students who lack confidence, motivation, or preparedness remains a persistent classroom management concern \cite{Venn-Wycherley2020}. Instructors also contend with limited lecture time \cite{Vahid2024}, inadequate feedback mechanisms \cite{Wang2021}, and covert use of AI tools in student learning \cite{Lau2023}. Constraints on time and institutional resources hinder the ability to provide individualized support \cite{Samarasekara2023,Forden2023}.

\subsubsection{TA Workload and Psychological Safety}
Teaching Assistants (TAs) are frequently overwhelmed, serving as primary contact points for students while being constrained by class size and time pressures \cite{Zaman2023,Huang2023,Lee2021}. Beyond technical assistance, they are expected to maintain classroom climate and manage group dynamics, including the prevention of harassment and the promotion of psychological safety \cite{Huang2023}.

\subsubsection{Online Learning and Student Conduct}
The shift to online learning brought new management challenges, including navigating platforms such as Zoom \cite{Perlman2021}, guiding students who were unprepared for digital formats \cite{Markel2021}, and mitigating misconduct like unauthorized online assistance \cite{Rusak2021}. In both online and in-person contexts, managing diversity, interpersonal conflict, and fluctuating student motivation remains essential \cite{Riese2021}. Tutors also face difficulties maintaining focus during collaborative exercises and adapting instruction to accommodate various learning styles \cite{Sentance2021,Goletti2021}.

\subsubsection{Capstone Course and Group Dynamics}
Instructors leading capstone or project-based courses encounter challenges scaling collaborative projects, managing unequal group contributions, and navigating varied student interaction preferences \cite{Hooshangi2025}. Resistance to unfamiliar tools perceived as unnecessary and discomfort with assigned group roles further complicate instruction \cite{Patel2024,Jia2022}.

\subsubsection{TA Coordination and Logistical Complexity}
In large instructional teams, effective TA coordination is often hindered by fragmented communication, inconsistent schedules, irregular attendance, and uneven task distribution \cite{Minnes2022,Akhmetov2024}. Additional burdens such as high grading workloads, inefficient time management, and queue management during office hours add to the complexity of classroom operations \cite{Kumar2022,Riese2022,Brunelle2022}.

\subsubsection{Recurring Logistical Issues}
Recurring logistical issues in CS classrooms include the lack of standardization in final project expectations \cite{Kao2020}, the time-intensive nature of in-class activities \cite{Kussmaul2022}, variable pacing across student teams \cite{Kussmaul2022}, and challenges with students who resist help or have inconsistent prior experience with Unix-based systems \cite{Krause-Levy2023}.


Managing large, diverse CS classrooms involves balancing engagement, timely feedback, and individual attention \cite{Thigpen2024,Valstar2020,Goncharow2021}. Challenges include student disinterest, anxiety, and conceptual difficulty \cite{Pieper2020,Venn-Wycherley2020,Vahid2024}. Delayed feedback and AI taboos complicate transparency \cite{Wang2021,Lau2023}. Limited resources and rising enrollments strain support systems \cite{Samarasekara2023,Forden2023}. TAs face behavioral issues, group conflicts, and harassment cases \cite{Zaman2023,Huang2023,Lee2021}. Tutors deal with uneven demand and unpermitted help concerns \cite{Markel2021,Rusak2021}. Differentiated teaching remains challenging due to diverse learning styles and tool familiarity gaps \cite{Goletti2021,Sentance2021,Hooshangi2025}. Coordination failures, high grading loads, and unclear guidance burden TAs \cite{Akhmetov2024,Minnes2022,Kao2020,Kussmaul2022,Kumar2022,Riese2022}.


Managing virtual classrooms presents challenges like controlling disruptive behavior \cite{Krause-Levy2023}, maintaining focus \cite{Anyango2021}, and handling technical issues \cite{Saraiva2021}. Ensuring active participation \cite{Hamouda2025}, dealing with varied learning speeds \cite{Izu2025}, and fostering inclusivity \cite{Patel2024} remain essential. Monitoring student progress \cite{Kirk2022}, setting conduct norms \cite{Brandes2020}, and preventing distractions \cite{Ju2020} are also challenging. Facilitating respectful communication \cite{Upadhyaya2020}, minimizing lost time due to technical problems \cite{Kalathas2022}, and motivating passive learners \cite{Nitta2022} require proactive strategies. Cyberbullying prevention \cite{Ishizue2024}, student well-being monitoring \cite{Berry2022}, and creating social presence \cite{Shrestha2022} are also priorities. Effective use of breakout rooms \cite{Mason2024}, individualized support \cite{Luxton-Reilly2023}, time management \cite{Lau2022}, equitable engagement \cite{Su2021}, conflict resolution \cite{Yadav2022}, virtual space design \cite{Wilde2024}, instructional clarity \cite{Marshall2020}, respect-building \cite{Cook2022}, Learning Management System (LMS) tools \cite{VanDeGrift2023}, and emergency preparedness \cite{Krause-Levy2023} contribute to classroom control \cite{Anyango2021}.Promoting student accountability and responsibility in virtual settings has been emphasized \cite{Tsan2022}, as well as establishing effective conflict resolution strategies for online classroom environments \cite{Tsan2022b}.



%Instructors face ongoing pedagogical and logistical hurdles, such as adapting practices to diverse classroom contexts and ensuring equitable participation \cite{Thigpen2024,Musaeus2024,Farghally2024}. Large class sizes exacerbate difficulties in maintaining instructional quality and responding to student needs \cite{Valstar2020,Goncharow2021,Pieper2020}.

% Engaging students who lack confidence, motivation, or preparedness remains a persistent issue \cite{Venn-Wycherley2020}. Instructors also struggle with limited lecture time \cite{Vahid2024}, inadequate feedback mechanisms \cite{Wang2021}, and the covert use of AI tools in learning \cite{Lau2023}. Constraints on time and resources further complicate efforts to offer individualized support \cite{Samarasekara2023,Forden2023}.

% TAs are often overwhelmed, acting as primary contact points yet constrained by course size and time \cite{Zaman2023,Huang2023,Lee2021}. They must manage not only technical support but also classroom climate and group dynamics, including preventing harassment and fostering psychological safety \cite{Huang2023}.

% The transition to online learning introduced new difficulties in managing platforms like Zoom \cite{Perlman2021}, guiding unprepared students \cite{Markel2021}, and addressing misconduct such as unauthorized online aid \cite{Rusak2021}. Managing student diversity, conflict, and varying motivation levels remains integral to classroom control \cite{Riese2021}. Tutors also face issues with maintaining focus during collaborative tasks and adapting instructions to different learning styles \cite{Sentance2021,Goletti2021}.

% Capstone instructors face challenges in scaling project-based work, managing uneven group contributions, and anticipating different student interaction styles \cite{Hooshangi2025}. Students’ resistance to tools perceived as extra work and discomfort with group roles present additional obstacles \cite{Patel2024,Jia2022}.

% In large teams, TA coordination is hindered by fragmented communication, schedule confusion, inconsistent attendance, and uneven task distribution \cite{Minnes2022,Akhmetov2024}. Grading workload, time management, and queue management during office hours add further pressure \cite{Kumar2022,Riese2022,Brunelle2022}.

% Other recurring issues include lack of standardization in final projects \cite{Kao2020}, time-consuming in-class activities \cite{Kussmaul2022}, varied team pacing \cite{Kussmaul2022}, and managing students who resist help or have inconsistent Unix backgrounds \cite{Krause-Levy2023}.


% Educators frequently lack the pedagogical content knowledge required for effective CS instruction, needing to adapt continuously to diverse student needs and contexts \cite{Thigpen2024} due to which students often struggle to transfer knowledge between sessions and peers, complicating collaborative learning \cite{Musaeus2024}.

% Preparation gaps among instructors and TAs hinder student motivation, often due to poor communication, unclear objectives, and social anxiety \cite{Farghally2024}. Instructors face conflicting guidance on teaching style, particularly with language-specific conventions \cite{Kirk2024}.

% Integrating industry practices remains uneven, especially in theory-heavy courses like algorithms \cite{Valstar2020}. A shortage of qualified CS teachers persists, with pedagogical training often insufficient \cite{Williams2020,Pieper2020}.

% Student enthusiasm drops when instructional methods or infrastructure are ineffective \cite{Venn-Wycherley2020}, and resilience is often lacking \cite{Venn-Wycherley2020}. Many instructors lack formal training and familiarity with evidence-based strategies \cite{Goncharow2021} leading to students struggle to transfer skills between languages \cite{Tshukudu2021}.

% Defining CS’s academic core and aligning it with pedagogy is difficult as standards evolve \cite{Ni2021}, and technical content often overshadows pedagogical focus \cite{Vahid2024}. Teacher qualifications and professional development remain ongoing issues \cite{Denny2024}.

% Lesson alignment with standards like CSTA is challenging, especially for new teachers \cite{McGill2023}. Translating culturally responsive pedagogy into practice, embedding cultural content, and fostering student-led learning remain difficult under curriculum constraints \cite{Hwang2023}. Integrating social justice content adds further complexity \cite{Hwang2023}.

% OER use introduces challenges in coverage, quality, customization, and currency in a rapidly evolving field \cite{Fowler2023}. Increased reliance on AI can hinder foundational learning and requires new prompt-crafting skills \cite{Lau2023}. CS1/CS2 courses still prioritize syntax over conceptual understanding \cite{Lau2023}.

% Project-based learning in CS is difficult due to topic complexity \cite{Samarasekara2023}. Resistance to centralized textbooks and digital tech integration adds friction \cite{Samarasekara2023}. Teachers also face skepticism when incorporating abolitionist or justice-oriented content \cite{Rosenbloom2023}, contributing to techno-nihilism and diminished pedagogical imagination \cite{Rosenbloom2023}.

% Feedback systems often confuse students, especially when relying on legacy platforms \cite{Forden2023}. Gamification tools in CS1 are debated in terms of relevance and complexity \cite{Forden2023}. TAs often lack deep content knowledge, limiting the quality of grading and support \cite{Zaman2023}.

% Varying prerequisite knowledge complicates task selection and goal-setting \cite{Sauerwein2023}. Debugging remains a consistent challenge for students and instructors alike \cite{Macann2023}. Educators frequently undervalue clear learning objectives and struggle with crafting exemplary materials. Many rely on log data without meaningful pedagogical feedback and fail to support isolated learners \cite{Singh2020}.


assestemenmt :
\subsubsection{Scalability and Feedback Mechanisms}
CS educators frequently struggle to design assessments that are scalable, meaningful, and timely. Innovations such as rubrics tailored for code-related support \cite{Esche2024} and structured TA hierarchies \cite{Akhmetov2024} have been used to improve the quality of feedback. Automated programming assessment systems enhance formative feedback processes \cite{Sauerwein2023}, while digital TAs offer personalized guidance—though their effectiveness depends on fostering student autonomy and not just delivering answers \cite{Denny2024}.

\subsubsection{Challenges in Online Assessment Environments}
Assessment in online education introduces unique challenges. These include preventing academic dishonesty \cite{Cook2022}, designing authentic and contextually rich assessments \cite{VanDeGrift2023}, and fairly grading collaborative student work \cite{Krause-Levy2023}. While automated grading \cite{Anyango2021} and digital feedback tools \cite{Saraiva2021} offer efficiencies, they often fall short in evaluating practical skills in remote settings \cite{Hamouda2025}.

\subsubsection{Higher-Order Thinking and Standardization}
Educators face persistent issues in assessing higher-order thinking skills \cite{Izu2025}, standardizing evaluation criteria across diverse contexts \cite{Patel2024}, and ensuring academic integrity in both physical and online settings \cite{Kirk2022}. Tools like online proctoring \cite{Brandes2020}, performance-based assessments \cite{Weintrop2022}, and collaborative project evaluations \cite{Ju2020} complicate implementation.

\subsubsection{Feedback, Workload, and Skill Coverage}
Providing meaningful feedback \cite{Upadhyaya2020}, assessing soft skills \cite{Kalathas2022}, and ensuring robust plagiarism detection \cite{Nitta2022} are critical yet challenging tasks. High grading workloads \cite{Ishizue2024} and the need for culturally responsive assessment tools \cite{Shrestha2022} add further complexity.

\subsubsection{Alignment, Validity, and Accommodations}
Educators often struggle to align assessments with learning outcomes \cite{Mason2024}, maintain validity across formats \cite{Luxton-Reilly2023}, and provide equitable accommodations \cite{Lau2022}. Formative assessments \cite{Tsan2022} and experiential learning evaluations \cite{Su2021} are essential for learner development, yet difficult to implement effectively.

\subsubsection{Peer Review, Adaptivity, and Analytics}
Peer and self-assessment strategies \cite{Lee2022}, adaptive testing methods \cite{Yadav2022}, and transparent grading practices \cite{Tsan2022} are increasingly valued. However, measuring their effectiveness \cite{Wilde2024}, integrating learning analytics \cite{Marshall2020}, and preparing students for high-stakes examinations \cite{Cook2022} remain persistent concerns. Evaluating interdisciplinary skills poses additional challenges \cite{VanDeGrift2023}.

\subsubsection{Inclusive and Adaptive Assessments}
Accommodations for students with disabilities in online assessments are increasingly recognized as vital \cite{Tsan2022}. The development of adaptive assessment strategies that dynamically respond to individual learner performance is an ongoing priority \cite{Tsan2022b}.

\subsubsection{Assessment Design and Conceptual Mastery}
Crafting effective in-class problems and homework questions is another common obstacle. Students’ difficulty in mastering advanced topics such as dynamic programming and NP-completeness further complicates fair and accurate assessment design \cite{Luu2023}.

% \subsection{Assessment Challenges Faced by Educators}




CS educators struggle to design scalable, meaningful, and timely assessments. Rubrics for code-related support \cite{Esche2024} and tiered TA structures \cite{Akhmetov2024} improve feedback. Automated programming systems enhance formative assessment \cite{Sauerwein2023}. Digital TAs offer personalized feedback, but only if they foster learning autonomy \cite{Denny2024}.

Assessment in online education poses challenges related to preventing cheating \cite{Cook2022}, crafting authentic assessments \cite{VanDeGrift2023}, and fairly evaluating group work \cite{Krause-Levy2023}. Automated grading \cite{Anyango2021}, feedback provision \cite{Saraiva2021}, and remote practical skill evaluation \cite{Hamouda2025} are often problematic. Educators face difficulties measuring higher-order thinking \cite{Izu2025}, standardizing assessments \cite{Patel2024}, and preserving academic integrity \cite{Kirk2022}. Online proctoring \cite{Brandes2020}, performance-based assessments \cite{Weintrop2022}, and collaborative project evaluation \cite{Ju2020} further complicate the process. Meaningful feedback \cite{Upadhyaya2020}, soft skill assessment \cite{Kalathas2022}, plagiarism detection \cite{Nitta2022}, grading workloads \cite{Ishizue2024}, and culturally responsive tools \cite{Shrestha2022} are pressing concerns. Aligning assessments with outcomes \cite{Mason2024}, maintaining validity \cite{Luxton-Reilly2023}, ensuring accommodations \cite{Lau2022}, formative assessment \cite{Tsan2022}, and experiential learning evaluation \cite{Su2021} are vital. Peer and self-assessment \cite{Lee2022}, adaptive strategies \cite{Yadav2022}, grading transparency \cite{Tsan2022}, effectiveness measurement \cite{Wilde2024}, use of learning analytics \cite{Marshall2020}, preparation for high-stakes exams \cite{Cook2022}, and interdisciplinary evaluation \cite{VanDeGrift2023} round out the assessment concerns.Accommodations for students with disabilities in online assessments are increasingly recognized as essential \cite{Tsan2022}, along with the need to develop adaptive assessment strategies that respond dynamically to learner performance \cite{Tsan2022b}.Assessment design presents its own set of issues, including crafting effective in-class problems and homework questions. Students’ difficulty in mastering topics like dynamic programming and NP-completeness further complicates evaluation \cite{Luu2023}.


Emotional:

\subsubsection{Burnout, Stress, and Institutional Pressures}
CS educators frequently experience stress, burnout, and low self-esteem due to unclear institutional expectations, overwhelming technological demands, and disengaged students \cite{Thigpen2024,Farghally2024,Venn-Wycherley2020}. Early-career and marginalized educators often feel unsupported in their roles, leading to feelings of isolation and underappreciation \cite{Vivian2020,Goncharow2021,Tshukudu2021,Ni2021}. Additional emotional burdens stem from cognitive overload, misalignment between assessments and instruction, and fatigue from constant feedback cycles \cite{Fowler2023,Forden2023,Lau2023}.

\subsubsection{Challenges for Teaching Assistants and Marginalized Groups}
Teaching Assistants (TAs) are often emotionally unprepared to handle classroom roles, especially when facing harassment or dealing with emotionally charged situations \cite{Huang2023}. Instructors and TAs also face emotional strain when accommodating students with accessibility needs, particularly Blind and Visually Impaired (BVI) learners \cite{Huff2021}. The COVID-19 pandemic exacerbated these stressors, introducing job insecurity, anxiety over digital platforms, and intensified pressure on tutors \cite{Perlman2021,Skuratowicz2021,Markel2021}. Moreover, overconfidence or resistance to training can stunt personal and professional growth \cite{Kumar2021,Munasinghe2021}.

\subsubsection{Emotional Burdens of Online Education}
Online learning environments have magnified emotional and psychological burdens for educators. Isolation, educator burnout, and declining student motivation are common concerns \cite{Saraiva2021,Hamouda2025,Izu2025}. Anxiety related to unfamiliar technologies \cite{Patel2024}, growing mental health challenges \cite{Kirk2022}, and difficulties in building meaningful relationships online \cite{Brandes2020} are frequent issues.

\subsubsection{Student Struggles and Institutional Responses}
Students themselves cope with academic pressure \cite{Weintrop2022}, screen fatigue \cite{Ju2020}, and loneliness \cite{Upadhyaya2020}, creating emotional ripple effects that educators must manage. Institutions are working to support wellness, but educators remain on the front lines of student emotional health \cite{Kalathas2022}. Technostress \cite{Nitta2022}, crisis support during emergencies \cite{Ishizue2024}, and anxiety around assessments \cite{Berry2022} require responsive and empathetic instructional strategies.

\subsubsection{Mental Health, Belonging, and Resilience}
Concerns such as a lack of belonging \cite{Shrestha2022}, difficulties with self-regulation \cite{Mason2024}, household distractions \cite{Luxton-Reilly2023}, and exacerbation of pre-existing mental health conditions \cite{Lau2022} demand active intervention. Educators must address digital addiction \cite{Tsan2022}, privacy concerns in remote counseling \cite{Su2021}, and student resilience \cite{Lee2022}, while also confronting imposter syndrome \cite{Yadav2022,Tsan2022b}.

\subsubsection{Well-Being, Support Systems, and Emotional Environment}
Other notable emotional concerns include peer support challenges \cite{Tsan2022}, screen-intensity fatigue \cite{Wilde2024}, fear of missing out (FOMO) in academic settings \cite{Marshall2020}, and sustaining educator well-being \cite{Cook2022}. Ensuring low-stress learning environments \cite{VanDeGrift2023}, addressing disparities in emotional support \cite{Krause-Levy2023}, and promoting mindfulness through technology \cite{Anyango2021} are essential. Finally, educators must be equipped to provide grief support when needed \cite{Hamouda2025}, ensuring a compassionate and emotionally inclusive learning environment.

%\subsection{Emotional and Psychological Challenges Faced by Educators}



Educators often experience stress, burnout, and low self-esteem due to unclear expectations, tech overload, institutional pressure, and student disengagement \cite{Thigpen2024,Farghally2024,Venn-Wycherley2020}. Early-career and marginalized teachers feel unsupported \cite{Vivian2020,Goncharow2021,Tshukudu2021,Ni2021}. Additional burdens include cognitive overload, misaligned assessments, and feedback fatigue \cite{Fowler2023,Forden2023,Lau2023}. TAs face harassment and lack emotional readiness \cite{Huang2023}, while accessibility challenges for (Blind and Visually Impaired)BVI students add strain \cite{Huff2021}. The pandemic amplified job insecurity, platform anxiety, and tutor stress \cite{Perlman2021,Skuratowicz2021,Markel2021}. Overconfidence or training resistance also limits growth \cite{Kumar2021,Munasinghe2021}.


Online education amplifies emotional and psychological burdens, such as isolation \cite{Saraiva2021}, educator burnout \cite{Hamouda2025}, and waning student motivation \cite{Izu2025}. Anxiety over technology \cite{Patel2024}, mental health concerns \cite{Kirk2022}, and relationship building online \cite{Brandes2020} are frequent challenges. Students cope with academic pressure \cite{Weintrop2022}, screen fatigue \cite{Ju2020}, and loneliness \cite{Upadhyaya2020}, while institutions strive to support wellness \cite{Kalathas2022}. Technostress \cite{Nitta2022}, crisis support \cite{Ishizue2024}, assessment anxiety \cite{Berry2022}, belongingness \cite{Shrestha2022}, self-regulation \cite{Mason2024}, distractions at home \cite{Luxton-Reilly2023}, and pre-existing conditions \cite{Lau2022} need active intervention. Other emotional concerns include digital addiction \cite{Tsan2022}, privacy in counseling \cite{Su2021}, resilience \cite{Lee2022}, imposter syndrome \cite{Yadav2022}, peer support \cite{Tsan2022}, screen-intensity fatigue \cite{Wilde2024}, fear of missing out (FOMO) \cite{Marshall2020}, educator well-being \cite{Cook2022}, low-stress learning environments \cite{VanDeGrift2023}, disparities in emotional support \cite{Krause-Levy2023}, mindfulness through tech \cite{Anyango2021}, and grief support \cite{Hamouda2025}.Educators must also support students with pre-existing mental health conditions that are exacerbated in online contexts \cite{Tsan2022}, and address the challenge of imposter syndrome, which affects learners’ self-perception and academic engagement \cite{Tsan2022b}.


technological:

\subsubsection{Tool Integration and Infrastructure Limitations}
Educators face persistent burdens related to tool integration, inadequate infrastructure, and lack of technical expertise \cite{Thigpen2024,Musaeus2024,Farghally2024}. Faculty often struggle to keep up with rapidly evolving industry demands \cite{Valstar2020}, while retrained teachers encounter difficulties in mastering new content and managing technical errors \cite{Vivian2020,Pieper2020}. Commonly used instructional and assessment tools such as Scratch and Python pose usability and accessibility challenges \cite{Wang2021,Tshukudu2021,McGill2023}.

\subsubsection{Limitations of Educational Tools and Interfaces}
Open Educational Resources (OERs) frequently lack proper Learning Management System (LMS) integration and fail to provide sufficient interactivity \cite{Fowler2023}. AI-based tools, though promising, are often flawed and difficult to adapt to specific classroom needs \cite{Denny2024}. Poorly designed interfaces, inaccessible Integrated Development Environments (IDEs), and persistent debugging challenges further hinder effective teaching and learning \cite{Forden2023,Greifenstein2023,Huff2021,Macann2023}. The rapid pivot to online teaching during the COVID-19 pandemic revealed major readiness gaps in technological preparedness and platform fluency \cite{Perlman2021,Skuratowicz2021,Simmonds2021}.

\subsubsection{Access, Devices, and Compatibility Barriers}
Technological equity remains a major concern. Many students and educators face issues with poor internet connectivity \cite{Izu2025}, lack of adequate devices \cite{Patel2024}, and cross-platform compatibility problems \cite{Kirk2022}. Additional barriers include cybersecurity threats \cite{Brandes2020}, insufficient technical support \cite{Weintrop2022}, and the accelerating pace of technology evolution \cite{Ju2020}. Data privacy \cite{Upadhyaya2020} and the need to ensure accessible tools and equitable internet access \cite{Kalathas2022,Nitta2022} require urgent institutional responses.

\subsubsection{Platform Management and Institutional Responsibilities}
Ensuring stable and well-managed platforms is critical for digital learning environments. Institutions must address student device distribution \cite{Ishizue2024}, platform management \cite{Berry2022}, digital literacy gaps \cite{Shrestha2022}, and secure online assessment infrastructure \cite{Mason2024}. Prompt and effective technical support is also essential, particularly in high-stakes settings \cite{Luxton-Reilly2023}. Responsibilities extend to maintaining reliable server infrastructure \cite{Lau2022}, resolving software glitches \cite{Tsan2022}, and guarding against data breaches \cite{Su2021}.

\subsubsection{Design, Licensing, and Specialized Technologies}
Device-OS compatibility \cite{Lee2022}, adherence to universal design principles \cite{Yadav2022}, and software licensing issues \cite{Tsan2022} are ongoing technological hurdles. The use of proctoring technologies \cite{Wilde2024}, managing technology upgrades \cite{Marshall2020}, and securing data storage and transmission \cite{VanDeGrift2023} present further complications. Faculty training in emerging technologies such as VR/AR \cite{Anyango2021}, infrastructure cost concerns \cite{Saraiva2021}, error handling in digital tools \cite{Hamouda2025}, and mobile learning app development \cite{Patel2024} also demand attention.

\subsubsection{Future Readiness and Inclusive Technology Design}
Planning for technological resilience and future readiness is a critical need in CS education \cite{Izu2025}. Institutions must ensure uninterrupted platform access by maintaining server uptime \cite{Tsan2022} and develop accessible technologies that cater to students with varied learning needs and contexts \cite{Tsan2022b}. These inclusive design practices are essential to achieving long-term equity and sustainability in digital education.

%\subsection{Technological Challenges Faced by Educators}

Tool integration, insufficient infrastructure, and lack of technical expertise burden educators \cite{Thigpen2024,Musaeus2024,Farghally2024}. Faculty struggle to align with industry needs \cite{Valstar2020}. Retrained teachers face difficulties with content and error handling \cite{Vivian2020,Pieper2020}. Assessment and instructional tools (e.g., Scratch, Python) present usability issues \cite{Wang2021,Tshukudu2021,McGill2023}.(Open Educational Resources) OERs lack (Learning Management Systems)LMS support and interactivity \cite{Fowler2023}. AI tools are flawed and hard to adapt \cite{Denny2024}. Poor interface design, inaccessible Integrated development environments (IDEs), and debugging challenges persist \cite{Forden2023,Greifenstein2023,Huff2021,Macann2023}. The COVID-19 shift exposed readiness gaps in online teaching \cite{Perlman2021,Skuratowicz2021,Simmonds2021}.


Technological barriers include poor internet \cite{Izu2025}, inadequate devices \cite{Patel2024}, and compatibility issues \cite{Kirk2022}. Cybersecurity \cite{Brandes2020}, technical support \cite{Weintrop2022}, rapid tech evolution \cite{Ju2020}, and data privacy \cite{Upadhyaya2020} present further challenges. Ensuring accessibility \cite{Kalathas2022}, equitable internet \cite{Nitta2022}, student device provision \cite{Ishizue2024}, and platform management \cite{Berry2022} are necessary. Gaps in digital literacy \cite{Shrestha2022}, secure assessments \cite{Mason2024}, and prompt tech help \cite{Luxton-Reilly2023} are essential. Institutions must also maintain stable servers \cite{Lau2022}, address software glitches \cite{Tsan2022}, and guard against data breaches \cite{Su2021}. Device-OS compatibility \cite{Lee2022}, universal design \cite{Yadav2022}, licensing \cite{Tsan2022}, proctoring tech \cite{Wilde2024}, technology upgrades \cite{Marshall2020}, bandwidth issues \cite{Cook2022}, data security \cite{VanDeGrift2023}, faculty training \cite{Krause-Levy2023}, VR/AR integration \cite{Anyango2021}, infrastructure cost \cite{Saraiva2021}, error handling \cite{Hamouda2025}, future readiness \cite{Izu2025}, and mobile learning apps \cite{Patel2024} complete the picture.Ensuring server stability and uptime for uninterrupted access to learning platforms remains a critical need \cite{Tsan2022}, as does the development of accessible technologies that cater to learners with varied abilities and contexts \cite{Tsan2022b}.


Administrative:

\subsubsection{Systemic and Organizational Barriers}
Educators face systemic barriers such as rigid and outdated curricula, ambiguous role definitions, resource shortages, and imbalanced workloads, all of which hamper effective teaching and professional satisfaction \cite{Farghally2024,Valstar2020,Williams2020,Hill2021}. Professional development (PD) initiatives are frequently reported as lacking formal structure, meaningful incentives, and institutional continuity \cite{McGill2023,Hu2023,Greifenstein2023,Lau2023}. Structural neglect also undermines efforts to promote inclusion and utilize Open Educational Resources (OERs), limiting both reach and efficacy \cite{Hwang2023,Rosenbloom2023,Fowler2023}. Teaching Assistants (TAs) are often burdened with excessive responsibilities without adequate pedagogical training, exacerbating instructional inequities \cite{Zaman2023,Huang2023,Minnes2022,Riese2022,Akhmetov2024}. Similarly, tutors face systemic challenges such as misaligned assignments and poor coordination with instructors, reducing their effectiveness in supporting learners \cite{Brunelle2022,Malik2024}. In many cases, educators are forced to develop instructional materials from scratch due to the lack of aligned standards and institutional support \cite{Repenning2021,Goncharow2021,Ni2021,Jia2022}.

\subsubsection{Institutional Policies and Administrative Complexities}
At the administrative level, institutions grapple with a host of challenges including the absence of clear policies for online education \cite{Kirk2022}, constrained infrastructure budgets \cite{Brandes2020}, and difficulties in meeting accreditation standards for digital formats \cite{Weintrop2022}. Faculty resistance to adopting new technologies, along with concerns about maintaining instructional quality at scale, are widespread \cite{Ju2020,Upadhyaya2020,Kalathas2022}. Additional barriers include legal and ethical ambiguities in online education \cite{Nitta2022}, bureaucratic inertia \cite{Ishizue2024}, and the lack of cohesive institutional strategies and policies \cite{Berry2022}. Crucial actions such as reallocating budgets for digital initiatives \cite{Shrestha2022}, improving institutional readiness \cite{Mason2024}, and implementing fair workload distribution models for faculty \cite{Luxton-Reilly2023} remain unmet in many contexts.

Further, issues surrounding online content ownership \cite{Lau2022}, regulatory compliance for digital instruction \cite{Tsan2022}, and weak interdepartmental collaboration \cite{Su2021} affect educational outcomes. Challenges extend to ensuring consistency in student services \cite{Lee2022}, managing institutional branding and reputation \cite{Tsan2022}, and fostering equitable access to teaching resources \cite{Marshall2020}. Strategic planning \cite{Yadav2022}, process streamlining \cite{VanDeGrift2023}, and updating institutional rules \cite{Krause-Levy2023} are essential for sustainable transformation. Additional complexities include developing innovation ecosystems \cite{Anyango2021}, overseeing third-party educational partnerships \cite{Saraiva2021}, maintaining accessibility standards \cite{Hamouda2025}, and resolving student grievances fairly \cite{Izu2025}. Institutions must also plan for disruptions such as pandemics \cite{Patel2024}, align online education with broader strategic goals \cite{Kirk2022}, and ensure compliance with international regulations \cite{Brandes2020}. Intellectual property rights over online content continue to emerge as a significant concern for faculty \cite{Tsan2022}, emphasizing the need for clear policy frameworks and strategic foresight to ensure the future viability of CS education ecosystems \cite{Tsan2022b}. Additionally, systemic discrimination persists, with some educators reporting that students’ disabilities are seen as instructional barriers due to insufficient structural and administrative support \cite{Yadav2022}.

%\subsection{Administrative and Institutional Challenges}



Educators face systemic issues like rigid curricula, unclear responsibilities, resource shortages, and uneven workloads \cite{Farghally2024,Valstar2020,Williams2020,Hill2021}. PD lacks structure or incentives \cite{McGill2023,Hu2023,Greifenstein2023,Lau2023}. Inclusion efforts and OERs suffer from structural neglect \cite{Hwang2023,Rosenbloom2023,Fowler2023}. TAs are overburdened and undertrained \cite{Zaman2023,Huang2023,Minnes2022,Riese2022,Akhmetov2024}. Tutors face misaligned assignments and coordination issues \cite{Brunelle2022,Malik2024}. Standard misalignment and lack of support force educators to create materials from scratch \cite{Repenning2021,Goncharow2021,Ni2021,Jia2022}.


Institutions face administrative hurdles such as the absence of clear online education policies \cite{Kirk2022}, limited infrastructure budgets \cite{Brandes2020}, and accreditation complexities \cite{Weintrop2022}. Faculty resistance to technology \cite{Ju2020}, assurance of course quality \cite{Upadhyaya2020}, and scaling solutions \cite{Kalathas2022} are common concerns. Legal and ethical ambiguities \cite{Nitta2022}, bureaucratic delays \cite{Ishizue2024}, and the need for unified institutional policies \cite{Berry2022} further hinder smooth transitions. Budget reallocation for digital initiatives \cite{Shrestha2022}, institutional readiness \cite{Mason2024}, and fair workload management \cite{Luxton-Reilly2023} are necessary. Additionally, institutions must tackle online content ownership \cite{Lau2022}, regulatory compliance \cite{Tsan2022}, cross-department collaboration \cite{Su2021}, and consistent student services \cite{Lee2022}. Long-term strategic planning \cite{Yadav2022}, brand and reputation management \cite{Tsan2022}, and equitable resource distribution \cite{Marshall2020} are essential, along with marketing \cite{Cook2022}, streamlined admin processes \cite{VanDeGrift2023}, and adapting existing rules \cite{Krause-Levy2023}. Cultivating innovation \cite{Anyango2021}, managing third-party partnerships \cite{Saraiva2021}, upholding accessibility standards \cite{Hamouda2025}, addressing student grievances \cite{Izu2025}, disruption preparedness \cite{Patel2024}, aligning online learning to institutional strategy \cite{Kirk2022}, and ensuring international regulatory compliance \cite{Brandes2020} are also critical.Among institutional issues, intellectual property rights for online teaching content are a growing concern \cite{Tsan2022}, and the formulation of forward-looking strategic plans is vital for the sustainable evolution of online education ecosystems \cite{Tsan2022b}.Systemic challenges persist in institutions where students' disability status is perceived as a barrier to participation. Teachers and administrators cite inadequate structural support for enabling full engagement of students with disabilities in computing education \cite{Yadav2022}.



training:

\subsubsection{Limited Pedagogical Preparation and Equity Training}
Many CS educators begin teaching with minimal or no formal pedagogical training, limiting their instructional effectiveness \cite{Krause-Levy2022,Akhmetov2024}. Professional development (PD) opportunities are often narrow in scope, short in duration, or inaccessible due to institutional and logistical constraints \cite{Sentance2021,Thigpen2024}. There is a noticeable scarcity of equity-focused training, which hampers educators’ readiness to address diversity, equity, and inclusion (DEI) concerns in CS education \cite{Hwang2023,Yadav2022Review,Parthasarathy2024,Friend2022}. Additionally, institutional constraints such as lack of time and funding often hinder deeper PD engagement \cite{Nugent2022,Grover2024}. Existing PD programs frequently fail to differentiate between educator roles (e.g., tutors, TAs, and classroom teachers), further reducing their effectiveness \cite{Krause-Levy2022}.

\subsubsection{Challenges for K-12 and Pre-Service Educators}
K-12 and pre-service CS educators face unique professional development challenges. These include limited access to structured PD, insufficient support for curriculum development, and minimal integration of ethics into CS teaching \cite{Shanley2023,Macann2023,DiPaola2023,Jetzinger2024,Grover2024,Greifenstein2023,Hu2023}. These educators often struggle to stay current with evolving curricular expectations while receiving inadequate institutional backing for pedagogical innovation.

\subsubsection{Digital and Online Teaching Preparedness}
The rise of online education necessitates upskilling faculty in digital pedagogy, yet training opportunities remain insufficient \cite{Weintrop2022}. Continuous development programs are lacking \cite{Ju2020}, and there is limited institutional support for integrating new teaching tools \cite{Upadhyaya2020}. Training is needed in digital instructional strategies \cite{Kalathas2022}, mentorship initiatives \cite{Nitta2022}, and technology updates \cite{Ishizue2024}. Institutions are encouraged to foster innovation \cite{Berry2022}, evaluate training effectiveness \cite{Shrestha2022}, and deliver comprehensive pedagogy workshops \cite{Mason2024}.

\subsubsection{Sustaining Long-Term Professional Development}
Sustaining effective PD involves ensuring the availability of training for technical support staff \cite{Lau2022}, multimedia content creation \cite{Tsan2022}, and assessment integrity in online settings \cite{Su2021}. Ongoing institutional priorities also include mental health support training \cite{Lee2022}, leadership development \cite{Yadav2022}, peer learning communities \cite{Tsan2022}, and specialization in emerging technologies such as AI and VR \cite{Wilde2024}. Addressing faculty resistance to change \cite{Marshall2020}, offering flexible and discipline-specific training \cite{Anyango2021,Cook2022}, and ensuring long-term PD impact through assessment and incentives \cite{VanDeGrift2023,Krause-Levy2023} are also essential.

\subsubsection{Specialized Training Dimensions}
Professional development must also include modules on data privacy \cite{Saraiva2021}, build a culture of continuous learning \cite{Hamouda2025}, and emphasize hands-on learning sessions \cite{Izu2025}. Equitable access to digital readiness tools \cite{Patel2024}, inclusivity training \cite{Kirk2022}, and emergency response preparedness \cite{Brandes2020} are vital. Hybrid teaching competencies \cite{Weintrop2022} and structured mentorship models \cite{Ju2020} should be institutionalized to support all educator levels. Additional attention is needed to train technical support staff for managing digital platforms \cite{Tsan2022} and to develop leadership competencies among online education administrators \cite{Tsan2022b}.

\subsubsection{Foundational Gaps in CT and Platform Navigation}
PD programs often reveal fundamental misunderstandings of computational thinking (CT), with educators misinterpreting it as simple computer use or lacking prior coding experience \cite{Jocius2021}. Many struggle to integrate CT meaningfully into disciplinary contexts and require sustained coaching and exposure. Virtual PD formats introduce challenges such as navigating unfamiliar digital platforms, collaborating effectively, and communicating through online tools—particularly during live coding sessions \cite{Jocius2021}.

\subsubsection{Support for Special Education Teachers}
Special education teachers face distinct hurdles when integrating CT using Universal Design for Learning (UDL) principles. These challenges include difficulty in offering multiple modes of content representation and a lack of systemic support and coaching during lesson planning and execution \cite{Yadav2022}.

\subsubsection{Challenges with Instructional Media and Engagement}
Instructor preparation is also impacted by the limitations of current instructional media. Live coding often induces pacing issues and cognitive overload, while video content creation can generate performance anxiety. Traditional textbooks and passive videos frequently fail to engage students effectively due to their non-interactive nature \cite{Mahoney2023}.

%\subsection{Training and Professional Development Challenges}


Many CS educators begin teaching with little pedagogical training \cite{Krause-Levy2022,Akhmetov2024}. PD is often narrow, short, or inaccessible \cite{Sentance2021,Thigpen2024}. Equity-focused training is scarce, limiting DEI preparedness \cite{Hwang2023,Yadav2022Review,Parthasarathy2024,Friend2022}. Institutional constraints (time, funding) limit engagement \cite{Nugent2022,Grover2024}. PD also fails to differentiate between roles (e.g., tutors vs. teachers) \cite{Krause-Levy2022}.K-12 and Pre-Service Teachers face unique challenges related to professional development \cite{Shanley2023,Macann2023,DiPaola2023,Jetzinger2024}, curriculum development \cite{Grover2024,Greifenstein2023}, and ethics integration \cite{Hu2023}. 

Online education calls for upskilling faculty, but there remains a shortage of training opportunities \cite{Weintrop2022}, insufficient continuous development programs \cite{Ju2020}, and limited support for new tools \cite{Upadhyaya2020}. Pedagogical training for digital teaching \cite{Kalathas2022}, mentorship programs \cite{Nitta2022}, and technological proficiency updates \cite{Ishizue2024} are needed. Institutions must encourage innovation \cite{Berry2022}, assess training outcomes \cite{Shrestha2022}, and offer full-spectrum pedagogy workshops \cite{Mason2024}. Sustaining professional development \cite{Luxton-Reilly2023}, tech staff training \cite{Lau2022}, multimedia content creation \cite{Tsan2022}, and online assessment integrity training \cite{Su2021} remain ongoing priorities. Supporting mental health roles \cite{Lee2022}, leadership grooming \cite{Yadav2022}, peer learning communities \cite{Tsan2022}, and emerging tool specialization (e.g., AI, VR) \cite{Wilde2024} are important. Additionally, institutions should address resistance to change \cite{Marshall2020}, offer flexible training \cite{Cook2022}, and measure long-term training impact \cite{VanDeGrift2023}. Incentives \cite{Krause-Levy2023}, discipline-specific training \cite{Anyango2021}, data privacy modules \cite{Saraiva2021}, continuous learning culture \cite{Hamouda2025}, hands-on sessions \cite{Izu2025}, equity in digital readiness \cite{Patel2024}, inclusivity training \cite{Kirk2022}, emergency response prep \cite{Brandes2020}, hybrid competency development \cite{Weintrop2022}, and structured mentorship programs \cite{Ju2020} are further essential strategies.Training technical support staff to handle digital platforms effectively is important \cite{Tsan2022}, along with initiatives to develop leadership competencies among online education administrators \cite{Tsan2022b}.Professional development programs often reveal gaps in teachers' initial understanding of computational thinking (CT), with some equating it to mere computer use. Many educators also lack prior coding experience, struggle with CT integration into disciplinary teaching, and require sustained scaffolding and exposure \cite{Jocius2021}. In virtual PD formats, teachers also report difficulties navigating digital platforms, collaborating through unfamiliar tools, and effectively communicating during online coding sessions \cite{Jocius2021}. 

Another dimension includes the lack of preparation for special education teachers to integrate CT using Universal Design for Learning (UDL) principles. These educators face difficulties providing multiple means of representation and require stronger support systems and coaching during planning and execution phases \cite{Yadav2022}.

Instructor preparation is also challenged by the limitations of current instructional media. Live coding introduces pacing and multitasking stress, while creating effective video content introduces performance anxiety and cognitive burden. Traditional books and videos often fail to engage students due to their passive or non-interactive nature \cite{Mahoney2023}.

Social:
Socio-cultural challenges in CS education emerge from broader systemic inequalities, cultural mismatches, and a lack of inclusion in pedagogical design. Educators often face underrepresentation, cultural misalignment, and resistance to diversity, equity, and inclusion (DEI) efforts \cite{Hwang2023,Everson2022,Rosenbloom2023}. Instructional materials frequently fail to represent the lived realities of diverse learners \cite{Greifenstein2023,Simmonds2021}, contributing to exclusionary experiences. International educators additionally confront linguistic marginalization \cite{Markel2021,Riese2021,Minnes2022,Krause-Levy2022}, which limits their participation and comfort in collaborative environments. Emerging technologies such as AI introduce new concerns, including embedded bias and the disempowerment of marginalized voices \cite{Lau2023,Sheard2024,Mahon2024}. The creation of inclusive classrooms is further constrained by limited TA support and inadequate collaboration-sensitive technologies \cite{Huang2023,Akhmetov2024}.
\subsubsection{Inequities in Online and Global Education}

The transition to online education amplifies socio-cultural disparities. Digital divides across income groups and geographical regions inhibit access \cite{Upadhyaya2020}, while pedagogical norms often reflect dominant cultures and exclude alternative approaches \cite{Kalathas2022}. Language barriers persist in multinational classrooms, reducing participation and confidence among non-native speakers \cite{Nitta2022}. Learners’ access and outcomes are also shaped by family support systems \cite{Ishizue2024}, societal doubts about the credibility of online degrees \cite{Berry2022}, and persistent structural exclusion \cite{Shrestha2022}. Additionally, limited cross-cultural understanding \cite{Mason2024}, socio-economic constraints \cite{Luxton-Reilly2023}, and restricted access for marginalized groups \cite{Lau2022} exacerbate learning inequities.

\subsubsection{Cultural Responsiveness and Inclusive Design}

Institutions must recognize and respond to cultural nuances in communication \cite{Tsan2022} and ensure curriculum relevance across academic and regional backgrounds \cite{Su2021}. Acknowledging inconsistencies in family support \cite{Lee2022} and addressing the risk of stereotype reinforcement in virtual settings are critical \cite{Yadav2022}. Inclusive design involves not just content diversity but also socially constructive environments \cite{Tsan2022}, as online learning can hinder social development \cite{Wilde2024}. Promoting global citizenship \cite{Marshall2020}, facilitating integrity across cultures \cite{Cook2022}, and supporting displaced and refugee learners \cite{VanDeGrift2023} further define the socio-cultural agenda in CS education.

\subsubsection{Addressing Identity-Based and Contextual Challenges}

Persistent gender gaps in technology adoption \cite{Krause-Levy2023}, cultural and political sensitivities \cite{Anyango2021}, and uneven access to technology across diverse cultural groups \cite{Saraiva2021} remain pressing. Institutions must tackle generational divides in tech usage \cite{Hamouda2025}, help communities resist displacement due to educational reform \cite{Izu2025}, and assist students affected by conflict \cite{Patel2024}. Strategies should also prioritize creating inclusive virtual classrooms \cite{Kirk2022}, linguistic adaptation for digital content \cite{Brandes2020}, and bridging parental digital literacy gaps \cite{Weintrop2022}. The promotion of civil dialogue in online spaces \cite{Ju2020}, prevention of rural brain drain \cite{Upadhyaya2020}, and inclusion of indigenous perspectives in curricular design \cite{Kalathas2022} are vital to fostering equity.

\subsubsection{Urgent Priorities and Remedies}

A recurring concern is the closure of the digital divide for disadvantaged learners \cite{Tsan2022}. This includes enhancing technological access, representation, and adaptability of content. Equally important is addressing implicit bias and stereotype propagation in online learning environments, which hinder the formation of inclusive and empowering virtual communities \cite{Tsan2022b}. Without culturally responsive and socially just design in both content and delivery, socio-cultural inequities will continue to undermine educational progress.

%\subsection{Socio-cultural Challenges Faced by Educators}




Educators face underrepresentation, cultural mismatch, and DEI resistance \cite{Hwang2023,Everson2022,Rosenbloom2023}. Materials often fail to reflect diverse realities \cite{Greifenstein2023,Simmonds2021}. International educators experience linguistic exclusion \cite{Markel2021,Riese2021,Minnes2022,Krause-Levy2022}. AI tools raise concerns about bias and disempowerment \cite{Lau2023,Sheard2024,Mahon2024}. Inclusive classrooms require better support for TAs and collaboration-sensitive tools \cite{Huang2023,Akhmetov2024}.


Online education exposes socio-cultural inequities, such as the digital divide \cite{Upadhyaya2020}, cultural differences in pedagogy \cite{Kalathas2022}, and language barriers in multinational classrooms \cite{Nitta2022}. Family support structures \cite{Ishizue2024}, societal skepticism about online degrees \cite{Berry2022}, and inclusion barriers \cite{Shrestha2022} impact learner participation. Cross-cultural understanding \cite{Mason2024}, socio-economic limitations \cite{Luxton-Reilly2023}, and marginalized access issues \cite{Lau2022} further compound the challenge. Institutions must consider cultural cues in communication \cite{Tsan2022}, support for diverse academic backgrounds \cite{Su2021}, and inconsistent family support \cite{Lee2022}. Online interactions also risk perpetuating stereotypes \cite{Yadav2022}, highlighting the need for inclusive content \cite{Tsan2022}, and impacting social development \cite{Wilde2024}. Promoting global citizenship \cite{Marshall2020}, academic honesty across cultures \cite{Cook2022}, and support for refugees \cite{VanDeGrift2023} are critical. Gender gaps in tech use \cite{Krause-Levy2023}, sociopolitical sensitivities \cite{Anyango2021}, and tech access across diverse cultural settings \cite{Saraiva2021} remain urgent. Additionally, managing generational tech divides \cite{Hamouda2025}, mitigating community displacement \cite{Izu2025}, assisting conflict-affected learners \cite{Patel2024}, supporting inclusive virtual classrooms \cite{Kirk2022}, linguistic adaptation \cite{Brandes2020}, parental digital gaps \cite{Weintrop2022}, online dialogue civility \cite{Ju2020}, rural brain drain \cite{Upadhyaya2020}, and indigenous inclusion in content \cite{Kalathas2022} complete the socio-cultural profile.Closing the digital divide for disadvantaged students is a recurring concern \cite{Tsan2022}, while combating stereotypes and implicit bias in online interactions is essential for creating inclusive virtual communities \cite{Tsan2022b}.





Parental:

\subsubsection{Lack of Awareness and Support}

A significant challenge is the lack of parental and community understanding of computer science (CS) and its career opportunities, which hinders student motivation and engagement \cite{Samarasekara2023}. Many parents are unfamiliar with the nature of CS as a discipline, limiting their ability to support learners at home. Without informed family encouragement, students—particularly those from underrepresented backgrounds—may not pursue or persist in computing pathways. Therefore, effective outreach and education for families remain critical in making CS more accessible and better supported at home.

\subsubsection{Identity-Based Barriers to Trust and Authority}

Pre-service teachers—particularly women of color—express fears of not being taken seriously by students or parents due to their identities, which affects confidence and trust-building in the classroom environment \cite{Everson2022}. These perceived barriers to professional legitimacy can undermine classroom authority, limit authentic engagement with families, and contribute to emotional labor for early-career educators from marginalized communities.

\subsubsection{Community Engagement Logistics and Continuity}

Community involvement in CS education also faces structural hurdles. Initiatives like service-learning and capstone projects, while valuable for applied learning, require extensive coordination with external partners \cite{Hooshangi2025}. These collaborations often involve significant logistical planning, such as partner training and alignment of goals. Moreover, the sustainability of such programs is threatened by organizational turnover and inconsistent availability of community collaborators, complicating efforts to maintain engagement across student cohorts.

%\subsection{Parental and Community Involvement Challenges}

A significant challenge is the lack of parental and community understanding of computer science (CS) and its career opportunities, which hinders student motivation and engagement \cite{Samarasekara2023}. Effective outreach and education for families remain critical in making CS more accessible and supported at home.

Pre-service teachers—particularly women of color—express fears of not being taken seriously by students or parents due to their identities, which affects confidence and trust-building in the classroom environment \cite{Everson2022}.

Additionally, community involvement faces structural issues. Service-learning and capstone projects require extensive coordination with external partners, including logistical efforts like training and maintaining relationships amidst organizational turnover. These challenges complicate consistent community engagement across cohorts \cite{Hooshangi2025}.


% Common themes of Parental and Community Involvement Challenges in our reviewed papers include the lack of parental and community understanding of computer science (CS) and its career opportunities for educators, which hinders student motivation and engagement \cite{Samarasekara2023}.
% Pre-service teachers—particularly women of color—express fears of not being taken seriously by students or parents due to their identities, which affects confidence and trust-building in the classroom environment \cite{Everson2022}.
% Additionally, community involvement faces structural issues. Service-learning and capstone projects require extensive coordination with external partners, including logistical efforts like training and maintaining relationships amidst organizational turnover. These challenges complicate consistent community engagement across cohorts \cite{Hooshangi2025}.

\subsection{Sense of Community/Belonging Challenges}

An educator’s sense of belonging encompasses feeling connected, supported, and valued within professional communities, whether within schools, departments, or broader networks. This sense is vital for reducing isolation, fostering professional growth, and enhancing teaching effectiveness.

\subsubsection*{Isolation and Lack of Peer Connection}
Many CS educators experience professional isolation, often being the sole CS teacher in their schools, which limits collegial dialogue and feedback opportunities \cite{Ni2021,Yadav2022,Basu2022,Flatland2022}. Such isolation hinders the development of professional identity and reduces access to shared teaching practices.

\subsubsection*{Lack of Collaborative and Supportive Environments}
Teachers often lack opportunities for meaningful collaboration or peer mentorship \cite{Samarasekara2023,Fowler2023,Skuratowicz2021,Simmonds2021,Riese2022,Kussmaul2022,Haglund2024}. TA communities, in particular, struggle with disconnected workflows and insufficient shared professional spaces despite recognizing the benefits of collaboration.

\subsubsection*{Challenges in Collaborative Processes and Communication}
Remote formats and fragmented team structures have disrupted collaborative lesson planning and peer coordination \cite{Denny2024,Lehtimki2022,Akhmetov2024,Brunelle2022,Lee2022}, weakening instructor-TA communication and impeding the development of shared community values.

\subsubsection*{Inclusivity and Identity-Related Challenges}
Perceptions of CS as niche or inaccessible, coupled with structural and social barriers, hinder inclusivity and connection \cite{Hwang2023,Lau2023,Rosenbloom2023,Everson2022,Huang2023}. Implicit biases, exclusionary practices, and cultural stigmas undermine students’ and educators’ sense of belonging in CS spaces.

\subsubsection*{Lack of Common Understanding and Systemic Support}
Gaps in shared terminology, resource infrastructure, and community stewardship reveal systemic challenges to fostering cohesive teaching communities \cite{Munasinghe2021,Marshall2020,Parthasarathy2024,Blanchard2022}. The absence of institutional frameworks to support community-building efforts compounds this issue.

\subsubsection*{Internal Team Dynamics}
Even within support structures like TA teams, ethical conflicts and insufficient conflict-resolution mechanisms challenge cohesion and trust \cite{Riese2021,Minnes2022}.

This isolation limits opportunities for collegial dialogue, feedback, and the exchange of effective teaching practices, ultimately stunting professional identity development \cite{Ni2021,Yadav2022,Basu2022,Flatland2022}. Compounding this issue is the lack of collaborative and supportive environments, where teachers and TAs often struggle to access meaningful peer mentorship or sustained professional communities despite the known benefits of collaboration \cite{Samarasekara2023,Fowler2023,Skuratowicz2021,Simmonds2021,Riese2022,Kussmaul2022,Haglund2024}. This challenge is further exacerbated by disruptions to collaborative processes and communication, particularly in remote or hybrid teaching formats that weaken team cohesion and hinder instructor-TA coordination \cite{Denny2024,Lehtimki2022,Akhmetov2024,Brunelle2022,Lee2022}.

In addition, many educators face inclusivity and identity-related challenges that prevent a full sense of belonging within the CS education ecosystem. Structural and social stigmas, implicit bias, and perceptions of CS as inaccessible marginalize both students and educators, particularly those from underrepresented groups \cite{Hwang2023,Lau2023,Rosenbloom2023,Everson2022,Huang2023}. The lack of common understanding and systemic support for building community among educators reflects a deeper problem: an absence of shared terminology, resource ecosystems, and institutional mechanisms that could foster collective identity and stewardship \cite{Munasinghe2021,Marshall2020,Parthasarathy2024,Blanchard2022}. Even within structured teams like TA groups, unresolved internal team dynamics—including ethical disagreements and a lack of conflict-resolution practices—further challenge efforts to build a cohesive, supportive teaching environment \cite{Riese2021,Minnes2022}.


Isolation, limited collaboration, and misalignment with institutional culture diminish educator belonging \cite{Ni2021,Yadav2022,Nugent2022}. Many lack peer networks or support even in PD \cite{Skuratowicz2021,Basu2022}. Fragmented TA teams and remote formats hinder team dynamics \cite{Akhmetov2024,Riese2022,Minnes2022,Haglund2024,Lehtimki2022}. Cultural pressures and gender bias reduce belonging \cite{Rosenbloom2023,Everson2022,Hwang2023}. OERs lack collaboration incentives \cite{Fowler2023,Blanchard2022}. Classroom group dynamics and miscommunication further impair inclusion \cite{Huang2023,Brunelle2022}. High school teachers often lack learning communities \cite{Flatland2022,Parthasarathy2024}.


Building community online is hindered by lack of connection \cite{Berry2022}, reduced peer collaboration \cite{Shrestha2022}, and fragile teacher-student rapport \cite{Mason2024}. Students may feel isolated \cite{Luxton-Reilly2023}, disengaged \cite{Lau2022}, or disconnected \cite{Tsan2022}. Educators attempt to encourage belonging \cite{Su2021}, emotional presence \cite{Lee2022}, and identity formation \cite{Yadav2022}. Peer interactions \cite{Tsan2022}, meaningful instructor relationships \cite{Wilde2024}, social spaces \cite{Marshall2020}, and anonymous environments \cite{Cook2022} hinder community-building. Active discussion participation \cite{VanDeGrift2023}, shared student identity \cite{Krause-Levy2023}, and safe storytelling spaces \cite{Anyango2021} are promoted. Virtual clubs \cite{Saraiva2021}, inclusive environments \cite{Hamouda2025}, and mentorship programs \cite{Izu2025} aid bonding. A welcoming tone \cite{Patel2024}, learning ownership \cite{Kirk2022}, and activity access equity \cite{Brandes2020} are key. Psychological tolls of online learning \cite{Weintrop2022}, community contributions \cite{Ju2020}, virtual orientation \cite{Upadhyaya2020}, student pride \cite{Kalathas2022}, common areas \cite{Nitta2022}, text-based rapport challenges \cite{Ishizue2024}, support culture \cite{Berry2022}, and alumni–student ties \cite{Shrestha2022} complete the picture.
Ensuring student retention and engagement through relational strategies and emotionally responsive practices is a central priority \cite{Tsan2022}, complemented by efforts to cultivate a strong sense of community and belonging among online learners \cite{Tsan2022b}.




































































\section{Background and related work}

\subsection{Who Are CS Educators?}

In computing education, the term \textit{CS educators} encompasses a diverse set of stakeholders involved in teaching, mentoring, and supporting learners at various academic levels and instructional contexts. This includes:

\textbf{Instructors and Faculty:} These are educators responsible for designing and delivering a wide range of CS curricula, including introductory courses like CS1 \cite{Vahid2024,Vahid2024b}, capstone courses \cite{Hooshangi2025}, ethics and accessibility integration \cite{Hu2023,Parthasarathy2024}, AI and machine learning in K-12 settings \cite{Grover2024,Jetzinger2024,DiPaola2023}, and advanced pedagogical strategies such as inclusive design \cite{Patel2024}. Faculty members are also central to shaping national computing standards \cite{Thigpen2024,McGill2024}, implementing curriculum-wide reform \cite{Musaeus2024}, and mentoring future CS teaching-focused faculty \cite{Farghally2024}. Their experiences are also being studied in the context of AI tool integration \cite{Sheard2024,Cucuiat2024} and debugging as a computational thinking practice \cite{Macann2023}.

\textbf{Teaching Assistants (TAs):} TAs play a critical role in providing feedback, tutoring support, and classroom management in large or complex CS courses \cite{Zaman2023,Akhmetov2024,Haglund2024}. Their responsibilities range from grading and content delivery to helping students understand subtle programming concepts \cite{Haglund2024}. The rise of AI-powered teaching tools like TA-Bot and other automated systems is aimed at augmenting TA workflows in large-scale settings \cite{Forden2023,Denny2024}. Effective TA management and feedback literacy are essential for their pedagogical impact \cite{Cheng2024,Akhmetov2024}.

\textbf{Tutors:} Tutors, whether human or AI-driven, offer one-on-one or small-group support for learners. Systems like \textit{Iris}, an AI-based tutor, provide real-time, context-aware support that fosters independent problem-solving \cite{Bassner2024}. Similarly, tools like \textit{TeachNow} enable volunteer teachers to deliver spontaneous 1:1 assistance in massive online courses \cite{Malik2024}. Tutors are also supported by just-in-time interventions that improve their instructional performance \cite{Cheng2024}.

\textbf{K-12 and Pre-Service Teachers:} A significant portion of computing educators operate in primary and secondary school settings. These educators face unique challenges related to professional development \cite{Shanley2023,Macann2023,DiPaola2023,Jetzinger2024}, curriculum development \cite{Grover2024,Greifenstein2023}, and ethics integration \cite{Hu2023}. Their perspectives shape the landscape of early computing education.

This comprehensive view acknowledges that CS educators are not a monolithic group but rather a network of professionals—faculty, TAs, tutors, and K-12 teachers—working across multiple modalities, technologies, and learner demographics.



\section{Challenges Identified}
After thoroughly reviewing 106 context-relevant papers, we identified challenges, which we have thematically categorized as mentioned in the following subsections.




\subsection{Pedagogical Challenges in CS Education}

Pedagogical challenges faced by Computer Science (CS) teachers and educators refer to the multifaceted difficulties and obstacles that educators encounter in effectively designing, delivering, and adapting computer science instruction. These challenges stem from the inherent nature of computer science as a discipline, the rapid evolution of technology, the societal implications of computing, and the institutional contexts in which teaching occurs.


\textbf{List of Pedagogical Challenges}

Educators frequently lack the pedagogical content knowledge required for effective CS instruction, needing to adapt continuously to diverse student needs and contexts \cite{Thigpen2024}. Students often struggle to transfer knowledge between sessions and peers, complicating collaborative learning \cite{Musaeus2024}.

Preparation gaps among instructors and TAs hinder student motivation, often due to poor communication, unclear objectives, and social anxiety \cite{Farghally2024}. Instructors face conflicting guidance on teaching style, particularly with language-specific conventions \cite{Kirk2024}.

Integrating industry practices remains uneven, especially in theory-heavy courses like algorithms \cite{Valstar2020}. A shortage of qualified CS teachers persists, with pedagogical training often insufficient \cite{Williams2020, Pieper2020}.

Student enthusiasm drops when instructional methods or infrastructure are ineffective \cite{Venn-Wycherley2020}, and resilience is often lacking \cite{Venn-Wycherley2020}. Many instructors lack formal training and familiarity with evidence-based strategies \cite{Goncharow2021}. Students also struggle to transfer skills between languages \cite{Tshukudu2021}.

Defining CS’s academic core and aligning it with pedagogy is difficult as standards evolve \cite{Ni2021}, and technical content often overshadows pedagogical focus \cite{Vahid2024}. Teacher qualifications and professional development remain ongoing issues \cite{Denny2024}.

Lesson alignment with standards like CSTA is challenging, especially for new teachers \cite{McGill2023}. Translating culturally responsive pedagogy into practice, embedding cultural content, and fostering student-led learning remain difficult under curriculum constraints \cite{Hwang2023}. Integrating social justice content adds further complexity \cite{Hwang2023}.

OER use introduces challenges in coverage, quality, customization, and currency in a rapidly evolving field \cite{Fowler2023}. Increased reliance on AI can hinder foundational learning and requires new prompt-crafting skills \cite{Lau2023}. CS1/CS2 courses still prioritize syntax over conceptual understanding \cite{Lau2023}.

Project-based learning in CS is difficult due to topic complexity \cite{Samarasekara2023}. Resistance to centralized textbooks and digital tech integration adds friction \cite{Samarasekara2023}. Teachers also face skepticism when incorporating abolitionist or justice-oriented content \cite{Rosenbloom2023}, contributing to techno-nihilism and diminished pedagogical imagination \cite{Rosenbloom2023}.

Feedback systems often confuse students, especially when relying on legacy platforms \cite{Forden2023}. Gamification tools in CS1 are debated in terms of relevance and complexity \cite{Forden2023}. TAs often lack deep content knowledge, limiting the quality of grading and support \cite{Zaman2023}.

Varying prerequisite knowledge complicates task selection and goal-setting \cite{Sauerwein2023}. Debugging remains a consistent challenge for students and instructors alike \cite{Macann2023}. Educators frequently undervalue clear learning objectives and struggle with crafting exemplary materials \cite{Saqr2024}. Many rely on log data without meaningful pedagogical feedback and fail to support isolated learners \cite{Singh2020}.


\subsection{Classroom Management Challenges}

Classroom management challenges in CS education involve organizing diverse learning environments, coordinating instruction, and fostering inclusive participation among students, tutors, and TAs. Educators must reflect on teaching practices to support diverse learners while addressing issues like social anxiety, lack of confidence, and limited communication skills \cite{Thigpen2024,Musaeus2024,Farghally2024}. Large class sizes overwhelm instructors, making it difficult to balance content delivery and individual attention \cite{Valstar2020,Goncharow2021}.

Students often face conceptual and technical difficulties \cite{Pieper2020}, lack interest or problem-solving resilience \cite{Venn-Wycherley2020}, and struggle with independent learning in CS1 courses \cite{Vahid2024}. Delayed feedback due to manual grading and time constraints hampers learning \cite{Wang2021}. Hidden AI usage and taboo around such tools limit transparency in student behaviors \cite{Lau2023}.

Limited resources and increasing enrollments reduce individualized support \cite{Samarasekara2023,Forden2023}, while TA responsiveness suffers in large classes \cite{Zaman2023}. TAs often manage interpersonal issues including harassment and psychological safety \cite{Huang2023}, while group projects require balancing participation and conflict \cite{Lee2021}. Online platforms continue to pose challenges for some instructors \cite{Perlman2021}.

Tutors face unequal time distribution between unprepared and advanced students, long queues, and concerns over unpermitted external help \cite{Markel2021,Rusak2021}. Diversity in learner backgrounds—including special needs and varied prior knowledge—adds complexity \cite{Riese2021}. Passive and outcome-focused students, classroom conflicts, and inefficient use of in-class time remain barriers \cite{Riese2021}.

TAs and tutors face difficulties in adapting teaching strategies, often lacking confidence or clarity in delivery \cite{Goletti2021}. Student learning styles vary; some prefer unguided exploration, while others struggle with engagement during discussion \cite{Sentance2021}. Unequal effort in group work and project-based courses demands careful monitoring \cite{Hooshangi2025}. Tools like GenderMag may be seen as additional burden \cite{Patel2024}, and managing large-scale capstone courses requires tailored strategies \cite{Hooshangi2025}.

TA coordination issues—such as poor communication, unbalanced workload, and last-minute cancellations—disrupt classroom flow \cite{Minnes2022,Akhmetov2024}. Systems like “week experts” increase stress and reduce consistency \cite{Akhmetov2024}. Heavy grading loads and inefficient office hours hinder instructional flexibility and fairness \cite{Kumar2022,Riese2022,Brunelle2022}. Inconsistent final project guidance and uneven team performance further complicate teaching \cite{Kao2020,Kussmaul2022}. Proficiency gaps in essential tools like Unix remain persistent \cite{Kussmaul2022}.


\subsection{Assessment and Evaluation Challenges}

Assessment and evaluation challenges revolve around the effective measurement of student learning outcomes and the quality of instructional responses in computer science education. These challenges span from developing reliable assessment instruments to ensuring scalable, equitable, and pedagogically meaningful feedback systems.

A critical concern lies in designing rubrics and evaluation frameworks to assess student interactions with code. For example, Esche \cite{Esche2024} introduced a structured rubric to evaluate the quality of support staff responses to student code queries, highlighting the need for consistent and pedagogically grounded feedback practices.

As enrollment in programming courses increases, educators face scalability issues that impact the quality of assessment and student feedback. Akhmetov et al. \cite{Akhmetov2024} addressed this challenge by implementing a tiered TA management structure in a large CS1 course, including dedicated teams for tasks such as plagiarism detection and student support, thereby improving course-wide evaluation consistency.

To further address scale and objectivity, the integration of Automated Programming Assessment Systems (APASs) has emerged as a formative assessment solution. Sauerwein et al. \cite{Sauerwein2023} proposed a success model for APASs, which provides timely, data-driven feedback and supports educators in managing increasingly heterogeneous student populations.

Finally, the adoption of AI-powered teaching assistants introduces new dimensions to feedback and evaluation. Denny et al. \cite{Denny2024} found that while digital TAs offer scalable and personalized feedback, their effectiveness hinges on their ability to scaffold learning rather than replace problem-solving with direct answers. Students appreciated these systems most when they facilitated autonomy and deep understanding.

Overall, these challenges underscore the need for well-designed, equitable, and technologically adaptive assessment practices to ensure effective learning in diverse CS classrooms.



\subsection{Emotional and Psychological Challenges}
Educators, including teachers, tutors, and TAs, face emotional and psychological challenges that impact their well-being, teaching efficacy, and job satisfaction. These stem from demands like managing students, adapting to curricula and technology, administrative pressures, and navigating institutional dynamics—leading to stress, burnout, anxiety, and low self-esteem.

Teachers’ awareness of their growth can guide development \cite{Thigpen2024}, yet the belief that teaching ability is innate can hinder motivation \cite{Farghally2024}. Female, rural, and early-career teachers report lower self-esteem in CS \cite{Vivian2020}, reducing instructional effectiveness, especially when students’ early interest fades due to lack of support \cite{VennWycherley2020}.

Educators often recreate resources despite curricula \cite{Goncharow2021}, face identity fragmentation \cite{Tshukudu2021,Ni2021}, and feel unsupported \cite{Vahid2024}, highlighting the need for adaptive, exploratory teaching environments \cite{Denny2024}. Cognitive overload from unclear expectations, CRT ambiguity, and fear of reputational risk adds strain \cite{Hwang2023,Fowler2023}, compounded by standardized testing and disengaged students \cite{Lau2023}.

Resource constraints, overwork, and resistance to systemic critique contribute to emotional exhaustion and fear of job loss \cite{Samarasekara2023,Rosenbloom2023}. Misunderstood assessment tools and overwhelming automated feedback also demotivate \cite{Forden2023}. TAs frequently confront harassment and discrimination without emotional preparation \cite{Huang2023}.

Students’ frustration with errors and teachers’ insecurity in CS content challenge confidence and engagement \cite{Macann2023,Greifenstein2023,Hill2021}. Accessibility issues, especially for BVI students, emotionally burden educators \cite{Huff2021}, while doubts about CS relevance and breaks in instruction reduce enthusiasm \cite{Repenning2021}.

Empathy and mistake-tolerant environments are critical \cite{Lee2021}. The pandemic magnified stress, job insecurity, and anxiety about unfamiliar platforms \cite{Perlman2021,Skuratowicz2021}. Tutors manage both their own and students’ emotions under academic stress \cite{Markel2021}, and fears about technology or discomfort with student interactions further complicate teaching \cite{Simmonds2021,Riese2021}.

Limited pedagogical training and classroom management challenges lower tutor confidence \cite{Goletti2021}, while some educators resist training due to overconfidence or pandemic-related fatigue \cite{Kumar2021}. Many feel overwhelmed by computing jargon and hesitant to engage at all \cite{Munasinghe2021}. These insights underscore the urgent need for mental health support, institutional flexibility, and context-sensitive professional development.



\subsection{Technological Challenges Faced by Educators}

CS educators, tutors, and TAs face persistent technological challenges including tool integration, inadequate resources, and limited technical support. Many educators struggle with teaching CS due to lack of prior experience, difficulties with programming, data analysis, and algorithms \cite{Thigpen2024}. Primary teachers cite technical problems and insufficient resources \cite{Musaeus2024}, and staffing issues arise from a shortage of qualified faculty \cite{Farghally2024}. Faculty often lack exposure to industry practices and struggle to teach topics like software maintenance and soft skills \cite{Valstar2020}. There is disagreement over the inclusion of industry preparation in curricula \cite{Valstar2020}.

Retrained teachers cite content gaps and difficulties addressing student misunderstandings and programming errors \cite{Vivian2020,Pieper2020}. Poor infrastructure and teaching quality can reduce student interest \cite{VennWycherley2020}. Despite national curriculum standards, instructional approaches remain ad hoc \cite{Goncharow2021}. Visual assessments and transitions between languages like Scratch and Python present challenges \cite{Wang2021,Tshukudu2021}. Digital tools face usability issues, such as submission form failures and storage limitations \cite{McGill2023}.

Open Educational Resources (OERs) are hard to locate and often lack features like auto-grading or LMS integration, making commercial tools preferable \cite{Fowler2023}. AI tools may produce subtly flawed code, lack analysis features, and become obsolete rapidly \cite{Denny2024}. Teachers also lack time, support materials, and infrastructure for unfamiliar topics \cite{Samarasekara2023}. These tools often perpetuate inequity and require educators to expose sociotechnical biases \cite{Rosenbloom2023}. Interface issues, like confusing diff outputs and inaccessible formats, further hinder learning \cite{Forden2023,Huang2023}.

Debugging remains difficult even when educators spot general faults but not specific bugs \cite{Macann2023}. Primary teachers often lack programming confidence and are unfamiliar with automated tools, which themselves can be limited or confusing \cite{Greifenstein2023}. BVI students struggle with inaccessible IDEs, requiring educators to devote time to navigation rather than content \cite{Huff2021}.

COVID-19 exacerbated these issues. Teachers lacked online-ready content, training, and confidence in using platforms like Zoom \cite{Perlman2021}. Just-in-time support helped, but glitches like faulty breakout rooms persisted \cite{Skuratowicz2021}. Tutors faced difficulties due to restrictions on device use and code access \cite{Markel2021}, while educators continued to experience anxiety with new technologies \cite{Simmonds2021}.






\subsection{Administrative and Institutional Challenges}

Administrative and institutional challenges refer to systemic, policy-driven obstacles rooted in educational structures, leadership, and operational practices that hinder educators', TAs', tutors', and teachers' ability to teach effectively. These include issues such as unclear expectations, lack of infrastructure, rigid curricula, insufficient support for ethics or DEI, inconsistent TA training, faculty shortages, and burdensome workloads.

Teaching-focused roles face unclear duties compared to tenured tracks \cite{Farghally2024}, and integrating industry needs into curricula receives mixed support \cite{Valstar2020}. Teacher shortages persist \cite{Williams2020,Hill2021}, with gaps in preparation infrastructure \cite{Lehtimki2022}. Inflexible course content and redundant efforts challenge CS1 instructors \cite{Vahid2024}. Teachers report vague PD goals \cite{McGill2023} and limited time for ethics, AI, or new CS topics \cite{Hu2023,Greifenstein2023,Lau2023,Grover2024}.

Structural barriers restrict inclusion initiatives \cite{Hwang2023,Rosenbloom2023}, while OER creation lacks incentives \cite{Fowler2023}. Teachers struggle with outdated resources \cite{Huff2021}, complex material dissemination \cite{Izu2025}, and CT curriculum demands \cite{Simmonds2021}. Administrative inefficiencies affect task delegation, PD, and exam logistics \cite{Patel2024,Perlman2021,McGill2024}.

TAs face unclear roles, inconsistent training, and overwhelming responsibilities \cite{Zaman2023,Minnes2022,Riese2022,Akhmetov2024}, often serving as primary student contact without adequate support \cite{Huang2023}. Tutors and TAs are affected by staffing shortages \cite{Sauerwein2023}, mismatched course assignments \cite{Minnes2022}, and lack of coordination systems \cite{Brunelle2022,Malik2024}. Certification policies increase teacher burden \cite{Everson2022}, and teacher colleges lag behind curricular shifts \cite{Simmonds2021}. Schools also face logistical constraints in integrating AI and digital tools into teaching \cite{Kumar2022,Kirk2022}.

Framework fragmentation (e.g., FW/FD split) and standard misalignment further complicate instructional delivery \cite{Repenning2021,Goncharow2021,Ni2021}. Some educators are forced to create their own content (e.g., Scratch) due to lack of institutional prioritization \cite{Jia2022}. Overall, these administrative burdens demand targeted policy, resource allocation, and structural reform to better support teaching roles in CS education.



\subsection{Training \& Professional Development Challenges}
Training and professional development (PD) challenges in computer science (CS) education refer to the barriers educators face in acquiring, accessing, or applying the knowledge, skills, and support systems needed to effectively teach CS. These challenges affect teachers, teaching assistants (TAs), and undergraduate tutors across K–12 and higher education settings.

A foundational challenge is the lack of formal pedagogical preparation for many educators entering CS teaching roles. Several studies highlight that instructors often assume teaching responsibilities without prior training in educational theory, CS pedagogy, or classroom practice, especially undergraduate TAs and novice teachers\cite{Krause-Levy2022,Akhmetov2024}. This gap undermines instructional quality and creates stress among educators unsure of how to effectively engage diverse learners.

The accessibility and structure of professional development programs also pose persistent issues. Research indicates that PD opportunities are either too short-term or narrowly focused on technical content without addressing the complex realities of classroom teaching\cite{Sentance2021}. Teachers express the need for context-sensitive training that equips them with practical strategies, culturally relevant content, and equity-focused pedagogy\cite{Hwang2023,Yadav2022Review}.

Institutional constraints exacerbate these issues. Educators cite lack of time, limited incentives, and absence of institutional support as key barriers to sustained professional development engagement\cite{Thigpen2024}. In under-resourced or rural settings, access to PD programs is further constrained by geographic isolation or funding gaps\cite{Nugent2022,Grover2024}.

Efforts to embed diversity, equity, and inclusion (DEI) principles into PD are also limited. Teachers report receiving little or no training on how to address the needs of students from marginalized or underrepresented communities in CS\cite{Parthasarathy2024,Friend2022}. This results in unintentional biases being reproduced in the classroom and a lack of preparedness to support all students equitably.

Moreover, the one-size-fits-all nature of many PD initiatives fails to recognize the varied roles educators play. For example, undergraduate peer tutors require different forms of mentorship and preparation than in-service high school teachers\cite{Krause-Levy2022}. Without role-specific training models, many educators are left unsupported in their instructional duties.

To address these issues, it is imperative to design sustained, inclusive, and context-aware professional development programs. Empowering educators with pedagogical, technical, and culturally responsive skills will foster more effective and equitable CS learning environments.



\subsection{Socio-cultural Challenges Faced by CS Educators}

Socio-cultural challenges in CS education arise from disparities in cultural norms, identities, and systemic inequities. Educators—particularly women and ethnic minorities—face barriers due to underrepresentation, non-inclusive curricula, and perceptions of CS as exclusive \cite{Hwang2023,Everson2022}. Teachers from marginalized backgrounds often encounter institutional pressures to conform and face resistance to culturally responsive pedagogy \cite{Rosenbloom2023}. Faculty engaged in community work navigate cultural translation and complex stakeholder expectations \cite{Hooshangi2025}.

Instructional materials may unintentionally reinforce stereotypes, and standardized resources often fail to reflect students’ diverse realities \cite{Greifenstein2023,Simmonds2021}. Teachers report insufficient institutional support for DEI efforts, particularly in rural settings \cite{Parthasarathy2024,Yadav2022Review,Nugent2022}. International educators and TAs face linguistic bias, exclusion from informal teaching networks, and difficulty adapting to local classroom cultures \cite{Markel2021,Riese2021,Minnes2022,Krause-Levy2022}.

Educators also express concern over the socio-cultural implications of AI tools, including bias, equity, and pedagogical disempowerment \cite{Lau2023,Sheard2024,Mahon2024}. TAs must manage peer dynamics and ensure inclusive classroom climates during collaboration-heavy activities \cite{Huang2023,Akhmetov2024}. Addressing these challenges requires systemic support for cultural competency training, inclusive content development, and authentic DEI engagement.


\subsection{Parental and Community Involvement Challenges}

Parental and community involvement challenges in CS education refer to the difficulties educators, TAs, and tutors face when engaging families and external stakeholders to support student learning. Limited parental understanding of CS as a career path often results in low student motivation and weak community backing. In New Zealand’s digital technology curriculum, experts stress the importance of outreach to educate parents about the role of CS in future jobs, highlighting the challenge for educators in gaining support for CS initiatives \cite{Samarasekara2023}.

Community-engaged learning, such as service-learning or capstone projects, adds burdens like managing logistics, partner turnover, and repeated onboarding processes, which strain educators' capacity and continuity of efforts \cite{Hooshangi2025}. Pre-service teachers—especially from underrepresented groups—also face identity-based fears of rejection or bias from students and families, affecting confidence and community trust-building \cite{Everson2022}.

These challenges highlight the need for sustained, inclusive engagement strategies between educators, families, and communities to strengthen CS education ecosystems.






\subsection{Sense of Community/Belonging Challenges}

CS educators—including teachers, tutors, and TAs—frequently experience isolation, fragmented collaboration, and cultural misalignment, all of which undermine their sense of belonging and hinder identity development, confidence, and retention \cite{Ni2021,Yadav2022,Nugent2022}. Many serve as the sole CS educator in their institution, limiting peer dialogue and support, while even professional development efforts often fail to cultivate lasting community ties \cite{Skuratowicz2021,Basu2022}.

Educators also face a lack of structured networks for sharing practices, especially in emerging fields like AI \cite{Denny2024,Jetzinger2024,Lee2022}, and instructor collaboration across institutions remains limited but valued when present \cite{Vahid2024,Marshall2020,Kussmaul2022}. TAs frequently work in isolation despite shared roles, facing inconsistent communication and weak team dynamics \cite{Akhmetov2024,Riese2022,Minnes2022,Haglund2024}.

Remote teaching has exacerbated community-building challenges, making co-creation harder and engagement in virtual formats more difficult \cite{Lehtimki2022,Skuratowicz2021}. Cultural pressures persist, with underrepresented educators feeling the need to conform to dominant norms, and pre-service teachers hesitant to enter male-dominated programs due to lack of respect or belonging \cite{Rosenbloom2023,Everson2022}. Broader stereotypes reinforce the perception of CS as unapproachable, especially for women and minorities \cite{Hwang2023}.

Efforts to build shared resources and OER communities are hampered by limited collaboration infrastructure and recognition mechanisms \cite{Fowler2023,Blanchard2022}. In classrooms, miscommunication and group dynamics affect both students’ and TAs’ inclusion experiences \cite{Huang2023,Brunelle2022}. High school teachers, in particular, often lack access to professional learning communities for reflection and growth \cite{Flatland2022,Parthasarathy2024}.



\section{Implemented Remedies}
Several interventions have been implemented to address the multi-faceted challenges faced by CS educators. Instructors have adopted student-centered pedagogical frameworks like Media Computation and contextualized computing to increase engagement and relevance \cite{Venn-Wycherley2020, Lee2021}. Tools such as programming tutors, formative feedback mechanisms, and automatic graders support scalable assessment in large classrooms \cite{Kumar2022, Wang2021}. Blended learning and flipped classroom models have also gained traction, promoting active learning in both in-person and remote settings \cite{Hooshangi2025, Brunelle2022}. 

Efforts to support teacher identity and mental well-being include professional learning communities and targeted TA training programs that address classroom management, inclusivity, and mental health \cite{Minnes2022, Huang2023}. Some institutions provide tailored School Support Visits and regional workshops to boost self-efficacy, especially among novice or retraining teachers \cite{Hill2021, Greifenstein2023}. Accessibility improvements include supporting visually impaired students through tools and platforms with screen reader compatibility and inclusive design principles \cite{Huff2021}. Meanwhile, AI usage is being guided through formative policy creation and dialogue around its responsible integration \cite{Lau2023, Denny2024}. 

Administrative strategies such as TA-Bot reduce coding-related workload \cite{Forden2023}, and shared TA norms aim to streamline instructional consistency across large or distributed courses \cite{Akhmetov2024}. Furthermore, professional development now increasingly includes DEI-aligned practices and culturally responsive pedagogy, albeit with varying degrees of institutional support \cite{Hwang2023, Rosenbloom2023}.

\section{Suggested Remedies}
Despite recent progress, several unmet needs remain. Recommendations include strengthening collaboration across educator networks to combat isolation and promote shared problem-solving \cite{Ni2021, Denny2024}. Structured TA training and workload management tools should be institutionalized to alleviate uneven responsibilities and stress \cite{Zaman2023, Akhmetov2024}. Faculty development must prioritize hands-on CS content training and inclusive pedagogical strategies, especially in underserved regions \cite{Nugent2022, Parthasarathy2024}.

To tackle technical barriers, investment in robust infrastructure, error-transparent tools, and accessible programming environments is essential \cite{Greifenstein2023, Macann2023}. Institutional policies must evolve to support ethics integration, curriculum flexibility, and equitable AI adoption \cite{Hu2023, Grover2024}. Involving educators in shaping these policies ensures their feasibility and relevance \cite{Mahon2024}. 

Finally, promoting parental and community awareness about CS is critical for long-term student motivation and diversity in participation \cite{Samarasekara2023, Everson2022}. Outreach programs and culturally aligned communication strategies can foster inclusive educational ecosystems and sustained community engagement.


\subsection{Sense of Community/Belonging Challenges}
When we talk about an educator's sense of community and belonging, we refer to their feeling of being connected, supported, and valued within their professional environment, whether that's their school, department, or a broader network of peers. This sense of belonging is crucial for professional development, sharing best practices, reducing isolation, and ultimately improving teaching effectiveness and job satisfaction.



\subsubsection*{Isolation and Lack of Peer Connection:}
The majority of computer science teachers are often isolated without other computer science teachers within the same school to share their teaching experiences and practice \cite{Ni2021}. Teachers can lack the opportunities for collegial dialogues and connections, which are an important mechanism that fosters teacher learning and the formation of teacher identity \cite{Ni2021}. They are isolated in their building \cite{Ni2021}. CS teachers often face isolation as they may be the only CS teacher in a school or district \cite{Yadav2022}. This isolation limits their support and the quality of feedback they receive \cite{Yadav2022}. It is harder for them to get quality feedback on their teaching or to benefit from another teacher's experience and ideas \cite{Yadav2022}. Teachers occasionally experience feelings of isolation in their CS teaching roles \cite{Basu2022}. Teachers face challenges related to a lack of opportunities to connect with other high school CS educators and a general absence of a professional learning community for CS teachers \cite{Flatland2022}.

\subsubsection*{Lack of Collaborative and Supportive Environments:}
Early on, few teachers shared their skills and prior knowledge with each other through online communication or peer support \cite{Samarasekara2023}. Achieving cross-curricular integration requires high levels of trust and cooperation between different subject experts, indicating a challenge in fostering strong collaborative professional communities among teachers across disciplines \cite{Samarasekara2023}. While not explicitly listed as a challenge, the paper notes that OER platforms often lack support for community interaction and network building around contributions, which is desired by some contributors as a form of recognition and a way to receive feedback and build reputation. The absence of this feature represents an unmet need that could hinder a sense of belonging or collaborative effort \cite{Fowler2023}. Building community (virtually) in a teacher professional development setting can be challenging even in person \cite{Skuratowicz2021}. The team prioritized efforts like shared physical experiences (e.g., "party pack" items) to foster this sense of community. Isolation within the group: While not explicitly stated as a challenge faced by teachers within the training program itself, the paper notes that community building can help raise teacher confidence and mitigate feelings of isolation within a group, implying that a lack of this sense of community could be a challenge \cite{Simmonds2021}. TAs have been found to work independently despite being tasked with the same duty, even though working collaboratively has been shown to be very successful \cite{Riese2022}. There is a recognized need to create a stronger TA community where ideas can be shared more easily, implying this is currently a challenge \cite{Riese2022}. While the project aimed to address the lack of a strong community, the absence of a supportive peer group or mentor could be considered a significant challenge for faculty trying to adopt POGIL independently. Instructors highly valued the "vital supportive community" provided by their teams and mentors, which helped them "not feel alone" and gain confidence. This implies that without such a community, the challenge of isolation and lack of support would be pronounced \cite{Kussmaul2022}. Although TAs recognize the benefits of collaboration (e.g., assessing work together for improved speed and consistency), some do not have sufficient opportunities to engage in supportive and collaborative environments where they can exchange teaching methodologies and refine their practices. This absence impacts their confidence and sense of belonging within the teaching staff \cite{Haglund2024}.

\subsubsection*{Challenges in Collaborative Processes and Communication:}
Personal networking among teachers in the sense of a community of practice is particularly important for this new topic (AI Teaching Assistants) \cite{Denny2024}. Challenges with remote collaboration for co-creation: For teachers involved in co-creating lesson plans, it was sometimes "challenging at times to know what would work best for some of the lesson plans especially when everyone wasn't there to discuss things in person" \cite{Lehtimki2022}. This highlights a difficulty in the collaborative process when face-to-face interaction was absent. TAs feeling less updated and involved in the CS2 course compared to CS1 \cite{Akhmetov2024}. Communication between instructors and TAs in CS2 wasn't as good, which sometimes left students uninformed. Some TAs also mentioned that they felt less updated and involved in CS2 compared to CS1, particularly praising the "level of organization and professionalism" of their CS1 experience. Maintaining instructor-student interaction: The asynchronous instruction and cohort structure led to less frequent direct student-instructor interaction and denied normal opportunities for casual interaction, a disconnect that both instructors and students lamented \cite{Brunelle2022}. The challenge of forming and maintaining a community of teachers interested in AI education remotely, particularly during the COVID-19 pandemic \cite{Lee2022}.

\subsubsection*{Inclusivity and Identity-Related Challenges:}
Perception of CS as a 'niche' subject: The low participation rates among women and ethnic minorities contribute to CS being viewed as a 'niche' subject that serves a smaller, more homogeneous group of students, potentially alienating others and hindering their sense of belonging \cite{Hwang2023}. Perception of CS as inaccessible: The impression held by both students and teachers that CS is inaccessible to them can create barriers to engagement and a sense of belonging within the subject \cite{Hwang2023}. Difficulty building deep relationships: Structural barriers like timetabling constraints make it challenging for teachers to build deep, long-term relationships and rapport with their students, which is crucial for fostering a sense of community and belonging in the classroom \cite{Hwang2023}. Stigma around AI use: Students may feel it's a "taboo topic" or akin to "cheating services" to use AI tools, leading to fear of being seen with them open, which could hinder open discussion or collaborative learning around these tools \cite{Lau2023}. The pressure on newly-recruited students and faculty to "assimilate into White supremacist, techno-colonial ways of knowing and being" and to "make white people comfortable" or "sell out" to succeed implies a significant challenge to fostering a genuine sense of belonging for those who resist these norms. This makes it difficult to build the "rebellious communities" that are described as a "refuge" for abolitionist teachers \cite{Rosenbloom2023}. A sense of not belonging or being respected in CS communities \cite{Everson2022}. Some candidates would not have joined the program if it was "taught by a bunch of dudes", highlighting the importance of supportive and inclusive instructor identities. The collaborative mindset of some candidates who declined to enroll to reserve limited funding for peers who they believed would benefit more immediately \cite{Everson2022}. Maintaining an inclusive and supportive classroom environment: Student achievement is directly correlated to a positive classroom climate, implying that TAs must possess skills to maintain an inclusive, welcoming, and supportive environment \cite{Huang2023}. The paper posits there is "no meaningful separation between pedagogical and climate skills," suggesting that separating these aspects in practice presents a challenge. Inadvertently discouraging student participation: Specific phrasing can make a student feel they "don't belong" \cite{Huang2023}. Managing sensitive group formation and dynamics: Ensuring students feel "safe and productive" when forming groups \cite{Huang2023}.

\subsubsection*{Lack of Common Understanding and Systemic Support:}
Lack of Common Understanding within Teaching Communities: It is crucial for teachers within their local teaching communities (e.g., school, peer groups) to establish a common understanding of commonly used jargon or acronyms to prevent internal misunderstandings and ensure consistency in teaching \cite{Munasinghe2021}. While the program itself aims to build a sense of community among faculty through collaborative engagements, the initial challenges highlighted in the paper do not explicitly list a lack of community among faculty as a pre-existing problem for them. Instead, the program offers a solution to this potential isolation \cite{Marshall2020}. While the paper recommends developing a community of practitioners for CS faculty interested in accessibility to learn from each other and get support, the absence of such a community is presented more as a systemic gap rather than a direct challenge impacting individual teachers' sense of belonging or isolation \cite{Parthasarathy2024}. The absence of a central, moderated tool repository and the lack of requirements for archival links in publications hinder the ability of the community to collectively access, maintain, and build upon shared tools, thus undermining a strong sense of collective ownership and effort \cite{Blanchard2022}. The risk of tools losing stewardship or supporting infrastructure highlights a gap in sustained community support mechanisms for adopted software \cite{Blanchard2022}.

\subsubsection*{Internal Team Dynamics:}
Discovering unethical behavior of other TAs, which despite the TA community being a support network, posed a challenge \cite{Riese2021}. While the course aimed to build community, the need for practicum groups to be "safe spaces" to troubleshoot inter-TA challenges indicates that maintaining positive team dynamics and a sense of belonging within TA teams can be a challenge \cite{Minnes2022}.



\subsection{Classroom Management Challenges}

Classroom management challenges are related to the effective organization and control of the learning environment. This includes managing teaching assistants and scaling courses effectively, as highlighted by experiences in managing a large number of teaching assistants in a CS1 course.

Teachers face numerous pedagogical and logistical challenges in managing their classrooms effectively. These include the need to routinely reflect on their practices, unique classroom contexts, and how their practices meet student needs \cite{Thigpen2024}. Differentiating between and engaging students, along with addressing student resilience issues such as ensuring equal participation and inclusion, and fostering collaboration, are crucial \cite{Musaeus2024}. Furthermore, students' motivation can be affected by a lack of communication skills, confidence, and social anxiety \cite{Farghally2024}. Large class sizes make it harder for instructors to simultaneously pay attention to both course structure and content \cite{Valstar2020,Goncharow2021}, and students often struggle with understanding concepts and technical problems \cite{Pieper2020}. There is also a recognized need to strengthen efforts to educate teachers in addressing programming errors \cite{Pieper2020}.

Student engagement is a persistent challenge, with pupils often lacking interest in computing and prioritizing other subjects, suggesting a perceived lack of applicability to their own interests \cite{Venn-Wycherley2020}. Moreover, students may not be prepared to independently solve programming problems and tend to give up quickly when faced with challenges, which is attributed to a lack of understanding and confidence \cite{Venn-Wycherley2020}. The traditional, manual assessment methods are often insufficient for providing timely feedback to all students in growing CS classrooms \cite{Wang2021}. Limited lecture time necessitates extensive activities outside of lecture for learning CS1 \cite{Vahid2024}. The increasing use of AI tools introduces new challenges, such as a lack of visibility into student AI usage due to student reluctance to disclose it \cite{Lau2023}, and a "taboo topic" sentiment that leads to hidden usage \cite{Lau2023}.

Indirect impacts from a lack of preparation time and insufficient resources further complicate the effective management of learning activities \cite{Samarasekara2023}. Increasing class sizes and stagnant instructor numbers decrease the time available for individual student help \cite{Forden2023}. Managing student procrastination, which leads to cooldown periods near deadlines and manual submission uploads, is another significant hurdle \cite{Forden2023}. Teaching assistants (TAs) frequently encounter difficulties, including not responding to students in time and finding it hard to give individual attention due to larger course sizes \cite{Zaman2023}. TAs often serve as the primary student contact in large courses for both course material and classroom climate issues \cite{Huang2023}, and they are tasked with combating harassment, retaliation, and discrimination among students in group settings \cite{Huang2023}, as well as ensuring psychological safety in teams \cite{Huang2023}. Managing group dynamics for fair participation and preventing unequal contributions in group projects are also critical responsibilities \cite{Lee2021}.

The shift to online learning introduced its own set of challenges, such as difficulty managing online lessons using Zoom, a hurdle some teachers have yet to overcome \cite{Perlman2021}. Tutors frequently spend long periods with unprepared students while "ready" students wait in help queues \cite{Markel2021}. Encouraging students to seek help at an "optimal" time and prioritizing those who have invested significant effort are ongoing concerns \cite{Markel2021}. The surge in unpermitted assignment and exam aid on public online platforms also presents a management challenge \cite{Rusak2021}. Educators must also handle the vast diversity of students, including those with special needs, personal problems, unhappiness with assessment, and difficulties with group work \cite{Riese2021}. Dealing with varying levels of content knowledge among students and meeting the needs of unmotivated, passive, and unprepared students, or those who did not want help or were only focused on end results, are common occurrences \cite{Riese2021}. Handling arising conflicts is also part of daily classroom management \cite{Riese2021}. In-class time constraints make it difficult to divide time evenly, prioritize students, assess effectively, and give adequate attention to advanced students \cite{Riese2021}.

Typical classroom management issues can hamper tutors' pedagogical confidence and their ability to adapt instructional experiments \cite{Goletti2021}. Tutors may adapt strategies orally rather than explicitly, potentially impacting the explicit nature of instruction \cite{Goletti2021}. Student talk can be a potential distraction for those who prefer to "tinker with the code" to investigate it, highlighting a need to manage different learning styles \cite{Sentance2021}, and keeping students focused during unguided talk is also a challenge \cite{Sentance2021}. In group projects, students may lack motivation and effort, leading to unequal contributions \cite{Hooshangi2025}, and managing conflict among students in teams is essential \cite{Hooshangi2025}. Instructors managing software engineering capstone courses face the challenge of managing teams of students \cite{Hooshangi2025} and anticipating a different interaction style with students compared to typical lecture-based courses \cite{Hooshangi2025}. Scaling software engineering capstone projects to increasingly large class sizes is also a significant management issue \cite{Hooshangi2025}.

Student displeasure or perception of extra work, such as associating specific tools like GenderMag with additional burdens, can also be a challenge \cite{Patel2024}. Managing large class sizes in primary and secondary schools requires consistent classroom management strategies \cite{Jia2022}. Troubleshooting inter-TA challenges that sometimes occur within TA teams can impact coordinated course management \cite{Minnes2022}. Fragmented information sharing among a large team of TAs \cite{Akhmetov2024} and a poor understanding of course activities among a large, horizontally structured TA team \cite{Akhmetov2024} contribute to management difficulties. The high volume of students' questions in a large course poses a significant challenge \cite{Akhmetov2024}. Some under-performing students may not want help or respond to outreach efforts \cite{Akhmetov2024}, and unbalanced workloads within TA support teams are common \cite{Akhmetov2024}. Last-minute swap requests or cancellations by TAs \cite{Akhmetov2024}, limitations in monitoring TA attendance \cite{Akhmetov2024}, and TAs being unaware of their schedules leading to absences \cite{Akhmetov2024} further complicate management. The "week expert" system for communication support can lead to a higher workload and mental strain \cite{Akhmetov2024}.

Finally, managing the heavy grading load resulting from assigning the amount of practice students truly need is a considerable challenge \cite{Kumar2022}. TAs also face time management challenges \cite{Riese2022}. Managing traditional office hours, including "pre-grading" requests and lengthy queues, can be difficult \cite{Brunelle2022}, as are logistical challenges for in-person adaptation of meetings \cite{Brunelle2022}. Coordination with rolling schedules means instructors cannot fairly issue corrections or host course-wide events \cite{Brunelle2022}. Inconsistencies from varying instructional guidance for final projects make standardization difficult \cite{Kao2020}. The time required to complete in-class activities often consumes significant class time \cite{Kussmaul2022}. Dealing with varying student team completion times, which sometimes disadvantages slower teams \cite{Kussmaul2022}, and managing student pushback or resistance regarding teamwork and roles \cite{Kussmaul2022} are also management concerns. Lastly, managing numerous students with heterogeneous Unix backgrounds presents a unique challenge . Instructors also find it difficult when students are unwilling to ask for help, hindering effective classroom support and remediation efforts \cite{Krause-Levy2023}.



===================================================================================================================================================

% \subsubsection*{Pedagogical Challenges}

% Several peer-reviewed studies have highlighted that many CS educators lack the pedagogical content knowledge (PCK) necessary to effectively teach computer science concepts. Teachers are encouraged to regularly reflect on their instructional practices, classroom contexts, and how their teaching meets student needs \cite{Thigpen2024}. Moreover, evolving standards in CS education often create confusion about what should be taught and how, leaving teachers uncertain about their qualifications or how to become certified as CS educators. This uncertainty can disrupt their professional identity. In particular, asking teachers to start teaching a CS course or to integrate computer science or computational thinking into existing subjects may fragment their sense of professional identity. \cite{McGill2024}.







% \subsubsection*{Assessment and Evaluation Challenges}
% \subsubsection*{Classroom Management Challenges}
% \subsubsection*{Emotional and Psychological Challenges}
% \subsubsection*{Technological Challenges}
% \subsubsection*{Administrative and Institutional Challenges}



% \textbf{List of Pedagogical Challenges}

% Teachers often lack the necessary pedagogical content knowledge to teach CS effectively. They must continuously reflect on their practices, adapt to classroom contexts, and ensure their methods meet students’ needs \cite{Thigpen2024}. A related concern involves students' difficulties in transferring knowledge between sessions or among peers during group work, which complicates collaborative learning and long-term comprehension \cite{Musaeus2024}.

% There are persistent gaps in the preparation of both instructors and teaching assistants (TAs), impacting their ability to motivate students. This includes issues like poor instructor communication, unclear objectives, procrastination, lack of confidence, and social anxiety \cite{Farghally2024}. Educators also find it difficult to obtain clear, consistent guidance on teaching style—often encountering language-specific or conflicting advice that leaves the definition of “good style” ambiguous \cite{Kirk2024}.

% Integrating industry-relevant practices into the classroom remains a challenge, with significant variation depending on the course content. Faculty in algorithms, for instance, are more hesitant to adopt such integration compared to software-focused educators \cite{Valstar2020}. Furthermore, there is a general shortage of qualified CS teachers \cite{Williams2020}, and developing pedagogical knowledge continues to be a systemic issue \cite{Pieper2020}.

% In many classrooms, student enthusiasm diminishes when teaching practices or infrastructure are ineffective \cite{Venn-Wycherley2020}, and students often lack the resilience needed to persist through challenges \cite{Venn-Wycherley2020}. Many instructors lack formal pedagogical training and are unaware of evidence-based strategies for course design \cite{Goncharow2021}, and students often fail to transfer concepts from one programming language to another \cite{Tshukudu2021}.

% As standards evolve, teachers struggle to define the academic core of CS and align it with effective teaching practices \cite{Ni2021}. The heavy focus on technical content can also distract instructors from addressing pedagogical and student support issues \cite{Vahid2024}. A lack of qualification among teachers remains a concern, and professional development must expand their overall competence \cite{Denny2024}.

% Aligning lesson plans with frameworks like the CSTA Standards is difficult, particularly for new or integrated CS teachers \cite{McGill2023}. Translating culturally responsive and relevant pedagogies into diverse educational settings is also a challenge \cite{Hwang2023}, as is embedding cultural elements into CS content and encouraging student-led learning \cite{Hwang2023}. Many students perceive CS as inaccessible, while curriculum constraints prevent teachers from fully implementing the intended programs \cite{Hwang2023}. Integrating social justice content further complicates lesson planning \cite{Hwang2023}.

% Open Educational Resources (OERs) pose multiple challenges: ensuring broad content coverage (especially for specialized areas), maintaining high quality, customizing for specific curriculum needs, and keeping content up to date in a rapidly evolving field \cite{Fowler2023}. Meanwhile, students increasingly rely on AI tools, but this can hinder foundational learning if the generated code is flawed or stylistically weak \cite{Lau2023}. Moreover, effective AI usage requires prompt-crafting expertise, adding another layer of complexity for both students and instructors \cite{Lau2023}. CS1/CS2 courses often overemphasize syntax and rote mechanics, limiting deeper conceptual learning \cite{Lau2023}.

% The inherent complexity of CS topics makes authentic, project-based learning difficult for all students \cite{Samarasekara2023}. There is resistance to adopting centralized textbooks, and educators struggle to integrate digital technologies across subjects \cite{Samarasekara2023}. Similarly, incorporating abolitionist educational principles into CS is met with skepticism \cite{Rosenbloom2023}, alongside a broader issue of techno-nihilism and reduced pedagogical imagination among teachers \cite{Rosenbloom2023}.

% Feedback systems present another cluster of challenges. Legacy platforms often deliver ineffective feedback and confuse students with automated responses \cite{Forden2023}. The complexity and relevance of gamification tools in CS1 courses are also debated \cite{Forden2023}. TAs commonly lack deep content knowledge and are underused for more pedagogically demanding tasks, often struggling to provide meaningful grading feedback \cite{Zaman2023}.

% Instructors must also cope with students entering courses with widely varying prerequisite knowledge \cite{Sauerwein2023}. This makes managing evolving learning goals and selecting appropriate tasks even more difficult \cite{Sauerwein2023}. Debugging, a critical programming skill, poses persistent problems: students misinterpret error messages or seek help prematurely, while teachers themselves may rely on informal or self-taught methods for providing debugging support \cite{Macann2023}.

% Educators frequently underestimate the value of clearly defined learning objectives when designing instructional tasks \cite{Saqr2024}. Creating exemplary code and assignments remains a pedagogical hurdle \cite{Saqr2024}. Many lack feedback mechanisms for improving their materials and rely on system-generated log data that lacks clear pedagogical insights \cite{Singh2020}. Additionally, students working in isolation are often under-supported, exacerbating disengagement and learning difficulties \cite{Singh2020}.



% \subsubsection{Classroom Management Challenges}

% Classroom management challenges in Computer Science (CS) education refer to the organization and oversight of learning environments, particularly in large and diverse classrooms. These include managing teaching assistants (TAs), addressing student behavior, coordinating instruction, and fostering inclusive and productive student interactions .

% Teachers must regularly reflect on their instructional practices and classroom contexts to address student needs effectively \cite{Thigpen2024}. A central concern is engaging diverse learners and promoting student resilience, participation, and collaboration \cite{Musaeus2024}. Challenges such as lack of student communication skills, confidence, and social anxiety further affect motivation \cite{Farghally2024}. Managing large class sizes often overwhelms instructors, making it difficult to balance attention between course structure and content \citation{Valstar2020,Goncharow2021}.

% Students often struggle with understanding content and face technical difficulties \cite{Pieper2020}. Teachers need more training to address common programming errors \cite{Pieper2020}. Additionally, students sometimes lack interest in computing, viewing it as irrelevant to their lives, and prioritize other subjects instead \cite{Venn-Wycherley2020}. Many are also unprepared to independently solve problems and may give up quickly when faced with difficulties \cite{Venn-Wycherley2020}.

% Manual assessment is insufficient in growing classrooms, leading to delays in feedback \cite{Wang2021}. Limited lecture time necessitates additional learning outside of class, particularly in CS1 courses \cite{Vahid2024}. Meanwhile, there is a lack of visibility into students' AI tool usage due to reluctance to disclose such practices \cite{Lau2023}, and the topic often carries a taboo, which hides important learning behaviors \cite{Lau2023}.

% Time and resource constraints hinder effective learning activity management \cite{Samarasekara2023}. Increasing class sizes without proportional increases in faculty reduce opportunities for individual student support \cite{Forden2023}. Procrastination leads to bottlenecks before deadlines, resulting in manual uploads and cooldown periods \cite{Forden2023}. TAs may not respond promptly or provide individual attention, especially in large courses \cite{Zaman2023}.

% In large classes, TAs often become the primary point of contact for content-related and interpersonal issues, including managing harassment, discrimination, and psychological safety \cite{Huang2023}. Group projects pose further challenges such as ensuring equitable participation and mitigating conflict \cite{Lee2021}. Online teaching adds complexity, with some educators still struggling with platforms like Zoom \cite{Perlman2021}.

% Tutors often spend too much time helping unprepared students while better-prepared students wait in long queues \cite{Markel2021}. Encouraging students to seek help at appropriate times is difficult \cite{Markel2021}. There is also concern about unpermitted help from public platforms during exams or assignments \cite{Rusak2021}. The increasing diversity of student backgrounds adds to classroom complexity, from special needs and content knowledge variability to personal issues \cite{Riese2021}.

% Unmotivated and passive students who are solely outcome-focused pose a motivational barrier \cite{Riese2021}. Teachers must also manage conflicts, optimize in-class time, and prioritize students effectively \cite{Riese2021}. Common classroom management issues hinder tutors’ pedagogical confidence and experimentation with new teaching strategies \cite{Goletti2021}, while oral adaptation of strategies may lack clarity and consistency \cite{Goletti2021}.

% Different learning styles require varied approaches; for instance, some students prefer exploration over discussion, which may become distracting \cite{Sentance2021}. Keeping students engaged during unguided talk is also challenging \cite{Sentance2021}. Group work further suffers when students lack effort or motivation or when they contribute unequally \cite{Hooshangi2025}. Conflicts in teams, especially in software engineering capstone courses, require careful management \cite{Hooshangi2025}.

% Instructors in capstone courses must adjust their interaction styles and find ways to scale projects for large class sizes \cite{Hooshangi2025}. Students may view inclusive tools like GenderMag as unnecessary extra work \cite{Patel2024}. Consistent strategies are required to manage large class sizes, particularly in K–12 settings \cite{Jia2022}. Internal TA issues—such as coordination challenges and communication gaps—further complicate classroom management \cite{Minnes2022,Akhmetov2024}.

% Many TAs lack a comprehensive understanding of course activities or awareness of their own schedules, resulting in missed sessions and poor attendance tracking \cite{Akhmetov2024}. TA workload is often unbalanced, and last-minute cancellations are frequent \cite{Akhmetov2024}. The “week expert” system for TA communication increases stress levels and responsibility burdens \cite{Akhmetov2024}.

% Heavy grading loads in large classes challenge instructors who want to assign adequate practice \cite{Kumar2022}. TA time management is strained under such pressure \cite{Riese2022}. Traditional office hours are inefficient, often involving lengthy queues and early grading requests \cite{Brunelle2022}. Logistical issues further complicate in-person sessions and scheduling, limiting fairness and coordination \cite{Brunelle2022}.

% Inconsistent instructional guidance during final projects creates difficulties in standardizing course delivery \cite{Kao2020}. In-class activities may consume too much time, and uneven group performance can disadvantage slower teams \cite{Kussmaul2022}. Resistance to group work and role assignments also requires careful handling \cite{Kussmaul2022}. Finally, managing students with differing Unix proficiency levels remains an ongoing concern 





% \subsubsection{Emotional and Psychological Challenges}
% Emotional and psychological challenges faced by educators encompass a range of difficulties that impact their mental well-being, professional efficacy, and job satisfaction. These challenges often stem from the demanding nature of the teaching profession, including managing student behavior, adapting to new curricula and technologies, dealing with administrative pressures, and navigating complex social dynamics within educational institutions. Such challenges can manifest as stress, anxiety, diminished self-esteem, isolation, and burnout, ultimately affecting their ability to effectively teach and support students.

% As teachers grow in their knowledge, they become more aware of their own progress, which can help identify future growth areas \cite{Thigpen2024}. However, many faculty members believe teaching ability is innate, leading to a lack of motivation among graduate students to enhance their teaching skills \cite{Farghally2024}. Self-esteem plays a pivotal role; female teachers, primary educators, and those with less experience or from rural regions reported significantly lower self-esteem in teaching computer science (CS) \cite{Vivian2020}. This low confidence can lead to challenges in delivering effective instruction, especially when students enter secondary school enthusiastic about CS but quickly lose interest without supportive teaching \cite{VennWycherley2020}.

% Despite existing national curriculum standards, educators often rely on intuition or recreate resources unnecessarily \cite{Goncharow2021}. Students may be discouraged or lack confidence when learning programming languages, and teachers must navigate their own fragmented identities when taking on unfamiliar content areas like CS \cite{Tshukudu2021,Ni2021}. This identity conflict is exacerbated when teachers feel they are merely surviving in a system that offers little support or flexibility \cite{Vahid2024}. Building self-efficacy requires room for exploration and adaptation \cite{Denny2024}.

% Teachers experience cognitive overload due to unclear expectations and excessive information \cite{Hwang2023}, with the process often described as overwhelming. Variability in culturally responsive teaching (CRT) conceptualizations, unconscious biases, and reluctance to address racial inequity further strain teachers emotionally \cite{Hwang2023}. Some fear reputational damage from public educational materials, and the lack of recognition for their efforts can be demotivating \cite{Fowler2023}. Additionally, high-stakes exams and rote mechanics of coding alienate students and pose challenges for educators attempting to sustain engagement \cite{Lau2023}.

% Heavy workloads, insufficient staffing, and limited resources create further pressure \cite{Samarasekara2023}. Educators also face institutional resistance when challenging systemic oppression, sometimes risking job loss or emotional exhaustion due to lack of support \cite{Rosenbloom2023}. Teaching tools like time-based scoring can be misunderstood by students, leading to morale issues and complaints \cite{Forden2023}, while automated feedback systems often overwhelm rather than aid learning \cite{Forden2023}. Emotional unpreparedness is common among TAs dealing with climate-related issues, harassment, or gender discrimination \cite{Huang2023}.

% Students’ low error tolerance frustrates educators during programming tasks, contributing to a lack of confidence and difficulty engaging in debugging processes \cite{Macann2023}. Teachers unfamiliar with CS often feel insecure about creating instructional tasks and report low confidence due to limited subject knowledge \cite{Greifenstein2023}. Teachers new to CS instruction particularly struggle with confidence and rely on support like School Support Visits to improve their self-efficacy \cite{Hill2021}.

% Inaccessibility of tools and materials can cause BVI students to fall behind, which deeply concerns educators, leading to fears about student progress and lowered self-confidence among learners \cite{Huff2021}. Some pre-service teachers question the relevance of CS to their future classrooms, creating an emotional barrier to engaging with the subject \cite{Repenning2021}. Breaks in instruction can further diminish student enthusiasm and self-belief \cite{Repenning2021}.

% A compassionate approach to students' learning difficulties is essential; educators must support learners empathetically and foster environments that tolerate mistakes as part of the learning process \cite{Lee2021}. The sudden shift to online teaching during the pandemic caused high stress, especially with looming matriculation exams, and raised concerns among new teachers about job security \cite{Perlman2021}. Many also experienced pre-existing anxiety about teaching mathematics and science, which was intensified by new requirements like computational thinking and unfamiliar virtual platforms \cite{Skuratowicz2021}.

% Both tutors and students face emotional regulation challenges. Tutors must remain calm while managing their own academic stress and offering emotional reassurance to anxious or insecure students \cite{Markel2021}. Teachers’ preconceived notions about computing, their anxiety about mastering new platforms, and broader fears about technology can hinder effective teaching \cite{Simmonds2021}. Interpersonal discomfort during emotional student interactions or difficult ethical decisions also strains educators \cite{Riese2021}. This includes discomfort with announcing failure, navigating complicated relationships, or setting appropriate boundaries \cite{Riese2021}.

% Classroom management struggles and insufficient pedagogical training can reduce tutors’ confidence, particularly when they don't see the value of proposed instructional strategies \cite{Goletti2021}. Some worry that these strategies might reduce student independence or feel lost without hands-on support \cite{Goletti2021}. A notable challenge is the misalignment between educators’ self-perception and actual programming skills, which leads to resistance to further training \cite{Kumar2021}. This overconfidence is compounded by pandemic-related stress, which affected participation in professional development \cite{Kumar2021}.

% Finally, teachers unfamiliar with computing often feel overwhelmed by technical jargon and hesitate to engage with the subject at all \cite{Munasinghe2021}. These emotional and psychological burdens underscore the need for better institutional support, mental health resources, and professional development tailored to the realities of teaching today.





% \subsubsection{Technological Challenges Faced by Educators}
% The peer paper's review outlines the significant technological challenges encountered by educators, drawing insights from recent academic literature. These challenges include difficulties in integrating new tools, a lack of resources, and issues with technical support and infrastructure, all of which impact teaching effectiveness.

% Educators today navigate a complex landscape fraught with various technological challenges. These issues can impede effective instruction, reduce job satisfaction, and hinder professional growth. Understanding and addressing these challenges is crucial for fostering a supportive educational environment and enhancing teaching quality.

% Technological challenges for educators involve difficulties in integrating new tools into the classroom, a lack of resources, and issues with technical support and infrastructure. A significant number of teachers who had not taught Computer Science (CS) previously found it challenging as it was their first opportunity to learn about teaching CS. They performed best in analyzing impacts of computing and modeling networks, but struggled with using and analyzing data, and developing programs and interpreting algorithms \cite{Thigpen2024}. Teachers identified technical problems and a lack of resources as significant challenges, particularly among primary education teachers. Researchers also noted practical issues with computational tools, though teachers did not always identify these as challenges themselves \cite{Musaeus2024}. A lack of qualified teaching faculty applicants contributes to staffing challenges in CS education \cite{Farghally2024}, and many faculty lack knowledge of current industry practices and resources, hindering their ability to integrate relevant material like software engineering best practices and soft skills into courses \cite{Valstar2020}. Some faculty teaching algorithms were split on the appropriateness of industry preparation in their course, while those teaching software construction courses rated industry preparation more highly \cite{Valstar2020}. They also cited topics like software maintenance as being difficult to teach and “soft” skills as under-taught \cite{Valstar2020}. Many felt under-resourced to improve course quality in these areas \cite{Valstar2020}. The majority believe that curricula should be improved with respect to industry preparation, although a sizeable portion of Programming Languages faculty disagreed on including such content \cite{Valstar2020}.

% Teachers initially struggle with teaching CS due to limited content knowledge \cite{Vivian2020}. Many re-trained teachers considered their incomplete understanding of the subject matter to be a hindrance \cite{Pieper2020}, and frequently cited issues with differentiation, students not understanding the material, and technical problems \cite{Pieper2020}. There is a clear need to better educate teachers in addressing programming errors \cite{Pieper2020}. Students may quickly lose interest in CS in the absence of supportive infrastructure and effective teaching \cite{VennWycherley2020}. Despite the availability of national curriculum standards, administrators and instructors often reinvent the wheel or rely heavily on intuition \cite{Goncharow2021}. Assessing visual and interactive programs poses technical challenges \cite{Wang2021}, and transitioning from Scratch to Python proves difficult \cite{Tshukudu2021}. Technical issues persist with tools, especially those aimed at classroom integration \cite{Tshukudu2021}. Teachers reported problems with digital submission forms, such as nonfunctional save features, upload issues, and broken links, as well as limited storage for artifacts \cite{McGill2023}.

% Locating relevant, high-quality Open Educational Resources (OERs) is time-consuming due to inadequate search and filter capabilities \cite{Fowler2023}. OERs also lack features like auto-grading, interactive content, and LMS integration, making commercial products more attractive \cite{Fowler2023}. AI tools can generate subtly incorrect code, lack robustness, and may be outdated or nondeterministic in their responses \cite{Denny2024}. These tools also do not perform static or runtime analysis, limiting their debugging value \cite{Denny2024}. Assignments designed to be "AI-proof" may become ineffective as AI capabilities evolve \cite{Denny2024}.

% Teachers cite a lack of time and resources to prepare and teach unfamiliar topics \cite{Samarasekara2023}, and report dissatisfaction with available support materials and exemplars \cite{Samarasekara2023}. There is a shortage of free, approved instructional resources \cite{Samarasekara2023}, exacerbated by limited infrastructure and inadequate hosting platforms \cite{Samarasekara2023}. The problem lies less in the inherent difficulty of technology than in how it is designed and used, often reinforcing systemic inequalities \cite{Rosenbloom2023}. Teachers must reveal the sociotechnical codes embedded in CS and guide students to understand its societal impact \cite{Rosenbloom2023}. For example, Linux diff outputs confuse students during testing, highlighting poor interface design \cite{Forden2023}. Web-based materials are preferred for accessibility over scanned documents \cite{Huang2023}, and debugging remains a challenge even when teachers can identify broad issues but not specific bugs \cite{Macann2023}.

% Primary school teachers often lack programming knowledge, making it hard to write example code or teach efficient programming practices \cite{Greifenstein2023}. Many are unaware of useful automated analysis tools or find them limited—unable to analyze semantics, prone to false positives, lacking auto-refactoring, or offering incomprehensible hints \cite{Greifenstein2023}. Accessibility is another concern; blind and visually impaired (BVI) students face barriers due to inaccessible development environments \cite{Huff2021}. Teachers spend as much time teaching IDE navigation as they do teaching programming content, while screen readers inconsistently recognize interface elements \cite{Huff2021}.

% The COVID-19 pandemic amplified these challenges. Teachers lacked Zoom-ready materials and the time to create them \cite{Perlman2021}, were unfamiliar with online platforms, and feared they could not navigate virtual systems \cite{Perlman2021}. Just-in-time training helped reduce such anxieties \cite{Perlman2021}, although technical glitches like incorrect breakout room assignments still disrupted activities \cite{Skuratowicz2021}. In tutoring contexts, the inability to use personal laptops or access student code complicates support efforts \cite{Markel2021}, while many educators report ongoing anxiety with mastering new platforms \cite{Simmonds2021}.

% The technological challenges faced by educators are significant and varied, ranging from insufficient resources and technical support to the complexities of integrating advanced tools like AI. Addressing these issues requires comprehensive strategies that provide adequate training, resources, and infrastructure to empower educators in a rapidly evolving digital landscape. By mitigating these challenges, we can foster a more effective and sustainable educational environment for all.





% \subsubsection{Administrative and Institutional Challenges}
% Administrative and institutional challenges faced by educators refer to systemic obstacles and policy-related issues originating from the organizational structure, leadership, and operational frameworks of educational institutions and broader educational systems. These challenges often involve, but are not limited to, funding, resource allocation, curriculum mandates, professional development, workload management, recruitment and retention policies, and administrative processes that directly impact educators' ability to perform their duties effectively, innovate, and contribute to student success. They encompass difficulties arising from organizational policies, lack of support, and the broader educational context rather than individual teaching competence or classroom-level pedagogical issues.

% \textbf{Administrative and Institutional Challenges Faced by Educators}



%   The differences in responsibilities, education, and employment conditions between teaching-focused faculty positions and traditional tenured/tenure-track positions are not well understood \cite{Farghally2024}.
%   Faculty face conflicting views about integrating industry preparation into curricula, with variable support across course areas \cite{Valstar2020}.
%   There is a shortage of teachers qualified to teach teaching \cite{Williams2020}.
%   Lack of supportive infrastructure can diminish student enthusiasm in CS despite initial interest \cite{Venn-Wycherley2020}.
%   Administrators and instructors often rely on intuition or duplicate efforts despite national standards \cite{Goncharow2021}.
%   CS education standards lack maturity and consistent certification requirements \cite{Ni2021}.
%   Instructors are restricted in modifying CS1 course content or programming language; redundant preparation efforts persist \cite{Vahid2024}.
%   Teachers report unclear expectations and administrative inefficiencies during professional development initiatives \cite{McGill2023}.
%   Diversity and inclusion mandates are poorly implemented due to structural curriculum and timetable constraints \cite{Hwang2023}.
%   Faculty lack institutional incentives or recognition for creating and sharing OERs \cite{Fowler2023}.
%   Institutions are struggling to develop timely and ethical AI integration policies, including curriculum updates \cite{Lau2023}.
%   Teachers face equity gaps and low uptake in Digital Technology participation, with limited resources and staffing \cite{Samarasekara2023}.
%   Institutional pressure to uphold "rigorous" curricula can undermine transformative teaching goals \cite{Rosenbloom2023}.
%   Administrative overhead for tasks like code testing is alleviated by automation tools like TA-Bot \cite{Forden2023}.
%   Inconsistent TA training practices and overwhelming workloads impact instructional quality \cite{Zaman2023}.
%   Tutor shortages and growing class sizes stress instructional support systems \cite{Sauerwein2023}.
%   Teachers report no time to integrate ethics due to overburdened CS curricula and lack of prioritization \cite{Hu2023}.
%   TAs often bear primary student-facing responsibilities without adequate training consistency \cite{Huang2023}.
%   Teachers face inadequate time and planning resources for implementing new CS topics \cite{Greifenstein2023}.
%   There is a significant national shortage of CS teachers and insufficient infrastructure to prepare them \cite{Hill2021}.
%   Many teachers lack basic teaching equipment and up-to-date resources \cite{Huff2021}.
%   Frameworks like FW/FD split CS teaching into disconnected pedagogical parts, complicating content delivery \cite{Repenning2021}.
%   Teachers must guide struggling students toward alternative academic pathways, requiring institutional awareness \cite{Lee2021}.
%   Pandemic-driven exam deadlines created abrupt systemic burdens despite school closures \cite{Perlman2021}.
%   Teacher colleges have not kept pace with curriculum demands like CT inclusion \cite{Simmonds2021}.
%   Dissemination of reusable CS materials remains logistically complex across contexts \cite{Izu2025}.
%   Certification in multiple subjects increases teacher workload without corresponding compensation \cite{Everson2022}.
%   Teacher accountability systems promote punitive test score usage, reducing professional development incentives \cite{McGill2024}.
%   Repetitive student consent forms create administrative fatigue \cite{Patel2024}.
%   Teachers must self-develop Scratch programming content due to its optional status \cite{Jia2022}.
%   Coordinating time for distributed volunteer teachers across time zones wastes valuable support minutes \cite{Malik2024}.
%   Lack of time and curriculum crowding prevent CS teachers from enhancing code quality instruction \cite{Kirk2022}.
%   National CS teacher certification programs and faculty expertise remain insufficient \cite{Weintrop2022}.
%   COVID-19 disrupted in-person workshop delivery, reducing effectiveness of training formats \cite{Lehtimki2022}.
%   TAs often face mismatched course assignments and unclear departmental norms \cite{Minnes2022}.
%   Delegating tasks to TAs is inefficient without strong instructor buy-in or scheduling systems \cite{Akhmetov2024}.
%   Schools struggle to integrate AI into packed curricula without supporting infrastructure \cite{Grover2024}.
%   Adopting new digital tools requires additional time and classroom adjustments \cite{Kumar2022}.
%   TA training remains decentralized, inconsistent, and costly for institutions \cite{Riese2022}.
%   Initial course setup and TA management demand extensive effort and space planning \cite{Brunelle2022}.



% \subsubsection{Socio-cultural Challenges Faced by CS Educators}

% Socio-cultural challenges in computer science (CS) education refer to the broad range of difficulties that arise due to disparities in cultural values, social norms, identity, race, ethnicity, and gender among teachers, students, and institutional structures. These challenges manifest in curriculum design, classroom practices, teacher identity, professional development, and perceptions of who belongs in CS.

% One of the core issues is the underrepresentation of marginalized groups, particularly women and ethnic minorities, which reinforces the perception of CS as a niche and exclusive domain. Teachers often confront the structural legacy of exclusion and a lack of culturally responsive curricula, which can alienate students and exacerbate feelings of not belonging\cite{Hwang2023}. Additionally, there is a widespread view that CS is inaccessible, particularly in classrooms lacking inclusive practices or diverse role models\cite{Everson2022}.

% Teachers from marginalized backgrounds may also face intersectional barriers. For example, some experience pressure to conform to dominant institutional cultures or encounter resistance when introducing alternative pedagogies\cite{Rosenbloom2023}. In professional spaces such as capstone coordination or community engagement, faculty may face added burdens of cultural translation, sustaining relationships with community partners, and managing student expectations across diverse settings\cite{Hooshangi2025}.

% Stereotypical narratives and teaching materials can unintentionally reinforce exclusion. Teachers report challenges with instructional examples that perpetuate gender norms or fail to connect with diverse student identities\cite{Greifenstein2023}. Likewise, even within professional development contexts, educators may find it difficult to relate standardized resources to the lived realities of their students\cite{Simmonds2021}.

% The lack of a strong community of practice around DEI (Diversity, Equity, and Inclusion) topics further limits progress. Teachers often report limited institutional support for equity-driven initiatives beyond surface-level acknowledgements, leaving them to navigate cultural and ethical issues alone\cite{Parthasarathy2024,Yadav2022Review}. This is compounded by geographic disparities that limit rural teachers’ access to DEI-aligned training and professional support\cite{Nugent2022}.

% International instructors and non-native speakers also face socio-cultural hurdles, including accent bias, reduced student trust, and exclusion from informal networks that support teaching excellence\cite{Markel2021,Riese2021}. Teaching assistants (TAs) in particular struggle with navigating cultural differences in student expectations, team collaboration, and feedback dynamics\cite{Minnes2022,Krause-Levy2022}.

% Socio-cultural dynamics affect how educators engage with new technologies as well. With the rise of AI in education, teachers express concerns about algorithmic bias, the loss of pedagogical control, and inequitable access to AI literacy\cite{Lau2023,Sheard2024}. These tensions become more pronounced when educators are not included in discussions about the ethical use of such tools\cite{Mahon2024}.

% Building equitable CS classrooms also means overcoming peer dynamics shaped by cultural assumptions. TAs must manage classroom climates to ensure inclusivity and psychological safety, especially during group projects or student-student collaboration\cite{Huang2023,Akhmetov2024}.

% Ultimately, addressing socio-cultural challenges requires a systemic shift that includes teacher training in cultural competency, support for inclusive curriculum development, and institutional commitments to sustained DEI practice. Only then can we foster a CS education ecosystem that is equitable, welcoming, and reflective of all learners’ experiences.



% \subsubsection{Parental and Community Involvement Challenges}

% Parental and Community Involvement Challenges in computer science education refer to the difficulties educators face when attempting to engage parents and external community stakeholders in meaningful support of students' academic journeys. These challenges are especially relevant for CS teachers, teaching assistants, and tutors who rely on informed community participation to enrich learning experiences and promote sustained interest in computing.

% One major challenge lies in the limited understanding among parents about the significance of digital technologies and computer science as viable and essential career paths. In the context of New Zealand’s secondary school digital technology curriculum, for instance, experts emphasize the critical need for community outreach and parental education to explain the role of CS and programming in future job markets. The lack of such awareness can lead to diminished student motivation and weak community support, making it difficult for educators to build momentum for CS education initiatives \cite{Samarasekara2023}.

% Another significant issue arises during community-engaged learning, such as service-learning or capstone projects. Educators often face the burden of coordinating logistics with external organizations, ensuring students are adequately trained (e.g., for background checks), and maintaining consistent relationships with these community partners. Frequent turnover in partner organizations can disrupt continuity and require educators to repeatedly reestablish networks and project frameworks for new cohorts, leading to operational fatigue and complexity \cite{Hooshangi2025}.

% Moreover, for pre-service teachers—particularly those from underrepresented groups—there are additional barriers rooted in identity-based fears about not being accepted or respected by students and parents. Some educators worry that due to their gender or racial identity, they may not be taken seriously in front of students or families, particularly in regions dominated by a homogenous tech culture. Such fears, often informed by past experiences of bias or exclusion, can undermine confidence and further isolate educators from building trust with families and local communities \cite{Everson2022}.

% Together, these challenges underscore the need for more inclusive, informed, and sustained engagement strategies between educational institutions, families, and local stakeholders in order to strengthen the overall ecosystem of computer science education.


% \subsubsection{Sense of Community/Belonging Challenges}

% Sense of community and belonging challenges in computer science (CS) education refer to the structural, cultural, and interpersonal barriers that hinder educators and students from feeling integrated, supported, and valued within their academic and professional environments. These challenges affect K-12 teachers, university instructors, and teaching assistants (TAs), and include issues of isolation, lack of collegial support, limited opportunities for collaboration, cultural misalignment, and perceived inaccessibility of CS. Such challenges can erode self-efficacy, reduce retention, and inhibit professional growth. Fostering inclusive environments, professional networks, and collaborative practices are crucial to addressing these issues.

% \paragraph{Isolation in CS Teaching Roles.} Many CS educators report feeling isolated due to being the only CS teacher in their school or department, limiting opportunities for peer interaction and feedback. This isolation negatively impacts teacher learning and identity development \cite{Ni2021,Yadav2022,Nugent2022}. Even in professional development settings, efforts must be made to foster community and mitigate the lack of shared professional spaces \cite{Skuratowicz2021,Basu2022}.

% \paragraph{Lack of Collegial Dialogue and Professional Networks.} Teachers often lack structured opportunities for peer dialogue and knowledge-sharing. Studies highlight the importance of communities of practice and personal networking, particularly in emerging fields like AI education \cite{Denny2024,Jetzinger2024,Lee2022}. In their absence, educators struggle to refine practices and build confidence.

% \paragraph{Fragmented TA Communities.} TAs face difficulty in building collaborative environments and cohesive team dynamics. Challenges include inconsistent communication across courses \cite{Akhmetov2024}, independent working despite shared responsibilities \cite{Riese2022}, and difficulty maintaining positive practicum group climates \cite{Minnes2022}. These gaps undermine the sense of belonging and shared mission among teaching teams \cite{Haglund2024}.

% \paragraph{Remote Collaboration and Limited Co-creation.} Remote teaching and professional development contexts often hinder community-building. Teachers report difficulty co-creating lesson plans without face-to-face interaction \cite{Lehtimki2022}, and virtual events require deliberate design strategies to simulate shared experiences and promote engagement \cite{Skuratowicz2021}.

% \paragraph{Cultural and Identity Barriers.} Cultural norms in CS education can marginalize individuals from underrepresented groups. For example, newly recruited students and faculty face pressure to assimilate into dominant cultural norms that do not reflect their identities \cite{Rosenbloom2023}. Similarly, pre-service teachers reported reluctance to join male-dominated programs where they felt they would not be respected or belong \cite{Everson2022}.

% \paragraph{Perception of CS as Inaccessible or Niche.} The perception of CS as an exclusive or highly technical subject contributes to alienation among students and teachers. This perception is compounded by low participation rates among women and minorities, timetabling constraints that restrict deep teacher-student relationships, and stereotypes that frame CS as unapproachable \cite{Hwang2023}.

% \paragraph{Barriers to Instructor Collaboration.} University instructors benefit from collaboration across institutions, yet such networks are rare. Where established, like in shared CS1 course discussions, instructors appreciated the camaraderie and support \cite{Vahid2024}. In other contexts, faculty development programs aim to address fragmentation and build sustainable communities \cite{Marshall2020,Kussmaul2022}.

% \paragraph{Challenges in Tool and Resource Sharing.} Community software development and open educational resource (OER) platforms often lack infrastructure for contributor recognition, feedback, and sustained collaboration. This limits the formation of communities around shared pedagogical tools and reduces the incentive for long-term engagement \cite{Fowler2023,Blanchard2022}.

% \paragraph{Climate and Inclusivity Challenges in Classrooms.} A welcoming climate is crucial for student and TA success. Miscommunication, insensitive phrasing, or poorly managed group dynamics can discourage participation and reinforce feelings of exclusion \cite{Huang2023,Brunelle2022}.

% \paragraph{Unmet Need for Professional Learning Communities.} Programs aimed at improving CS teaching capacity have identified a consistent absence of learning communities, particularly among high school educators. Teachers report lacking opportunities to connect, share, and reflect with peers \cite{Flatland2022,Parthasarathy2024}.



% \subsubsection*{Pedagogical Challenges}

% Pedagogical challenges in computer science (CS) education refer to the multifaceted difficulties that educators face in effectively designing, delivering, and adapting instruction within the rapidly evolving domain of computing. These challenges emerge from the inherent complexity of CS concepts such as abstraction \cite{Begum2025}, the abstract and often inconsistent nature of programming guidelines \cite{Kirk2024}, the integration of inclusive and equitable teaching practices \cite{Patel2024}, and the adaptation of teaching methods to emerging technologies like Generative AI \cite{Mahon2024}. 

% A central issue is the gap between students' conceptual understanding and their ability to apply CS concepts in varied contexts \cite{Begum2025}. Additionally, educators often struggle to reconcile conflicting or language-specific coding style guidelines when teaching text-based programming \cite{Kirk2024}. The incorporation of inclusive design principles—critical for fostering equity and retention—remains underrepresented and underdeveloped in mainstream CS curricula \cite{Patel2024}. Furthermore, the accelerating introduction of tools like GenAI into classrooms necessitates significant rethinking and adaptation of teaching strategies, often without established best practices \cite{Mahon2024}.

% These pedagogical difficulties are intensified by the pace of technological advancement, the societal impact of computing, and institutional constraints, making CS pedagogy a domain in constant flux that demands continuous reflection and innovation from educators.






% \subsubsection{Parental and Community Involvement Challenges}

% Parental and community involvement challenges refer to the difficulties CS educators face in engaging external stakeholders—such as parents, community organizations, and local industry partners—in meaningful, supportive roles in computing education. These challenges manifest in both K–12 and higher education contexts.

% At the K–12 level, a major issue is the lack of parental understanding of computer science concepts, their educational value, and career relevance. As Samarasekara et al.\ \cite{Samarasekara2023} observe, digital technology (DT) educators in New Zealand emphasized the need for broader community and parental education to promote student participation and interest in computing. Without this foundational understanding, efforts to foster computing identity and motivation among students may be undermined by a lack of support at home.

% In higher education, educators often struggle with managing relationships with community partners in service-learning or capstone settings. Hooshangi et al.\ \cite{Hooshangi2025} highlight the substantial coordination effort needed to ensure students are prepared to work with community organizations and maintain long-term institutional partnerships, especially when staff turnover occurs. These logistical hurdles can obstruct consistent student engagement with real-world contexts.

% In pre-service CS teacher education, identity-related fears also play a role in shaping perceptions of community acceptance. Everson and Ko \cite{Everson2022} report that women of color in CS teacher preparation programs often fear being disrespected or dismissed by students and parents due to their race or gender. These perceptions contribute to hesitancy around entering or remaining in CS education, especially in communities with entrenched stereotypes.

% Together, these challenges emphasize that building strong, inclusive, and sustainable partnerships with families and communities is essential for the long-term success of computing education at all levels.



% \begin{itemize}
% \item Who all do we mean by CS educators? --> instructors teaching variety of CS courses, TAs, tutors at all levels of teaching.








% \item What are CS educator problems
% \item What all has been done for CS educators
% \item What were the results.

% \item Highlight what the gap in this entire body of work is, and what we are doing. That is, where are the prior works lacking --> don't know, so we are trying to synthesize and find.

% \item Also highlight no prior synthesis and so we are having to do this job. 


\subsubsection{Sense of Community/Belonging Challenges}

CS educators—teachers, tutors, and TAs—often face barriers to feeling integrated and supported within their institutions. These include isolation, lack of collaboration, cultural misalignment, and perceptions of CS as inaccessible, which hinder retention, identity development, and growth \cite{Ni2021,Yadav2022,Nugent2022}.

\paragraph{Isolation and Lack of Support.} Many report being the only CS educator in their school, limiting peer dialogue and feedback \cite{Ni2021,Yadav2022,Nugent2022}. Even PD programs often fail to foster meaningful community ties \cite{Skuratowicz2021,Basu2022}.

\paragraph{Limited Collaboration and Networks.} Educators lack structured spaces for sharing practices, which hinders confidence-building and professional growth, especially in emerging fields like AI \cite{Denny2024,Jetzinger2024,Lee2022}.

\paragraph{TA Team Fragmentation.} TAs often work independently despite shared duties, facing inconsistent communication and weak practicum group climates \cite{Akhmetov2024,Riese2022,Minnes2022,Haglund2024}.

\paragraph{Remote and Virtual Barriers.} Remote contexts complicate co-creation and community-building; virtual formats need intentional design to foster engagement \cite{Lehtimki2022,Skuratowicz2021}.

\paragraph{Cultural and Identity Tensions.} Underrepresented educators face pressure to assimilate into dominant norms \cite{Rosenbloom2023}, and pre-service teachers often avoid male-dominated programs due to poor belonging \cite{Everson2022}.

\paragraph{CS as Unapproachable.} CS is often perceived as niche and exclusionary, reinforced by gender disparities, time constraints, and stereotypes \cite{Hwang2023}.

\paragraph{Collaboration Gaps.} Instructor collaboration across institutions is rare but valued when present \cite{Vahid2024}. Faculty development programs aim to reduce fragmentation \cite{Marshall2020,Kussmaul2022}.

\paragraph{Resource Sharing Barriers.} Community-driven tools and OER platforms lack mechanisms for recognition and collaboration, reducing sustained engagement \cite{Fowler2023,Blanchard2022}.

\paragraph{Classroom Climate and Inclusivity.} Miscommunication and poor group dynamics affect students’ and TAs’ sense of belonging \cite{Huang2023,Brunelle2022}.

\paragraph{Need for Learning Communities.} High school CS teachers frequently lack professional peer networks to reflect and grow \cite{Flatland2022,Parthasarathy2024}.




% \subsection{Citation Insights Across Challenge Categories}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{Images/cite.png}
%     \caption{Number of Unique Paper References per CS Educator Challenge Category}
%     \label{fig:challenge-distribution}
% \end{figure}

% An analysis of the distribution of research paper citations across different CS educator challenge categories reveals significant disparities in scholarly attention. The most heavily cited categories include \textbf{Pedagogical Challenges} (104 papers), \textbf{Administrative and Institutional Challenges} (82), and \textbf{Training \& Professional Development Challenges} (72), indicating strong research focus in these areas. Other well-represented areas include \textbf{Technological Challenges} (69) and \textbf{Emotional and Psychological Challenges} (61).


% However, the analysis also highlights five categories that have received comparatively limited attention, each with fewer than 50 citations:
% \begin{itemize}
%     \item \textbf{Classroom Management Challenges} (42)
%     \item \textbf{Socio-cultural Challenges} (50)
%     \item \textbf{Assessment and Evaluation Challenges} (55)
%     \item \textbf{Sense of Community/Belonging Challenges} (30)
%     \item \textbf{Parental and Community Involvement Challenges} (3)
% \end{itemize}

% This uneven distribution suggests that while core teaching and institutional issues dominate the literature, there is a critical need for further research into the underrepresented areas—particularly those concerning community involvement and educators' sense of belonging. Addressing these gaps can contribute to a more comprehensive understanding of the multifaceted challenges faced by CS educators. As shown in Figure~\ref{fig:challenge-distribution}, the citation counts clearly reflect these research priorities and gaps.



% \subsection{Remedy Citation Insights Across Challenge Categories}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{Images/remedy.png}
%     \caption{Number of Remedy Citations per CS Educator Challenge Category}
%     \label{fig:remedy-distribution}
% \end{figure}

% The distribution of remedy-oriented citations across CS educator challenge categories further confirms the uneven nature of scholarly intervention:

% \begin{itemize}
%     \item \textbf{Extensively Addressed Categories:}
%     \begin{itemize}
%         \item \textbf{Pedagogical Challenges} again lead with 107 remedy citations, underscoring a substantial body of solutions aimed at improving classroom instruction and curriculum design.
%         \item \textbf{Administrative and Institutional Challenges} (91) and \textbf{Training \& Professional Development} (88) show strong remedy support, reflecting actionable frameworks to support educators at systemic and individual levels.
%         \item \textbf{Emotional and Psychological Challenges} (77) also receive considerable remedy attention, revealing growing efforts to mitigate teacher stress, burnout, and emotional fatigue.
%     \end{itemize}

%     \item \textbf{Moderately Addressed Categories:}
%     \begin{itemize}
%         \item \textbf{Assessment and Evaluation} (73) and \textbf{Technological Challenges} (71) are areas where practical interventions are being explored to improve grading systems and integrate digital tools effectively.
%         \item \textbf{Classroom Management} (55), \textbf{Socio-cultural Challenges} (56), and \textbf{Sense of Belonging} (54) reflect moderate remedy efforts, but these still fall short considering their foundational importance to an inclusive learning environment.
%     \end{itemize}

%     \item \textbf{Critically Underaddressed:}
%     \begin{itemize}
%         \item \textbf{Parental and Community Involvement} (11) remains vastly underexplored in terms of remedies, signaling a persistent blind spot in CS education research concerning collaboration with families and communities.
%     \end{itemize}
% \end{itemize}

% Figure~\ref{fig:remedy-distribution} highlights the urgent need to extend remedy efforts beyond pedagogy and institutional reform. Future research should prioritize holistic and inclusive strategies that integrate community voices, cultural context, and emotional support into CS educator interventions.













% Figure~\ref{fig:wordcloud} presents a word cloud generated from the keywords of the 120 final filtered papers included in our review. Prominent terms such as “pedagogy”, “programming”, “training”, “students”, “curriculum”, and “assessment” highlight the dominant focus areas in recent literature. The visual representation underscores a strong emphasis on faculty development, learning environments, and programming instruction, reflecting the multifaceted concerns surrounding CS teacher preparation and support.





% In computing education, the term \textit{CS educators} encompasses a diverse set of stakeholders involved in teaching, mentoring, and supporting learners at various academic levels and instructional contexts. This includes:

% \textbf{Instructors and Faculty:} These are educators responsible for designing and delivering a wide range of CS curricula, including introductory courses like CS1 \cite{Vahid2024,Vahid2024b}, capstone courses \cite{Hooshangi2025}, ethics and accessibility integration \cite{Hu2023,Parthasarathy2024}, AI and machine learning in K-12 settings \cite{Grover2024,Jetzinger2024,DiPaola2023}, and advanced pedagogical strategies such as inclusive design \cite{Patel2024}. Faculty members are also central to shaping national computing standards \cite{Thigpen2024,McGill2024}, implementing curriculum-wide reform \cite{Musaeus2024}, and mentoring future CS teaching-focused faculty \cite{Farghally2024}. Their experiences are also being studied in the context of AI tool integration \cite{Sheard2024,Cucuiat2024} and debugging as a computational thinking practice \cite{Macann2023}.

% \textbf{Teaching Assistants (TAs):} TAs play a critical role in providing feedback, tutoring support, and classroom management in large or complex CS courses \cite{Zaman2023,Akhmetov2024,Haglund2024}. Their responsibilities range from grading and content delivery to helping students understand subtle programming concepts \cite{Haglund2024}. The rise of AI-powered teaching tools like TA-Bot and other automated systems is aimed at augmenting TA workflows in large-scale settings \cite{Forden2023,Denny2024}. Effective TA management and feedback literacy are essential for their pedagogical impact \cite{Cheng2024,Akhmetov2024}.

% \textbf{Tutors:} Tutors, whether human or AI-driven, offer one-on-one or small-group support for learners. Systems like \textit{Iris}, an AI-based tutor, provide real-time, context-aware support that fosters independent problem-solving \cite{Bassner2024}. Similarly, tools like \textit{TeachNow} enable volunteer teachers to deliver spontaneous 1:1 assistance in massive online courses \cite{Malik2024}. Tutors are also supported by just-in-time interventions that improve their instructional performance \cite{Cheng2024}.

% \textbf{K-12 and Pre-Service Teachers:} A significant portion of computing educators operate in primary and secondary school settings. These educators face unique challenges related to professional development \cite{Shanley2023,Macann2023,DiPaola2023,Jetzinger2024}, curriculum development \cite{Grover2024,Greifenstein2023}, and ethics integration \cite{Hu2023}. Their perspectives shape the landscape of early computing education.



\subsection{Remedies Implemented for Pedagogical Challenges}

Computer science (CS) education faces a variety of pedagogical challenges, ranging from effectively training instructors and teaching assistants (TAs) to making CS accessible and engaging for diverse student populations. In response, researchers and educators have proposed and implemented a variety of targeted remedies.

A significant focus has been on improving the pedagogical skills of CS instructors and TAs, many of whom lack formal training in teaching methodologies, which can hinder student learning \cite{Cook2022,Riese2021,Zaman2023}. Remedies include Explicit pedagogical instruction that is Programs now train TAs to provide effective, non-prescriptive feedback, identify gaps in understanding, use complete sentences, and ask guiding questions. Strategic use of code snippets (e.g., examples or test cases) is emphasized over direct solutions \cite{Cook2022,Zaman2023}.
    %Structured practicum and mentorship
Also Small-group practicum sessions enable TAs to practice micro-teaching,grading, and discuss scenarios. Experienced TAs act as mentors while new TAs receive observation-based feedback \cite{Minnes2022,Akhmetov2024}.
    
To remediate Classroom climate and inclusivity issues, training now incorporates inclusive practices, focusing on language use, diverse examples, and accessible course content to foster a welcoming environment \cite{Huang2023}.
Also for TAs Just-in-time teaching tips that is Short, actionable tips provided immediately before tutoring sessions help TAs guide conversations, ask open-ended questions, and diagnose misconceptions \cite{Cheng2024}.
    
To improve the Content and pedagogical content knowledge (PCK) Instructor development programs address core CS concepts, abstract reasoning, and the adaptation of existing material \cite{Yadav2022,McGill2024,Everson2022,Kumar2021}. TA training also integrates general pedagogy, PCK, and TPACK models \cite{Riese2022}.


For teachers the Make-a-Thon (MAT) was specifically designed to empower teachers as AI curriculum designers, enabling them to "understand, use modify, and create AI curricula" rather than just implementing pre-written materials. The core of the MAT involved co-design of AI literacy materials, where teachers played a central role in the design process.\cite{DiPaola2023}

As observed is listed challenges that teacher lacked content knowledge so as part of study a Faculty Development Program (FDP) was conducted aimed at demonstrating improved methods for conducting CS1 programming labs. This involved providing instructors with examples of programming tasks and assigning them as hands-on exercises to offer a student's perspective.\cite{Kumar2021}.Similarly as diagonatic tool was introduced in year 2024 and The core purpose of the diagnostic tool itself is to provide targeted professional development (PD) recommendations that support teachers' content and pedagogical content knowledge in CS.For this the mixed-methods study involved 66 teachers and a revised diagnostic tool that collected actual evidence of classroom practices through submitted artifacts and justifications, alongside a self-assessment instrument measuring practices connected to the CSTA Standards. While the diagnostic tool proved helpful in recommending PD for two-thirds of the participating teachers and the majority of teachers agreed with the identified strengths and growth areas, the self-assessment instrument was found to be largely uncorrelated with the diagnostic results, likely due to the Dunning-Kruger effect, where teachers tended to overestimate their proficiency.

As part of Curriculum Design and Delivery innovative curriculum strategies seek to enhance student engagement, understanding, and application such as contextualized and real-world learning in which 
Projects are made relevant to students’ lives using local stories and real-world applications, especially in underrepresented regions 
\cite{Venn-Wycherley2020,Samarasekara2023,Hamouda2025}.
    
More over Project-based learning where Hands-on team projects, game development, and Arduino-based activities foster practical experience and industry relevance \cite{Lee2021,Hooshangi2025,Repenning2021,Hamouda2025}.
Also Scaffolded instruction where "Many small programs" and progressive tasks help students build skills incrementally. Automated assessment systems (APASs) support timely feedback \cite{Vahid2024,Sauerwein2023}.
Introduction of Educational technology Tools like \textit{Storyteller} and \textit{SnapCheck} enhance interactivity and automate feedback in visual programming tasks \cite{Mahoney2023,Wang2021}.
Interdisciplinary modules where integrating CS with math or ethics provides richer learning contexts and helps build connections across domains \cite{Kalathas2022,Hu2023}.

    
    % \item \textbf{Collaborative learning:} Strategies such as PRIMM (Predict, Run, Investigate, Modify, Make) foster student discussion around shared programming artifacts. Collaboration platforms also ensure equitable participation \cite{Sentance2021,Musaeus2024}.
    
Visualizing student thought processes such as CodeProcess Charts allow educators to analyze how students approach problems, aiding in instructional design \cite{Shrestha2022}.


\subsubsection*{Addressing Specific Student Needs and Challenges}

Tailored strategies help support diverse learners and address individual challenges:

\begin{itemize}
    \item \textbf{Disability support and UDL:} Universal Design for Learning (UDL) principles are applied in special education settings. Materials are adapted for visual impairments and multisensory engagement \cite{Yadav2022,Huff2021}.
    
    \item \textbf{Bridging knowledge gaps:} Adding lab sections and employing mastery learning ensures students have the prerequisite knowledge before advancing 
    \cite{Luu2023,Krause-Levy2022,Krause-Levy2023,Hooshangi2025}.
    
    \item \textbf{Growth mindset through language:} Educators replace stigmatizing terms like “wrong” with “debugging,” helping students view errors as part of the learning process \cite{Macann2023}.
    
    \item \textbf{Adapting to Generative AI:} Instructors are reshaping curricula to prepare students for a future with AI-assisted development. This includes training students to critically evaluate AI outputs and use tools as learning aids rather than crutches \cite{Mahon2024,Sheard2024,Lau2023}.
\end{itemize}

\subsection{Remedies Implemented for Assessment and Evaluation Challenges}

Educators in computer science face numerous assessment and evaluation challenges, ranging from ensuring fairness and consistency to effectively gauging complex learning outcomes. A variety of remedies—spanning technological tools, pedagogical practices, and policy interventions—have been proposed and implemented to address these concerns.

\subsubsection*{Enhancing Feedback and Grading Efficiency}

Providing timely, actionable feedback while managing large classes remains a persistent challenge. To address this, educators are leveraging automation and structured assessment practices:

\begin{itemize}
    \item \textbf{Automated Assessment Systems (APASs):} Tools like \textit{ShellOnYou} and \textit{TA-Bot} offer automated, instant feedback on programming exercises, easing grading loads and supporting iterative learning \cite{Berry2022,Forden2023,Sauerwein2023}. Auto-graders with immediate feedback and partial credit are common in large courses \cite{Vahid2024}.
    
    \item \textbf{Improved autograder feedback:} Educators recommend enhancing autograder outputs with detailed error messages, correct answers after repeated incorrect submissions, and options for awarding partial credit \cite{Shanley2023}.
    
    \item \textbf{Rubrics and exemplars:} Clear, multi-level rubrics with well-defined categories help standardize grading. Exemplars serve to align student expectations with instructor evaluation criteria \cite{Esche2024,Kirk2022,Hooshangi2025}.
    
    \item \textbf{Code quality tools:} Static analysis tools assist in identifying code issues objectively, supporting instructors in focusing feedback on conceptual or stylistic improvements \cite{Izu2025}.
    
    \item \textbf{Data-driven instructional insights:} Tools like \textit{UserFlow} and \textit{Solvelets} track fine-grained student activity and problem-solving steps. This data helps instructors evaluate engagement and conceptual growth beyond binary correctness \cite{Singh2020,Kumar2022}.
\end{itemize}

\subsubsection*{Ensuring Fairness, Consistency, and Academic Integrity}

Fair assessment practices and the rising challenge of AI-based plagiarism require proactive strategies:

\begin{itemize}
    \item \textbf{Unique and randomized exams:} Frameworks like \textit{Unique Exams} generate individualized assessments to deter plagiarism and allow flexible exam formats \cite{Rusak2021}.
    
    \item \textbf{Multiple assessment modalities:} Incorporating diverse formats—such as oral, video-based, or image-based exams—reduces reliance on AI-generated code and supports authentic evaluation \cite{Mahon2024,Hamouda2025,Lau2023,Sheard2024}.
    
    \item \textbf{Process-based assessment:} Evaluating student work throughout the development cycle, rather than just final output, discourages shortcut solutions and promotes deeper understanding \cite{Mahon2024,Sheard2024,Lau2023}.
    
    \item \textbf{Plagiarism detection tools:} Systems like \textit{MOSS} and \textit{CodeProcess Charts} help identify copied or cosmetically altered work by tracing code development history \cite{Forden2023,Shrestha2022}.
    
    \item \textbf{Clear policies on AI usage:} Institutions are implementing explicit guidelines on permissible AI use, requiring disclosure, and warning against dishonest practices \cite{Mahon2024,Sheard2024}.
    
    \item \textbf{TA training on academic integrity:} Training programs prepare TAs to detect and address plagiarism and navigate ethical dilemmas \cite{Riese2022}.
    
    \item \textbf{Standardized assessments and data pooling:} Standard exams across institutions enable benchmarking and consistent evaluation. Shared question banks also support refinement of assessment practices through analytics \cite{Krause-Levy2023,Vahid2024}.
\end{itemize}

\subsubsection*{Developing Comprehensive Assessment Literacy}

Improving educators' understanding of assessment principles and practices is essential for effective evaluation:

\begin{itemize}
    \item \textbf{Professional development for assessment literacy:} PD programs focus on eliciting, interpreting, and applying assessment data. They support the design of formative assessments and educative scoring rubrics \cite{Basu2022}.
    
    \item \textbf{Targeted diagnostic tools:} Tools are being piloted to measure CS content and pedagogical knowledge, allowing for objective, growth-oriented insights into teacher competency \cite{McGill2024,Thigpen2024}.
    
    \item \textbf{Integrating assessment in course design:} Faculty development initiatives encourage alignment of intended learning outcomes (ILOs) with assessment strategies using frameworks such as Bloom’s Taxonomy \cite{Farghally2024,Huang2023}.
    
    \item \textbf{Calibration sessions for subjective grading:} Collaborative discussions among graders help establish consistent scoring standards for subjective evaluations such as projects and essays \cite{Kao2020,Hooshangi2025}.
    
    \item \textbf{Reframing assessment purpose:} Instructors are encouraged to view assessments not just as grading tools but as instruments to inform instruction and identify student difficulties \cite{Basu2022}.
\end{itemize}

These multi-pronged strategies contribute to a more robust, transparent, and equitable assessment framework in computer science education, equipping educators to better evaluate, support, and guide student learning.

\subsection{Remedies Implemented for Classroom Management Challenges}

Effective classroom management is foundational for maintaining a productive and inclusive learning environment in computer science education, particularly amid growing class sizes, evolving technologies, and diverse learner needs. Educators are adopting a combination of technological, pedagogical, and organizational strategies to address these multifaceted challenges.

\subsubsection*{Managing Large Class Sizes and Workload}

With surging enrollments in CS courses, managing large student cohorts and the associated instructional workload is a pressing concern. Several scalable and supportive approaches are being implemented:

\begin{itemize}
    \item \textbf{Leveraging TAs and support teams:} Instructors increasingly rely on teaching assistants for individualized interaction. Dedicated support teams for communication (e.g., Discord) and scheduling (e.g., lab coordination) have significantly reduced instructor overhead \cite{Mason2024,Akhmetov2024}.
    
    \item \textbf{Automated tools for efficiency:} Assessment tools such as \textit{TA-Bot} and APASs streamline grading and provide instant feedback, enabling instructors to prioritize student engagement and instruction \cite{Sauerwein2023,Wang2021,Forden2023,Vahid2024}.
    
    \item \textbf{Scalable course structures:} Structuring courses around small student cohorts (e.g., groups of six) fosters personal interaction and reduces congestion during office hours. Staggered deadlines can also help balance instructional load \cite{Brunelle2022}.
    
    \item \textbf{Self-contained learning tools:} Tools like \textit{Solvelets} allow students to practice independently without requiring instructor-led demonstrations, thereby reducing in-class time spent on tool training \cite{Kumar2022}.
\end{itemize}

\subsubsection*{Fostering Engagement and Addressing Behavioral Issues}

Classroom management also entails sustaining attention, minimizing disruptions, and promoting constructive collaboration:

\begin{itemize}
    \item \textbf{Engaging and flexible curricula:} Personalized, project-driven activities support sustained interest and minimize behavioral issues. Flexible lesson structures (e.g., “critical paths”) allow educators to adapt pacing and depth \cite{Venn-Wycherley2020}.
    
    \item \textbf{Promoting productive collaboration:} Structured teamwork (e.g., booked lab rooms, digital collaboration tools) enhances peer learning. TA training on group facilitation and psychological safety further promotes inclusive collaboration \cite{Berry2022,Huang2023,Musaeus2024}.
    
    \item \textbf{Addressing distractions and unproductive behaviors:} Recognizing off-task behavior as potential indicators of learning difficulties enables timely support. Monitoring tools and teacher awareness can reduce disengagement \cite{Pieper2020}.
    
    \item \textbf{Clear expectations and classroom policies:} Transparent grading policies, deadlines, and guidelines for AI tool use help reduce confusion and maintain order. Educators are urged to articulate what uses of AI are permissible and the associated consequences of misuse \cite{Vahid2024,Mahon2024}.
\end{itemize}

\subsubsection*{Supporting Diverse Learning Environments and Student Needs}

Adapting classroom practices to accommodate diverse student backgrounds, technical configurations, and learning preferences is essential:

\begin{itemize}
    \item \textbf{Consistent development environments:} Containerization tools like Docker (e.g., for RVCE emulator) ensure all students work in a standardized technical environment, reducing configuration-related disruptions \cite{Nitta2022}.
    
    \item \textbf{Support for virtual and remote learning:} Platforms like \textit{Replit.com} and \textit{NetsBlox} facilitate collaborative remote programming. Instructors also use PD strategies such as scheduled breaks and breakout rooms to mitigate “Zoom fatigue” \cite{Flatland2022,Skuratowicz2021}.
    
    \item \textbf{Individualized support for varied skill levels:} Flexible office hours, pre-learning materials, and career guidance help meet the needs of students with differing levels of prior experience. Tailored interventions also support students with disabilities \cite{Lee2021,Huff2021}.
    
    \item \textbf{Culturally responsive practices:} Educators foster authentic engagement by integrating students’ cultural experiences and personal interests into class discussions. Careful facilitation of intercultural collaboration can enhance inclusivity \cite{Rosenbloom2023,Hamouda2025}.
    
    \item \textbf{Professional development for classroom management:} PD programs equip teachers and volunteers with classroom strategies, focusing on student-centered management, communication skills, and age-appropriate engagement techniques \cite{Yadav2022,Williams2020}.
\end{itemize}

By combining automated tools, strategic TA deployment, inclusive pedagogy, and professional development, educators aim to create CS learning environments that are manageable, equitable, and responsive to diverse student needs.


\subsection{Remedies for Emotional and Psychological Challenges}

Emotional and psychological challenges can significantly impact both educators and students in computing education, affecting motivation, confidence, and overall well-being. Addressing these issues often involves fostering supportive environments, building self-efficacy, and adopting empathetic teaching practices.

\subsubsection*{Boosting Confidence and Self-Efficacy}

Many educators, especially those new to teaching CS, grapple with feelings of inadequacy, stress, and isolation. Students, too, can experience frustration and low confidence when facing difficult concepts.

\begin{itemize}
    \item \textbf{Targeted Professional Development (PD) and Training:} PD programs are designed to directly address teacher self-doubt and foster positive self-perceptions in CS \cite{Vivian2020}. This includes emphasizing that developing expertise takes time (e.g., four years or more for CS self-esteem), thereby promoting a growth mindset \cite{Vivian2020}. TA training modules incorporate concepts like growth mindset and stereotype threat to encourage more empathetic teaching practices \cite{Zaman2023}.
    
    \item \textbf{Building a Supportive Community:} Professional learning communities (PLCs) offer teachers and TAs opportunities for peer support and mentorship, addressing professional isolation and promoting well-being \cite{Flatland2022,Kussmaul2022,Perlman2021,Jocius2021,Skuratowicz2021,Tsan2022,Lee2022,Wilde2024,Haglund2024}. These communities validate educators’ experiences and enable collaborative problem-solving \cite{Minnes2022,Goletti2021,Farghally2024}.
    
    \item \textbf{Co-creation and Collaborative Learning:} Involving teachers in co-designing curricula and resources (e.g., through Make-a-Thons) enhances ownership and confidence in applying new content \cite{DiPaola2023,Musaeus2024,Lehtimki2022}. For students, collaborative approaches such as pair programming help mitigate isolation and increase confidence \cite{Hamouda2025}.
    
    \item \textbf{Increased Instructor Support and Feedback:} Providing clear curricular resources and human support enhances confidence in addressing complex topics such as code quality \cite{Kirk2022}. TAs are trained to offer motivational rather than evaluative feedback, reframing their role as supportive allies \cite{Cook2022,Zaman2023}. Additionally, automated tools reduce social pressure and support self-paced learning \cite{Wang2021}.
    
    \item \textbf{Reduced Workload and Autonomy:} Centralized resources and minimized administrative burdens free instructors to focus on engaging instruction, improving job satisfaction \cite{Vahid2024}. Allowing TAs to choose team preferences also reduces stress and increases autonomy \cite{Akhmetov2024}.
\end{itemize}

\subsubsection*{Addressing Stress, Anxiety, and Emotional Well-being}

Educators and students can experience stress and anxiety due to heavy workloads, imposter syndrome, and emotionally difficult classroom dynamics.

\begin{itemize}
    \item \textbf{Creating Safe and Inclusive Environments:} Classrooms designed with a ``climate-first'' approach promote psychological safety and reduce stereotype threat, imposter syndrome, and microaggressions \cite{Huang2023}. TA training includes modules on unconscious bias and anti-discrimination strategies to foster inclusion and student openness to help-seeking \cite{Krause-Levy2023}.
    
    \item \textbf{Destigmatizing Mistakes:} Reframing errors as part of the learning process (e.g., ``debugging'' instead of being ``wrong'') encourages persistence and reduces anxiety \cite{Macann2023}. Gamified tools such as \textit{ShellOnYou} offer playful learning experiences, lowering fear of failure \cite{Berry2022}.
    
    \item \textbf{Flexible and Adaptable Programs:} Shorter, asynchronous or staggered PD programs reduce scheduling stress and accommodate personal responsibilities \cite{Tsan2022}. Similarly, features like code playback let students revisit materials at their own pace, reducing stress during live coding sessions \cite{Mahoney2023}.
    
    \item \textbf{Direct Support for Mental Health:} Some programs explicitly encourage TA mental health discussions, reflection, and emotional resilience \cite{Farghally2024,Riese2022,Minnes2022}. Safe reflection spaces help TAs process their teaching challenges constructively.
    
    \item \textbf{Confronting Difficult Topics:} Engaging educators with real-world issues—like algorithmic bias or accessibility—through workshops helps develop confidence in navigating sensitive discussions while fostering student agency and awareness \cite{Hu2023,Parthasarathy2024}.
\end{itemize}




\subsection{Remedies for Technological Challenges}
Technological challenges in computing education are multifaceted, encompassing limited infrastructure, inconsistent access to tools, and difficulties in keeping pace with rapidly evolving technologies such as AI. In response, educators and institutions have adopted several strategic remedies aimed at improving accessibility, reducing technical barriers, and facilitating the meaningful integration of emerging technologies.

\subsubsection*{Providing Accessible and User-Friendly Tools}
\begin{itemize}
    \item \textbf{Web-Based and Containerized Environments:} Tools deployed via the browser and Docker-based containers ensure consistent, cross-platform access to development environments. Solutions like the RISC-V Console Emulator (RVCE) eliminate hardware dependencies, allowing seamless embedded system instruction from any location \cite{Kumar2022,Nitta2022,Forden2023}.
    
    \item \textbf{Low-Cost Devices and Open-Source Tools:} In resource-constrained contexts, using affordable hardware like Raspberry Pi or Arduino, combined with open-source platforms such as Linux USBs and Moodle, offers a practical and cost-effective approach to hands-on computing education \cite{Hamouda2025}.
    
    \item \textbf{User-Friendly Interfaces:} Developing intuitive platforms and selection-based UIs—for example, for test authoring or instructional tools—lowers the barrier for educators and enhances tool adoption \cite{Wang2021,Forden2023}.
    
    \item \textbf{Living and Centralized Repositories:} Dynamic repositories curated with up-to-date tools and resources help educators stay aligned with rapidly evolving technologies. AI teaching repositories and centralized tool databases facilitate discoverability and quality assurance \cite{Grover2024,Blanchard2022,Fowler2023}.
\end{itemize}

\subsubsection*{Addressing Technical Barriers and Infrastructure Gaps}
\begin{itemize}
    \item \textbf{Low-Tech and Offline Alternatives:} Using printed workbooks as alternatives to online tools ensures continuity in instruction where IT infrastructure is unreliable \cite{Lehtimki2022}.
    
    \item \textbf{Remote and Low-Bandwidth Adaptations:} Browser-based labs, collaborative coding environments, and minimal-internet solutions like “chat-only mode” or modified Google Docs enable equitable access across devices, even in bandwidth-constrained regions \cite{Malik2024,Flatland2022,Hamouda2025}.
    
    \item \textbf{Technical Support and Institutional Roles:} Proactive “tech checks” before professional development (PD) sessions and dedicated help desks address real-time issues. Institutional support staff also play a critical role in classroom tech maintenance \cite{Jocius2021,Skuratowicz2021,Flatland2022}.
    
    \item \textbf{Technological Pedagogical Training:} Formal training on Technological Pedagogical Content Knowledge (TPACK) equips TAs and teachers with strategies to apply technology meaningfully in instruction, avoiding assumptions about innate technical fluency \cite{Riese2021,Riese2022,Williams2020}.
    
    \item \textbf{Automation of Administrative Workflows:} Automating tasks such as grading, plagiarism detection, and student support through scripts or LMS-integrated tools reduces cognitive load and streamlines instructional efforts \cite{Akhmetov2024}.
\end{itemize}

\subsubsection*{Navigating Emerging Technologies (e.g., AI and GenAI)}
\begin{itemize}
    \item \textbf{AI Integration for Feedback and Support:} Enhancing tools like program repair systems with LLMs (e.g., GPT-3.5, GPT-4) enables personalized, scalable feedback without sacrificing efficiency \cite{Ishizue2024}.
    
    \item \textbf{Prompt Engineering and AI Guardrails:} Designing prompts for desirable AI outputs and implementing guardrails (to avoid direct solution leakage) fosters responsible student engagement with AI tools \cite{Ishizue2024,Denny2024}.
    
    \item \textbf{Redesigning IDEs for AI-Aware Pedagogy:} Future IDEs are being reimagined to support critical coding skills—like debugging, comprehension, and critique—while incorporating readability and formatting improvements in AI-generated content \cite{Lau2023,Cucuiat2024}.
    
    \item \textbf{Addressing Ethical and Bias Concerns:} As AI becomes embedded in classrooms, educators must consider issues like biased outputs, data privacy, and responsible usage. Training should also include effective student interaction with GenAI through prompt design and critical evaluation \cite{Mahon2024}.
    
    \item \textbf{Unplugged AI Activities:} To foster AI literacy without tech dependencies, unplugged activities (e.g., paper-based debugging or simulation games) are used to teach core concepts and logic in an engaging and equitable manner \cite{Macann2023,Grover2024}.
\end{itemize}

\subsection{Remedies for Administrative and Institutional Challenges}

Administrative and institutional challenges in computing education stem from structural constraints such as faculty shortages, funding limitations, rigid curricula, and inconsistent policy support. Overcoming these barriers requires multi-pronged strategies involving staffing reforms, policy development, and sustained institutional support.

\subsubsection*{1. Addressing Staffing Shortages and Workload}

\begin{itemize}
    \item \textbf{Hiring Adjuncts and Alumni:} Universities are mitigating faculty shortages by recruiting alumni as adjunct instructors for introductory CS courses. This helps distribute teaching loads, reduce class sizes, and enhance student engagement \cite{VanDeGrift2023}.
    
    \item \textbf{Tiered TA Structures:} Introducing structured TA hierarchies (instructors, lead TAs, and sub-teams) improves role clarity and workload delegation. Functional teams (e.g., Scheduling, Communication, Plagiarism Support) enhance operational efficiency \cite{Akhmetov2024}.
    
    \item \textbf{Automation Tools:} The use of automated assessment platforms (e.g., TA-Bot, Solvelets) significantly reduces grading effort and supports personalized learning at scale \cite{Sauerwein2023,Forden2023,Wang2021,Kumar2022}.
    
    \item \textbf{Centralized Course Materials:} Shared repositories of syllabi, assessments, and content allow instructors to focus on student interaction and innovation rather than redundant preparation work \cite{Vahid2024}.
    
    \item \textbf{Financial Incentives:} Scholarships and stipends for teacher certification help attract and retain CS educators, particularly in underserved areas \cite{Everson2022,Yadav2022,Perlman2021}.
\end{itemize}

\subsubsection*{2. Enhancing Teacher Preparation and Professional Development}

\begin{itemize}
    \item \textbf{Expanding Recruitment Pipelines:} Partnering with iSchools provides alternative routes to train K--12 CS educators, broadening the talent pool beyond traditional CS departments \cite{Weintrop2022}.
    
    \item \textbf{Formal Certification Pathways:} Creating structured pathways (e.g., emergency permits, postgraduate add-on licenses) is key to preparing a certified CS teaching workforce \cite{Yadav2022,Flatland2022}.
    
    \item \textbf{Scalable PD Models:} Online and hybrid PD formats (e.g., MOOCs, virtual workshops) offer cost-effective and accessible training for large cohorts of teachers \cite{Jetzinger2024,Tsan2022}.
    
    \item \textbf{Long-Term Institutional Investment:} Continued support from universities and governments is essential for sustainable PD programs, resource provisioning, and lab infrastructure \cite{Yadav2022,Flatland2022,Huff2021,Saraiva2021,Hamouda2025}.
    
    \item \textbf{Strategic Alliances:} Collaborations between ministries, universities, and industry partners ensure curriculum relevance and policy alignment through evidence-based approaches \cite{Simmonds2021,Hamouda2025,Friend2022}.
\end{itemize}

\subsubsection*{3. Curriculum Alignment, Policy, and Institutional Support}

\begin{itemize}
    \item \textbf{Standardizing Curricula and Policies:} Establishing national CS standards and inter-university course sharing initiatives reduces redundancy and promotes consistent quality \cite{Upadhyaya2020,Jia2022,Vahid2024}.
    
    \item \textbf{Stakeholder Education:} Training administrators on CS and AI literacy enables them to better support curricular integration and resource allocation \cite{Grover2024,Simmonds2021,Parthasarathy2024}.
    
    \item \textbf{Addressing Time Constraints:} Embedding CS within other subjects and leveraging tools for rapid content creation (e.g., code playback, game generators) allows efficient curriculum delivery without overburdening faculty \cite{Kalathas2022,Anyango2021,Mahoney2023}.
    
    \item \textbf{Flexible Curriculum Design:} Ensuring adaptability in curricula helps teachers contextualize content for local needs and pivot effectively in response to emergencies (e.g., virtual learning) \cite{Jia2022,Hwang2023,Brunelle2022,Skuratowicz2021}.
    
    \item \textbf{Recognition for Faculty Contributions:} Incentivizing Open Educational Resources (OER) development through formal recognition, citation tracking, and scholarly normalization promotes sustainable content creation \cite{Fowler2023}.
    
    \item \textbf{Policy Development for AI Integration:} Institutions must proactively develop guidelines for ethical use of Generative AI tools in teaching and assessment, involving multi-stakeholder collaboration \cite{Mahon2024,Lau2023}.
\end{itemize}


\subsection{Remedies for Training and Professional Development Challenges}

The rapid evolution of computer science (CS) and the growing demand for CS education have intensified training and professional development (PD) challenges for educators at all levels. A significant proportion of teachers and teaching assistants (TAs) lack formal backgrounds in CS or discipline-specific pedagogical training, highlighting the critical need for sustained, accessible, and context-relevant professional learning opportunities.

\subsubsection*{Comprehensive and Sustained Training Programs}
Traditional PD formats are often short, generic, or disconnected from classroom realities. To address this, effective remedies emphasize the design of long-term, iterative, and multifaceted PD programs that support continuous learning and reflection.

\begin{itemize}
    \item \textbf{Extended and Iterative PD Models:} Programs that span months rather than days allow educators to reflect, apply, and adapt knowledge over time \cite{Tsan2022,Lee2022}. The Everyday AI (EdAI) initiative, for example, combines a year-long AI Book Club, Summer Practicum, and monthly webinars to systematically scaffold teachers' understanding and application of AI curricula \cite{DiPaola2023}. This approach mitigates cognitive overload and fatigue \cite{Lee2022}.
    
    \item \textbf{Integrated Content and Pedagogy:} PD must strengthen both content knowledge and pedagogical content knowledge (PCK), equipping educators to teach CS concepts effectively \cite{Basu2022,Everson2022,Tsan2022,Yadav2022}. Techniques include structured debugging, clear instructional strategies, and cognitive activation methods \cite{Macann2023,Jia2022}. The ``pedagogical double-decker'' principle emphasizes learning both what and how to teach, particularly in AI education \cite{Jetzinger2024}.
    
    \item \textbf{Hands-on and Active Learning:} Active engagement through lesson rehearsals, collaborative coding, and the use of physical computing tools enhances learning retention and application \cite{Patel2024,Tsan2022,Skuratowicz2021,Hamouda2025}. Co-creating educational materials further deepens ownership and understanding \cite{DiPaola2023,Musaeus2024,Lehtimki2022,Grover2024}.
    
    \item \textbf{Structured Mentoring and Peer Learning:} Regular interaction with mentors and peers, both virtually and in person, promotes reflective practice and mutual learning \cite{Kussmaul2022,Minnes2022,Flatland2022,Wilde2024,Haglund2024,Markel2021}. This is particularly beneficial for TAs navigating complex classroom dynamics \cite{Riese2021}.
\end{itemize}

\subsubsection*{Addressing Specific Knowledge Gaps and Skills}
Educators’ varied backgrounds demand targeted PD interventions that address distinct knowledge and skill deficiencies.

\begin{itemize}
    \item \textbf{Foundational CS Skills:} Programs should focus on core programming and computational thinking, particularly for new or transitioning teachers \cite{Kumar2021,Everson2022,Flatland2022}, including hands-on familiarity with modern IDEs and online tools \cite{Kumar2021}.
    
    \item \textbf{Emerging Topics:} PD must keep pace with emerging areas such as AI, data science, and cybersecurity, often through specialized workshops and curated reading resources \cite{McGill2024,Grover2024,Hu2023,Marshall2020,Yadav2022}.
    
    \item \textbf{Pedagogical Techniques:} Training should cover approaches to teaching code quality, language transferability, and effective digital resource usage \cite{Izu2025,Tshukudu2021,Munasinghe2021}.
    
    \item \textbf{Accessibility and Inclusion:} Dedicated workshops on digital accessibility, disability etiquette, and inclusive teaching prepare educators to foster more equitable classrooms \cite{Parthasarathy2024}.
    
    \item \textbf{Ethics in Computing:} PD should also cover CS ethics, including algorithmic bias and social implications of technology, empowering educators to handle such topics confidently \cite{Hu2023}.
\end{itemize}

\subsubsection*{Optimizing Training Delivery and Support Systems}
Resource constraints, scheduling issues, and diverse teaching environments necessitate PD models that are adaptable and well-supported.

\begin{itemize}
    \item \textbf{Flexible and Scalable Delivery:} Blended formats, such as MOOCs combined with occasional in-person sessions, increase reach and adaptability \cite{Jetzinger2024,Tsan2022,Perlman2021,Minnes2022}. For example, TA training modules hosted on Canvas provide low-cost, accessible learning in under-resourced contexts \cite{Zaman2023,Riese2022}.
    
    \item \textbf{Just-in-Time Support:} Brief pedagogical tips offered to TAs before tutoring sessions have proven effective in enhancing teaching strategies \cite{Cheng2024}.
    
    \item \textbf{Clear Documentation and Resources:} Streamlined instructions with embedded examples, tutorial videos, and handbooks reduce cognitive load and improve PD usability \cite{McGill2023}.
    
    \item \textbf{Technical Assistance:} Pre-session tech checks and live help desks ensure that technical barriers do not hinder participation \cite{Jocius2021,Skuratowicz2021}.
    
    \item \textbf{Incentives and Recognition:} Monetary compensation, certification, and PD credits increase motivation and retention among participants \cite{Everson2022,Flatland2022,Wilde2024}.
    
    \item \textbf{Feedback and Data-Driven Refinement:} Diagnostic tools help identify learning gaps and tailor content accordingly \cite{McGill2024}. Participant feedback ensures iterative improvement in both content and delivery \cite{Zaman2023,Kussmaul2022}.
\end{itemize}

\subsection{Remedies for Socio-cultural Challenges}

Socio-cultural challenges in computing education stem from entrenched inequities, systemic biases, and the diverse cultural, linguistic, and socioeconomic backgrounds of learners. Addressing these challenges requires multi-pronged efforts focused on equity, inclusion, and cultural responsiveness across curriculum design, pedagogy, educator training, and student engagement.

\subsubsection*{Promoting Diversity, Equity, and Inclusion (DEI)}

\begin{itemize}
    \item \textbf{Culturally Responsive and Sustaining Education:} Curricula and professional development initiatives increasingly integrate culturally responsive pedagogies that connect computing content with students’ lived experiences, interests, and community contexts \cite{Hill2021,Venn-Wycherley2020,Hwang2023,Hamouda2025,Wilde2024}. Strategies include using local languages, culturally relevant examples, and storytelling to contextualize learning \cite{Hamouda2025}.
    
    \item \textbf{Addressing Bias and Stereotypes:} TA training programs now include modules on implicit bias, stereotype threat, and inclusive communication. These encourage the use of inclusive examples, language, and reflective practice to foster equitable interactions \cite{Huang2023,Simmonds2021}.
    
    \item \textbf{Broadening Participation:} National and grassroots initiatives (e.g., CS for All) work to expand access to computing education in underrepresented communities, particularly rural and low-income regions. These programs emphasize recruiting diverse educators, supporting high-needs schools, and reducing financial barriers \cite{Hill2021,Flatland2022,Nugent2022,Weintrop2022}.
    
    \item \textbf{Integrating Ethics and Societal Impact:} Embedding discussions on ethics, bias, and computing’s societal implications—especially regarding AI—is used to engage students in critical reflection, foster civic responsibility, and highlight CS as a tool for social good \cite{Grover2024,Lee2022,Mahon2024,Hu2023,Rosenbloom2023,Yadav2022}.
\end{itemize}

\subsubsection*{Fostering Inclusive Learning Environments}

\begin{itemize}
    \item \textbf{Building Community and Connection:} Teacher and TA communities of practice help reduce professional isolation and foster collaborative learning environments. International peer programs like TeachNow help students build cross-cultural connections and motivation \cite{DiPaola2023,Perlman2021,Flatland2022,Malik2024}.
    
    \item \textbf{Promoting Collaboration and Peer Support:} Techniques like pair programming support cooperative learning, help reduce isolation, and empower marginalized groups such as girls to participate more actively \cite{Hamouda2025,Sentance2021}.
    
    \item \textbf{Addressing Individual Needs and Power Dynamics:} Training for TAs and tutors includes raising awareness about implicit bias, power imbalances, and student comfort in help-seeking. Anonymous support systems further alleviate intimidation \cite{Markel2021}.
    
    \item \textbf{Flexible and Contextualized Learning:} Instructional materials tailored to local culture, student interests, and diverse attainment levels—coupled with tangible computing resources—support engagement among all learners, including those initially disengaged \cite{Venn-Wycherley2020,Hwang2023,Hamouda2025}.
\end{itemize}

\subsubsection*{Adapting to Cultural and Linguistic Diversity}

\begin{itemize}
    \item \textbf{Culturally Contextualized Materials:} Integrating students' cultural heritage into programming tasks—through the use of culturally grounded themes and local languages—enhances student engagement and representation \cite{Hamouda2025}.
    
    \item \textbf{Training for Cultural Competency:} Professional development for international and domestic TAs includes language support (intonation, stress, clarity) and cross-cultural communication strategies to foster effective teaching \cite{Zaman2023}.
    
    \item \textbf{Bridging Disciplinary Interpretations:} Interdisciplinary teaching (e.g., in data science) benefits from collaborative dialogue and the establishment of shared conceptual frameworks to bridge communication across domains \cite{Marshall2020}.
    
    \item \textbf{Challenging Societal Misconceptions:} Efforts to reshape public perceptions of computing as inclusive, creative, and socially relevant help widen participation and break stereotypes about who belongs in CS \cite{Repenning2021}.
\end{itemize}

\subsection{Remedies for Sense of Community/Belonging Challenges}

A strong sense of community and belonging is crucial for both students and educators in computer science (CS), fostering motivation, reducing isolation, and supporting learning. Challenges often arise from the solitary nature of programming, lack of diverse representation, and traditional teaching structures.

\subsubsection*{Cultivating Supportive Communities for Educators}

Many CS teachers and TAs, especially those in K-12 settings, often work in isolation. Building a strong professional community is vital for their support and growth.

\textbf{Professional Learning Communities (PLCs)}: Establishing robust PLCs is a central remedy. These communities provide structured and ongoing opportunities for teachers and college faculty to connect, share ideas, resources, and discuss challenges 
\cite{Flatland2022,Kussmaul2022,Perlman2021,Ni2021,Hill2021,Tsan2022,Lee2022,Nugent2022,Yadav2022,Wilde2024}. This includes:
\begin{itemize}
    \item \textit{Regular Meetings}: Bi-weekly or monthly meetings, both in-person and virtual, foster consistent interaction and peer support \cite{Flatland2022,Marshall2020,Nugent2022,Wilde2024,Jetzinger2024}.
    \item \textit{Shared Spaces}: Utilizing online platforms like Slack or discussion forums (e.g., in Canvas) provides virtual spaces for ongoing dialogue and support \cite{Jocius2021,Nugent2022,Lee2022}.
    \item \textit{Collaborative Activities}: Co-creating curricula or resources within these communities strengthens bonds and fosters a shared sense of accomplishment \cite{DiPaola2023,Lehtimki2022,Musaeus2024}.
\end{itemize}

\textbf{Mentorship and Peer Support}: Pairing novice TAs with experienced mentors enables observation, feedback, and informal knowledge transfer. Formal mentorship programs also offer sustained guidance and reduce professional isolation \cite{Markel2021,Riese2021,Riese2022,Wilde2024}.

\textbf{Structured Training Programs}: Well-designed TA training programs that include community-building components (e.g., collaborative lesson planning, peer reflections) help foster shared professional identity and belonging \cite{Riese2022,Minnes2022,Akhmetov2024,Haglund2024,Huang2023}.

\textbf{Broadening Networks}: Encouraging participation in CS teacher associations (e.g., CSTA) and academic conferences helps educators expand their networks, particularly benefiting those in rural or isolated contexts \cite{Flatland2022,Ni2021}.

\textbf{Institutional Recognition}: Institutional efforts to cultivate community (e.g., shared teaching initiatives, interdisciplinary collaborations) enhance faculty cohesion and job satisfaction \cite{Vahid2024}. Open Educational Resources (OER) platforms also facilitate connection and visibility among contributors \cite{Fowler2023}.

\subsubsection*{Fostering Belonging for Students}

Students, particularly those from underrepresented backgrounds, may struggle to feel a sense of belonging in CS. Inclusive pedagogical and community-building strategies are vital.

\textbf{Culturally Responsive Pedagogy}: Teaching practices that affirm students' cultural identities and integrate their lived experiences into computing instruction promote deeper engagement and a stronger sense of connection \cite{Hamouda2025,Hwang2023,Rosenbloom2023}.

\textbf{Promoting Collaboration}: Small cohort models and interactive formats (e.g., pair programming, group projects) encourage interpersonal connections and a peer-supportive environment 
\cite{Brunelle2022,Vahid2024,Hamouda2025,Luxton-Reilly2023}.

\textbf{Inclusive Classroom Climate}: A “climate-first” orientation in TA training ensures inclusive language use, active listening, and responsiveness to microaggressions, fostering a respectful and welcoming environment \cite{Huang2023}.

\textbf{Personalized Support and Connection}: One-on-one guidance through tools like TeachNow bridges isolation in digital learning, providing students with individualized support and emotional connection \cite{Malik2024}.

\textbf{Destigmatizing Mistakes}: Encouraging growth mindset practices—such as viewing errors as opportunities for learning (e.g., through debugging)—reduces anxiety and boosts participation \cite{Macann2023}.

\textbf{Connecting with the Broader CS Community}: Events linking students with industry professionals and external mentors foster a sense of inclusion within the global CS community and build confidence \cite{Venn-Wycherley2020,Samarasekara2023,Wilde2024}.

\textbf{Transparent and Supportive Instruction}: Strong teacher-student relationships, built on clear communication and sincere encouragement, improve student retention and foster a welcoming classroom culture \cite{Vahid2024,Zaman2023}.


\subsection{Remedies for Parental and Community Involvement Challenges}

Effective Computer Science (CS) education extends beyond classroom walls and thrives through active engagement with parents, communities, and industry stakeholders. Overcoming barriers such as limited parental awareness, insufficient community buy-in, and weak industry collaboration is essential for building robust and sustainable CS education programs.

\subsubsection*{Increasing Awareness and Gaining Buy-in}

\textbf{Public Awareness Campaigns:} Designing and executing targeted campaigns via social media and print (e.g., zines, flyers) helps raise awareness of CS and AI literacy, encouraging engagement from policymakers, parents, and the public \cite{DiPaola2023}.

\textbf{Educating Parents and Communities:} Outreach efforts to educate families about the value and application of CS—particularly its connections to employment and general life skills—can be facilitated through online learning modules and informational programs \cite{Samarasekara2023,Yadav2022}.

\textbf{Early and Widespread Exposure:} Making CS compulsory from early secondary levels (e.g., Year 7) increases exposure across gender and socioeconomic lines, enabling broader understanding and acceptance of CS as a viable academic and career path \cite{Williams2020}.

\textbf{Promoting Program Outcomes:} Showcasing student capstone projects—especially those involving industry partners—can improve public visibility, strengthen credibility, and build enthusiasm among community stakeholders \cite{Hooshangi2025}.

\subsubsection*{Fostering Collaboration and Partnerships}

\textbf{Industry Collaboration:} Including professionals as project mentors, guest lecturers, or “Professors of Practice” fosters industry-relevant curriculum alignment and bridges academic-industry gaps \cite{Hooshangi2025,Lee2021,Parthasarathy2024}.

\textbf{Community Partnerships:} Sustained engagement with local organizations and activists helps contextualize CS within real-world challenges (social, environmental, political), promoting culturally responsive pedagogy \cite{Rosenbloom2023,Yadav2022}.

\textbf{School–College Partnerships:} Establishing joint initiatives between K-12 institutions and universities supports teacher development and combats educator isolation through shared training, coursework, and events \cite{Flatland2022}.

\textbf{Alumni Engagement:} Recruiting alumni as adjunct instructors or mentors offers dual benefits: staffing support and firsthand industry feedback. Alumni involvement also contributes to recreating a small-class mentoring atmosphere \cite{VanDeGrift2023}.

\textbf{Volunteer Programs:} Initiatives such as \textit{CS in Schools} pair tech professionals with school teachers, offering co-teaching, real-time student support, and professional development within classrooms \cite{Williams2020}.

\subsubsection*{Engaging Parents in Student Learning}

\textbf{Home-Based Resources:} Providing materials such as computational thinking (CT) exercise books enables students and parents to collaborate at home, extending learning beyond the classroom \cite{Lehtimki2022}.

\textbf{Facilitating Communication:} Surveys and formal parent–teacher meetings can help teachers understand students’ socio-economic and cultural contexts. Inviting family members to share CS-related experiences in class also enhances community connection \cite{Hwang2023}.

\textbf{Navigating Cultural Sensitivities:} When CS activities intersect with cultural norms or prohibitions, educators are encouraged to offer sensitive alternatives and foster mutual respect \cite{Hamouda2025}.

\textbf{Community Events:} Organizing events such as hackathons or community breakfasts promotes equity-oriented CS education, strengthens familial understanding, and builds inclusive networks around CS classrooms \cite{Hill2021}.

\vspace{0.5em}
By leveraging these multidimensional strategies, CS educators can cultivate a more integrated ecosystem—uniting schools, families, industry, and communities to ensure holistic and equitable computing education.



related work:


\subsection{Prior Work on CS Educators}


Research in computer science education (CSEd) has increasingly focused on supporting CS educators across educational levels. Prior work highlights several thematic areas, including professional development (PD), community support, teacher confidence and identity, tutor training, integration of emerging content areas, and the iterative development of teaching tools.

\subsubsection{Professional Development}

Effective professional development (PD) in CSEd is not simply about one-off workshops or knowledge transfer—it is increasingly framed as a structured, sustained, and community-centered process. Longitudinal and hands-on models have demonstrated greater efficacy than brief interventions \cite{Kussmaul2022,Flatland2022,Nugent2022}. For instance, Nugent et al.\ implemented a 100-hour K–8 PD program integrating CS content and pedagogy through graduate-level courses, Saturday workshops, and hands-on robotics activities. These sessions emphasized active learning and teacher collaboration, functioning as communities of practice that broke professional isolation and enhanced teachers’ CS self-efficacy and instructional skill \cite{Nugent2022}. Flatland et al.\ described multi-year college/high school partnerships where teachers receive extensive support through summer PD, coursework (up to 12 credits), and bi-monthly community-building events, fostering sustained engagement and reducing isolation in rural districts \cite{Flatland2022}. Shanley et al.\ introduced a five-week asynchronous PD for APCSA teachers, emphasizing flexible access and integrating expert video content, autograders like CodeWorkout and CodeCheck, and modules on pedagogy and online instruction. Participants reported statistically significant gains in both content knowledge and instructional confidence \cite{Shanley2023}. Kussmaul et al.\ piloted a virtual, diffuse-schedule PD for K–8 teachers that combined weekly synchronous sessions with asynchronous collaborative coding activities. The virtual format increased accessibility, and structured peer interaction built community and deepened engagement \cite{Kussmaul2022}.

Beyond content delivery, a growing body of literature highlights the importance of reflective practice and educator co-design. DiPaola et al.'s \textit{AI Educator Make-a-Thon} exemplifies this, emphasizing process-oriented design and professional identity development over deployable outcomes. The Make-a-Thon positioned teachers as co-designers alongside AI experts, cultivating a sense of belonging and agency in the AI education community \cite{DiPaola2023}. More broadly, PD efforts increasingly incorporate reflective teaching practices such as self-assessment diagnostics, critical vignettes, and culturally responsive review. These structures help teachers recognize pedagogical blind spots and navigate the complexity of real-time instructional decisions \cite{Tsan2022}.

Industry-education partnerships also offer a promising model. The \textit{CS in Schools} initiative in Australia addresses teacher shortages by pairing computing professionals with teachers in a two-pass co-teaching model across six months. Teachers begin by observing, then gradually assume instructional leadership with support from mentors and scaffolded resources. The program has yielded notable improvements in teacher confidence and classroom autonomy \cite{Williams2020}.

Faculty development in emerging content areas follows similar trends of iteration, peer collaboration, and course integration. In inclusive software design, Patel et al.\ conducted summer workshops for faculty on the GenderMag method, followed by collaborative curriculum development and ongoing support to enable low-barrier integration of inclusive practices into computing courses \cite{Patel2024}. For AI education, Grover et al.\ promote curricular co-design and learning-by-doing through PD formats such as the Teacher-Learner-Observer (TLO) model and the AI Book Club—a 20-hour, community-based PD featuring hands-on learning, ethical AI discussions, and collaborative adaptation of materials for classrooms \cite{Grover2024}. In data science, Marshall et al.\ applied a two-phase PD model: an intensive learner retreat followed by a year-long educator support phase involving consultations and seminars. Faculty participants reported deeper conceptual understanding, confidence in customizing content, and strong peer networks that sustained implementation beyond the PD period \cite{Marshall2020}.

Across these initiatives, effective professional development is distinguished by its sustained nature, alignment with authentic teaching contexts, collaborative design processes, and emphasis on teacher agency. Whether in foundational K–12 education or in emerging areas such as AI and data science, the most successful PD models treat teachers as reflective practitioners and co-creators of curriculum—not passive recipients of prescribed knowledge.


% \subsubsection{Community and Support Systems}

% Community building is a critical dimension of educator support, fostering environments where teachers can collaborate, share experiences, and receive mutual encouragement. Programs that integrate structured peer interactions—such as weekly TA meetings at UC Berkeley \cite{Huang2023} or co-creation workshops for computational thinking resources \cite{Yadav2022}—foster communities of practice that extend beyond isolated events. The Make-a-Thon event, for example, culminated a year-long PD program that intentionally cultivated a sense of belonging and collaborative spirit \cite{DiPaola2023}.

% Several initiatives exemplify formalized peer interaction and mentoring. The CS-orona project in Israel, launched during the COVID-19 pandemic, successfully enabled teachers to fulfill psychological needs for belonging and esteem by fostering a strong community of practice through peer-led Zoom presentations and shared resources. Similarly, the CS in Schools program in Australia supports teachers via a vibrant Slack-based community, while the Computer Science for San Antonio (CS4SA) initiative promotes collaboration through monthly workshops and mentoring \cite{Williams2020}. The Process Oriented Guided Inquiry Learning (POGIL) project also builds instructor support communities through structured peer and mentor meetings.

% TeachNow, a spontaneous 1:1 help system in MOOCs, was found to double as a platform for community building, bridging isolation across continents by facilitating connections among like-minded educators. Instructors involved in the CS1 ``common course'' pilot described bi-weekly meetings as the most valuable part of the experience, underscoring the role of recurring interaction in reducing feelings of isolation.

% Online professional development (PD) programs have also prioritized community-building. The Virtual Pivot PD for computational thinking created teacher communities through creative engagement strategies such as ``party packs'' and themed Zoom rooms, while a virtual elementary CT PD used structured digital tools and informal sessions to foster collaboration. In TA development programs, structured community environments are shown to play a vital role in both pedagogical development and job satisfaction, with initiatives adopting a ``climate-first'' approach to embed inclusivity and peer connection in the training design \cite{Huang2023}.

% Cross-institutional initiatives such as Open Educational Resources (OERs) and collaborative platforms like \textit{CS Materials} serve dual purposes: enabling evidence-based course design and supporting professional communities through shared contributions and public attribution \cite{Blanchard2022,Fowler2023}. Educators contributing to OERs have emphasized the importance of interaction, searchability, and recognition. Similarly, the ``disciplinary commons'' approach for capstone courses has been proposed to strengthen identity and knowledge-sharing across institutions.

% The AI Book Club and the Make-a-Thon event are further examples of community-oriented PD models that foster sustained engagement among educators, researchers, and organizational partners in AI education. Other platforms, like GreenSoft, aim to expand professional networks by actively encouraging educator participation in green computing and sustainability-focused communities.

% Despite such innovations, challenges persist. Many CS educators remain the sole representative of their subject in their schools, lacking both departmental support and daily collegial interaction, particularly in emerging areas like AI education. This persistent isolation underscores the importance of intentional, well-structured efforts to cultivate professional community in CS education.

% \subsubsection{Teacher Confidence and Identity}

% Boosting teacher confidence and strengthening professional identity remain key concerns in CS education, especially for women and primary-level teachers who often report lower self-efficacy in teaching computing concepts \cite{Vivian2020,Ni2021}. Many educators feel they do not belong to the CS teaching community or question their competence, highlighting the need for targeted support structures.

% A variety of empirical strategies have been developed to measure and support teacher identity and confidence. Instruments such as the ``CS Pedagogical Confidence'' scale assess instructors' confidence in teaching diverse student populations using research-based methods, while surveys tracking factors such as commitment to CS teaching, engagement skills, and belongingness help identify needs for targeted intervention \cite{McGill2023,Thigpen2024}. The adapted Teacher CS Self-Esteem scale, for instance, found that female and primary-level teachers score significantly lower than their male and secondary-level counterparts, pointing to specific groups needing sustained support.

% Structured and sustained PD models have demonstrated efficacy in improving teacher identity and confidence. The Make-a-Thon program significantly increased participants’ self-efficacy as AI curriculum designers, empowering them to lead rather than simply implement curricular change \cite{DiPaola2023}. TeachNow provided impactful on-demand teaching opportunities, with the majority of participants rating it as transformative for their development.

% Programs like CS4SA, which offer long-term PD and college coursework for certification, report measurable increases in content mastery and confidence. Similarly, the K–8 PD model demonstrated growth in CS content knowledge and teaching confidence across diverse demographics. Notably, rural teachers showed greater gains in self-efficacy, illustrating the value of targeted interventions in underserved regions.

% Other interventions include School Support Visits (SSVs) featuring individualized coaching and the Teacher-Learner-Observer (TLO) model, which are designed to uplift confidence levels—especially for teachers starting from a lower baseline. The co-creation of CT resources in Ireland led to pre-service teachers expressing high comfort and readiness to teach CT, evidencing the power of collaborative learning in shaping identity.

% Additional efforts such as debugging-focused PD using strategies like ``WHAT?!? A MESS'' help build teacher efficacy in specific domains. PD formats such as the AI Book Club combine cognitive scaffolding and community support, allowing educators to openly express learning difficulties and receive peer-based reassurance. Similarly, mandatory CS modules for Swiss pre-service primary teachers increased comfort with programming and computing concepts, reinforcing the importance of foundational preparation.

% Ultimately, teachers with higher self-efficacy adopt more integrative and student-centered teaching approaches, while those with lower confidence tend to revert to traditional, less adaptive methods. Enhancing teacher identity and confidence, therefore, emerges as a critical lever for improving the overall quality and inclusiveness of CS instruction.

\subsubsection{Community and Support Systems}
Community building is a critical dimension of educator support, fostering environments where teachers can collaborate, share experiences, and receive mutual encouragement. Programs that integrate structured peer interactions—such as weekly TA meetings at UC Berkeley \cite{Huang2023} or co-creation workshops for computational thinking resources \cite{Yadav2022}—foster communities of practice that extend beyond isolated events. The Make-a-Thon event, for example, culminated a year-long PD program that intentionally cultivated a sense of belonging and collaborative spirit \cite{DiPaola2023}.

Several initiatives exemplify formalized peer interaction and mentoring. The CS-orona project in Israel, launched during the COVID-19 pandemic, successfully enabled teachers to fulfill psychological needs for belonging and esteem by fostering a strong community of practice through peer-led Zoom presentations and shared resources. Similarly, the CS in Schools program in Australia supports teachers via a vibrant Slack-based community, while the Computer Science for San Antonio (CS4SA) initiative promotes collaboration through monthly workshops and mentoring \cite{Williams2020}. The Process Oriented Guided Inquiry Learning (POGIL) project also builds instructor support communities through structured peer and mentor meetings\todo{missing citation}.

TeachNow, a spontaneous 1:1 help system in MOOCs, was found to double as a platform for community building, bridging isolation across continents by facilitating connections among like-minded educators \todo{cite}. Instructors involved in the CS1 ``common course'' pilot described bi-weekly meetings as the most valuable part of the experience, underscoring the role of recurring interaction in reducing feelings of isolation \todo{cite}.

Online professional development (PD) programs have also prioritized community-building. The Virtual Pivot PD for computational thinking created teacher communities through creative engagement strategies such as ``party packs'' and themed Zoom rooms, while a virtual elementary CT PD used structured digital tools and informal sessions to foster collaboration \todo{cite}. In TA development programs, structured community environments are shown to play a vital role in both pedagogical development and job satisfaction, with initiatives adopting a ``climate-first'' approach to embed inclusivity and peer connection in the training design \cite{Huang2023}.

Cross-institutional initiatives such as Open Educational Resources (OERs) and collaborative platforms like \textit{CS Materials} serve dual purposes: enabling evidence-based course design and supporting professional communities through shared contributions and public attribution \cite{Blanchard2022,Fowler2023}. Educators contributing to OERs have emphasized the importance of interaction, searchability, and recognition. Similarly, the ``disciplinary commons'' approach for capstone courses has been proposed to strengthen identity and knowledge-sharing across institutions.

The AI Book Club \todo{cite}, similar to Make-a-Thon \todo{cite}, is another example of community-oriented PD model that fosters sustained engagement among educators, researchers, and organizational partners in AI education. Other platforms, like GreenSoft \todo{cite}, aim to expand professional networks by actively encouraging educator participation in green computing and sustainability-focused communities.

Despite such innovations, challenges persist. Many CS educators remain the sole representative of their subject in their schools, lacking both departmental support and daily collegial interaction, particularly in emerging areas like AI education \todo{cite}. This persistent isolation underscores the importance of intentional, well-structured efforts to cultivate professional community in CS education.

\subsubsection{Teacher Confidence and Identity}

Boosting teacher confidence and strengthening professional identity remain key concerns in CS education, especially for women and primary-level teachers who often report lower self-efficacy in teaching computing concepts \cite{Vivian2020,Ni2021}. Many educators feel they do not belong to the CS teaching community or question their competence, highlighting the need for targeted support structures \todo{cite}.

A variety of empirical strategies have been developed to measure and support teacher identity and confidence. Instruments such as the ``CS Pedagogical Confidence'' scale assess instructors' confidence in teaching diverse student populations using research-based methods, while surveys tracking factors such as commitment to CS teaching, engagement skills, and belongingness help identify needs for targeted intervention \cite{McGill2023,Thigpen2024}. The adapted Teacher CS Self-Esteem scale \todo{cite}, for instance, found that female and primary-level teachers score significantly lower than their male and secondary-level counterparts, pointing to specific groups needing sustained support.

Structured and sustained PD models have demonstrated efficacy in improving teacher identity and confidence. The Make-a-Thon program significantly increased participants’ self-efficacy as AI curriculum designers, empowering them to lead rather than simply implement curricular change \cite{DiPaola2023}. TeachNow provided impactful on-demand teaching opportunities, with the majority of participants rating it as transformative for their development  \todo{cite}.

Programs like Computer Science for San Antonio (CS4SA) in the U.S. \todo{full form and cite}, which offer long-term PD and college coursework for certification, report measurable increases in content mastery and confidence. Similarly, the K–8 PD model demonstrated growth in CS content knowledge and teaching confidence across diverse demographics. Notably, rural teachers showed greater gains in self-efficacy, illustrating the value of targeted interventions in underserved regions \todo{cite}.

Other interventions include School Support Visits (SSVs) featuring individualized coaching and the Teacher-Learner-Observer (TLO) model, which are designed to uplift confidence levels—especially for teachers starting from a lower baseline \todo{cite}. The co-creation of CT resources in Ireland led to pre-service teachers expressing high comfort and readiness to teach CT, evidencing the power of collaborative learning in shaping identity\todo{cite}.

Additional efforts focus on teacher efficacy in specific domains. For example, a debugging-focused PD using strategies like ``WHAT?!? A MESS'' aims to build teacher efficacy in specific domains \todo{fix details and cite}. PD formats such as the AI Book Club combine cognitive scaffolding and community support, allowing educators to openly express learning difficulties and receive peer-based reassurance \todo{cite}. Similarly, mandatory CS modules for Swiss pre-service primary teachers increased comfort with programming and computing concepts, reinforcing the importance of foundational preparation \todo{cite}.

Ultimately, teachers with higher self-efficacy adopt more integrative and student-centered teaching approaches, while those with lower confidence tend to revert to traditional, less adaptive methods. Enhancing teacher identity and confidence, therefore, emerges as a critical lever for improving the overall quality and inclusiveness of CS instruction.


\subsubsection*{Training and Pedagogical Development for Teaching Assistants (TAs) and Tutors}

Teaching Assistants (TAs) and tutors play a critical role in scaling computer science instruction, yet many face considerable challenges stemming from insufficient pedagogical preparation. A recurring issue is the lack of formal training in instructional methods, with TAs often equating lecturing with teaching, struggling to scaffold learning, and providing feedback that is either overly prescriptive or lacks clarity \cite{Krause-Levy2022}. This gap in pedagogical knowledge can negatively affect student engagement, concept acquisition, and retention \todo{cite}. Content knowledge gaps also emerge, especially around complex or subtle topics like parameter passing and aliasing, which hinder grading accuracy and conceptual support. Time pressures due to concurrent academic responsibilities further exacerbate the issue, leading to rushed feedback or limited participation in training \todo{cite}.

Low-quality feedback—such as ambiguous code snippets or non-actionable comments—can confuse students, lowering their motivation and increasing the risk of dropout \todo{cite}. Moreover, inconsistent grading practices, particularly for subjective elements like code quality, are common due to vague rubrics and limited assessment training. Emotional and psychological stress is another compounding factor, with many TAs experiencing low self-efficacy, imposter syndrome, and difficulty managing interpersonal dynamics during peer tutoring or high-pressure sessions. In some countries, international TAs (ITAs) face additional challenges due to linguistic and cultural mismatches, often receiving training focused narrowly on pronunciation while lacking guidance on nuanced classroom interaction or role expectations \todo{cite}.

In response, several institutions have developed comprehensive, structured TA training programs. UC Berkeley’s semester-long “climate-first” course for first-time TAs integrates pedagogical techniques with classroom inclusivity training through weekly group meetings, reflections, and peer observations \cite{Huang2023}. KTH Royal Institute of Technology mandates a formal TA preparation course grounded in the TPACK framework, covering assessment, tutorial planning, and interpersonal challenges \cite{Riese2022}. These efforts are complemented by reflective practices such as journaling and role-playing, which enhance metacognitive awareness and build teaching confidence \todo{cite}. Other universities have adopted term-long Graduate TA (GTA) programs incorporating mentored practicum, Computer Education Research (CER) engagement, and exposure to the Scholarship of Teaching and Learning (SoTL), leading to measurable improvements in teaching self-efficacy and instructional quality \todo{cite}.

Emerging PD models also emphasize on training educators to provide actionable feedback. The "WHAT?!? A MESS" debugging framework and bite-sized scaffolding techniques were also targeted towards TA and tutors (in addition to teachers) as a form of feedback training \todo{check and fix citation}. Just-in-time PD interventions before tutoring sessions have significantly increased TA use of evidence-based strategies and student-centered dialogue. Community cohesion is cultivated through weekly meetings, small-group mentoring, and team-teaching structures that pair novice and experienced TAs, facilitating peer support and social learning \cite{Forden2023}. Programs addressing international TA-specific challenges provide cultural competency training, focusing on interaction styles, intonation, and role clarification within Western educational systems \cite{Zaman2023}.

To address scalability, technological interventions have also been deployed. AI Teaching Assistants (e.g., CodeHelp) offer 24/7 support, alleviating human workload, while Automated Assessment Tools (AATs) expedite feedback loops in large classrooms \todo{cite}. Platforms such as CS Materials and ShellOnYou support structured curriculum mapping and automated practice in shell environments, respectively, promoting evidence-based pedagogy at scale \todo{cite}. 

Finally, specialized PD efforts are emerging to address the implications of AI in CS education. Initiatives like AI Book Clubs and blended MOOC-based programs equip educators with the conceptual and pedagogical skills needed to navigate AI-integrated classrooms \todo{cite}.. These efforts reflect a broader shift toward sustained, scalable, and inclusive PD practices that recognize the multifaceted responsibilities of TAs and tutors in modern CS instruction.

\subsubsection{Teaching the Programming Process}

Recent studies emphasize the importance of teaching not only the outcomes of programming but the entire process—including algorithm formulation, design, and debugging. Tools such as \textit{Solvelets} guide students through multi-step problem solving and emphasize proficiency through feedback minimization rather than correctness alone \cite{Kumar2022}. \textit{Solvelets} present a sequence of scaffolded prompts that lead students from a problem statement to a complete and correct program. Rather than relying on post-hoc diagnostic feedback, Solvelets offer immediate assistance at varying levels of specificity, allowing students to overcome conceptual obstacles without being stuck. These tutors reinforce expert design practices—such as loop planning and conditional structuring—while measuring student proficiency through the number of assist requests rather than correctness alone. The tool is openly available and supports C++ and Java, with detailed student action logs to support instructor analysis.

Other tools also focus on formative, automated feedback. \textit{ShellOnYou}, for example, helps students gain practical Unix command-line skills through individualized, auto-graded exercises that both prevent plagiarism and promote peer learning communities \cite{Berry2022}. Similarly, \textit{SnapCheck} addresses the challenges of assessing interactive, visual programs in Snap! by allowing instructors to specify property-based tests and simulate student interactions, making assessment scalable and timely \cite{Wang2021}.

To address instructional invisibility into student workflows, \textit{CodeProcess Charts} provide visualizations of student coding behavior using fine-grained keystroke data, enabling instructors to identify coding strategies, common pitfalls, and even instances of potential plagiarism \cite{Kirk2022}. Instructors have noted that exposing students to their own development trajectories encourages metacognitive reflection. Likewise, \textit{Storyteller}, an open-source extension for Visual Studio Code, supports the creation of multimedia-rich code playbacks, allowing instructors to annotate and narrate program evolution with videos, screenshots, and questions. This alternative to live coding not only facilitates asynchronous learning but also outperforms traditional textbooks in student preference and accessibility \cite{Forden2023}.

Structured tutoring models are gaining traction as a remedy for unproductive tutoring behaviors. Studies have found that many tutors provide direct solutions rather than promoting conceptual understanding or encouraging students to articulate their problems \cite{Tsan2022}. In response, structured self-reflection prompts and cognitive scaffolding strategies have been introduced to improve the tutoring process. For example, the \textit{WHAT?!? A MESS} debugging scaffold helps novice teachers guide students through identifying bugs in their code without supplying direct fixes \cite{Everson2022}. It prompts students to analyze the intended behavior of the program and explore common error types systematically, while also encouraging peer support through strategies like “three before me.”

AI tutors and teaching assistants are increasingly designed with constraints that prevent them from providing full solutions. Instead, they offer step-by-step natural language or pseudocode guidance and conceptual explanations, aligning more closely with pedagogical goals. This approach is complemented by just-in-time training programs for human tutors, which improve the quality and consistency of support \cite{Cheng2024}.

Together, these tools and strategies represent a shift from product-oriented evaluation to process-oriented instruction—akin to providing students with a GPS navigation system rather than a static map. They illuminate the journey of problem-solving, helping students internalize expert practices while offering instructors unprecedented insight into student learning trajectories.
\subsubsection{Tool and Assessment Development as Iterative Processes}

Effective educational tools and assessments in Computer Science Education (CSEd) are fundamentally not static creations but iterative outcomes shaped through continual educator feedback, expert validation, and technological adaptation. One such example is the development of a diagnostic tool aimed at identifying the professional development (PD) needs of K-12 CS teachers. Initially, this tool faced design issues, such as stress due to unclear expectations and lengthy instructions, with completion times averaging over two hours. Inter-rater agreement among external reviewers was low (43--60\%), revealing the cognitive load and inconsistency challenges. To address these concerns, the tool underwent substantial restructuring: materials were streamlined, and rubric items were reduced from 18 to 13, cutting the completion time in half. Future enhancements include adding auto-scorable vignettes aligned with the CSTA Standards and simplifying the review process by introducing targeted training modules for reviewers on specific teaching dimensions like ``Teach'' and ``Assess'' \cite{McGill2023}.

A parallel diagnostic tool focused on assessing content knowledge among AP Computer Science Principles (AP CSP) teachers also incorporated AI-driven item generation and expert review. Piloted with 18 high school teachers, this tool revealed a preference for raw scores over ranges, motivating refinements in both scoring transparency and eligibility—specifically allowing new CS teachers to participate. Such tools are being adapted to directly inform PD content, aligning closely with instructional needs \cite{Thigpen2024}.

Other innovations like the \textit{UserFlow} dashboard demonstrate the benefits of user-centered design for visualizing student engagement with teaching materials. Its development involved collaboration with CS instructors, instructional designers, and learning analytics experts to ensure the data collected was pedagogically actionable. The system visualizes document interaction across multiple scales—annotations, traversal paths, reading duration, and student profiles—allowing instructors to analyze engagement patterns at macro, meso, and micro levels \cite{Musaeus2024}.

Assessment tools are also evolving to maintain academic integrity while reducing instructor burden. The \textit{Unique Exams Framework} was developed in response to integrity concerns during the COVID-19 pandemic in online learning settings. It generates conceptually identical, personalized exams with lexical or numerical variations, based on a shared skeleton. Each version includes a corresponding answer key, making grading efficient while deterring collaboration or online content sharing. Though preparation time may initially increase, grading overhead remains comparable to traditional exams \cite{Rusak2021}.

Rubrics and AI-powered evaluation tools also reflect iterative development and empirical validation. The General Pedagogical Knowledge (GPK) and Pedagogical Content Knowledge (PCK) rubric, designed to evaluate written tutor responses to programming questions, integrates theoretical models emphasizing coherence, completeness, and representational diversity. Internal validation on 85 TA responses revealed areas for rubric improvement in TA training. External expert interviews highlighted missing aspects, such as teaching strategies and language appropriateness. The rubric is language-agnostic and readily adoptable in diverse CS instruction contexts \cite{Ishizue2024}.

In parallel, advanced program repair tools now blend GPT-based models (e.g., GPT-3.5-Turbo and GPT-4) with symbolic reasoning (e.g., Refactory) to correct student code submissions. These hybrid tools address syntax errors and low-submission scenarios, improving repair success rates by 1--43\% without significantly increasing runtime. This demonstrates the efficacy of integrating LLMs into assessment and feedback systems for scalable instructional support \cite{Ishizue2024}.

\subsubsection{Responding to Emerging Challenges}

The evolving technological landscape, particularly the rise of Generative AI (GenAI), has prompted educators to reassess and redesign pedagogical priorities. With tools like ChatGPT and GitHub Copilot becoming increasingly accessible, the instructional emphasis has shifted from basic code generation to cultivating higher-order thinking skills such as code reading, critique, debugging, and problem decomposition. Educators now stress the importance of requirements formulation—training students to frame precise prompts and critically analyze AI-generated code. This shift also necessitates revised assessment strategies, where the focus moves away from the correctness of final outputs to evaluating students' problem-solving processes and code development journeys \cite{Sheard2024,Lau2023}.

New formats like process-based assessments—grading feature branches, pull requests, or code reviews—are gaining traction as they better reflect real-world software development practices. Additionally, oral assessments and unique local-context assignments are being used to ensure academic integrity. Instructors are even leveraging GenAI to generate assignment variants dynamically, offering novel challenges that deter direct copying. Concurrently, there is an increasing institutional effort to clarify acceptable uses of GenAI and foster student understanding of its affordances and limitations.

Tools like \textit{TA-Bot} exemplify how community-centered development philosophies support such pedagogical shifts. Originally a command-line interface, TA-Bot has been reimagined as a web-based Automated Assessment Tool (AAT) that incorporates dynamic rate-limiting features to encourage early assignment starts and integrates Pylint with beginner-friendly feedback. The tool evolved through iterative feedback from both students and faculty. While instructors valued real-time feedback mechanisms, students perceived some features—like rate-limiting and gamified leveling—as punitive or confusing. These findings underscore the critical role of user perception in iterative tool refinement \cite{Forden2023}.

Another domain undergoing transformation is environmental sustainability. The inclusion of green computing principles in CS curricula has gained traction, driven by collaborations between educators, researchers, and industry stakeholders. Modular, project-based models now support incremental integration of green computing topics from introductory courses (CS1/CS2) to advanced electives. Pedagogical approaches include hands-on labs using tools like RAPL and jStanley to analyze energy efficiency, and cloud-based platforms like GreenCode and GreenSoft to provide virtual labs and community knowledge-sharing hubs. This broader effort requires sustained engagement across academia and industry to periodically reassess and restructure computing curricula in line with sustainability goals \cite{Saraiva2021}.



\subsection{Student-Focused Interventions and Learning Tools}

A growing body of work in Computer Science Education (CS Ed) focuses on developing tools and interventions that enhance student engagement, understanding, and equity. Among these, personalized support systems like \textit{TeachNow} and intelligent tutoring platforms such as \textit{Solvelets} have demonstrated measurable impact in large-scale introductory programming courses \cite{Malik2024,Bassner2024}. \textit{TeachNow} facilitated over 12,000 minutes of tutoring through real-time, spontaneous teacher-student pairings in collaborative online environments, significantly reducing dropout rates and improving student retention by up to 15\%. Meanwhile, \textit{Solvelets} supports learners throughout the entire program development cycle by providing progressively detailed scaffolding and accommodating semantically diverse solutions, which helps reduce plagiarism while encouraging authentic learning practices \cite{Berry2022}.

Interactive platforms such as \textit{ShellOnYou} offer automated feedback for Unix-based command-line skills, enabling students to engage in low-stakes iterative practice with immediate grading. This not only reduces the burden on instructors but also fosters peer engagement and reflection \cite{Su2021}. \textit{DeCode}, a game-based system that teaches Data Structures and Algorithms using a 2.5D "carpark" metaphor, has shown promise in early trials for helping students visualize abstract operations and reinforce their problem-solving skills \cite{Anyango2021}.

Gamification is further leveraged by tools like the \textit{Recursive Game Generator (RGG)} and \textit{SnapCheck}. RGG allows instructors to rapidly prototype games for teaching recursion—a traditionally difficult topic—and was found accessible and valuable by a majority of instructors in pilot studies \cite{Wang2021}. \textit{SnapCheck} automates testing and feedback for Snap! programs, allowing students to iteratively refine their code while receiving nonjudgmental, property-based feedback. This scaffolds systematic testing behaviors and promotes sustained engagement.

Equity-focused initiatives include \textit{CS4SA}, an online PD program designed to broaden Latinx participation in CS and STEM. The program introduces culturally responsive pedagogy and community-connected practices, equipping teachers to design inclusive classroom activities and lead extracurricular STEM engagement \cite{Friend2022}. Universal Design for Learning (UDL)-informed interventions, such as those integrated into assistive technology courses for special education teachers, have improved participants’ ability to adapt computing instruction for learners with disabilities using multiple sensory and physical representations \cite{Weng2021}. Inclusive design principles are increasingly embedded throughout undergraduate computing curricula. Modules based on frameworks like GenderMag encourage students to detect and resolve inclusivity issues in software, fostering sustained awareness and application across the degree pathway \cite{Ko2021}.

\subsection{Building the Field of CS Education}

Significant progress has been made in formalizing Computer Science Education as a scholarly discipline, particularly through the development of diagnostic instruments, professional standards, and shared curriculum models. The Computer Science Teachers Association (CSTA) Standards for Teachers have guided the creation of both artifact-based and multiple-choice diagnostics aligned with competencies in content knowledge, pedagogy, and equity. Piloted with K–12 educators, these tools not only reveal teachers’ strengths and growth areas but also inform personalized professional development trajectories. AI-assisted item generation and expert feedback further enhance the reliability and scalability of such diagnostics \cite{Fowler2023}.

A professional identity survey developed to assess CS teachers’ sense of teaching commitment, pedagogical confidence, and community belonging found strong correlations between identity scores and years of teaching experience \cite{Ni2021}. The findings underscore the importance of targeted support for novice educators, especially those transitioning from other subjects or entering isolated teaching roles.

Curriculum misalignment has been a recurring theme in CS Ed literature, particularly regarding the disconnect between academic instruction and industry expectations. Studies reveal that students often struggle with algorithmic reasoning due to the abstract nature of formalism and lack of real-world contextualization \cite{Luu2023}. Faculty acknowledge the importance of preparing students for collaborative, communicative, and software engineering-oriented roles but cite constraints like large class sizes, outdated syllabi, and limited time as barriers to integrating industry practices into coursework \cite{Ju2020}.

Collaborative course models have emerged to mitigate redundancy and improve scalability. For example, the “common course” framework allows institutions to share core materials, grading infrastructure, and pedagogy, reducing preparation time and encouraging adoption of innovative practices. Instructors across participating universities reported time savings, improved learning outcomes, and stronger alignment with curricular goals. Centralized course models also enable large-scale data analysis for continuous refinement \cite{Denny2024}.

Efforts to support tool discoverability and reuse are ongoing. While many CS Ed tools show strong results in isolated studies, challenges persist around versioning, integration, and long-term maintenance. CS Materials, a repository designed to align educational content with national standards, offers a promising model. However, broader adoption remains limited, prompting calls for a centralized, peer-reviewed repository managed collaboratively by the research community \cite{Vahid2024}.

\subsection{Ongoing Gaps and Opportunities}

Despite the breadth of current research, several persistent gaps continue to constrain the impact of CS Ed innovations. Professional development remains unevenly distributed, with many educators—particularly in under-resourced schools—lacking access to high-quality, sustained training. Elementary teachers and women educators often experience fragile confidence and isolation, highlighting the need for identity-supportive communities and mentorship \cite{Vivian2020,Ni2021}.

The research-practice divide is another critical barrier. Although novel tools and strategies proliferate in the literature, many are underutilized due to usability issues, steep learning curves, or misalignment with institutional constraints. Moreover, few studies evaluate long-term effectiveness or offer models for scaling interventions in diverse educational contexts \cite{Tshukudu2021,Blanchard2022}.

The integration of generative AI in education presents both new possibilities and significant challenges. Tools like ChatGPT and GitHub Copilot can enhance creativity and code generation, but they also necessitate rethinking assessment strategies to prioritize process over output. Emerging practices include oral code reviews, contextualized assignments, and AI-resilient problem designs \cite{Sheard2024}. At the same time, educators are beginning to adopt generative tools for instructional support, using them to create problem variants, simulate code walkthroughs, or generate formative feedback at scale.

Ultimately, the sustainability and inclusivity of CS education reform depend on more than tool development. Longitudinal studies, participatory design approaches, and institutional backing are required to ensure that interventions persist beyond pilot phases and address the needs of all learners. Community-driven research and resource sharing, supported by robust policy frameworks, will be vital in closing equity gaps and maintaining momentum in CS education advancement.




\subsection{Remedies for Training and Professional Development Challenges}

The rapid evolution of computer science (CS) and the growing demand for CS education have intensified training and professional development (PD) challenges for educators at all levels. A significant proportion of teachers and teaching assistants (TAs) lack formal backgrounds in CS or discipline-specific pedagogical training, highlighting the critical need for sustained, accessible, and context-relevant professional learning opportunities.
Common themes of Training and Professional Development Remedies
in our reviewed papers are \textbf{1.Comprehensive and Sustained Training Programs}
Traditional PD formats are often short, generic, or disconnected from classroom realities. To address this, effective remedies emphasize the design of long-term, iterative, and multifaceted PD programs that support continuous learning and reflection.
For example Extended and Iterative PD Models\cite{Tsan2022,Lee2022},\cite{DiPaola2023}\cite{Lee2022},Integrated Content and Pedagogy\cite{Basu2022,Everson2022,Tsan2022,Yadav2022}\cite{Macann2023,Jia2022}\cite{Jetzinger2024},Hands-on and Active Learning\cite{Patel2024,Tsan2022,Skuratowicz2021,Hamouda2025}\cite{DiPaola2023,Musaeus2024,Lehtimki2022,Grover2024},Structured Mentoring and Peer Learning\cite{Kussmaul2022,Minnes2022,Flatland2022,Wilde2024,Haglund2024,Markel2021}\cite{Riese2021}.

\textbf{2.Addressing Specific Knowledge Gaps and Skills}
Educators’ varied backgrounds demand targeted PD interventions that address distinct knowledge and skill deficiencies.
For example Foundational CS Skills\cite{Kumar2021,Everson2022,Flatland2022}\cite{Kumar2021},Emerging Topics such as AI, data science, and cybersecurity\cite{McGill2024,Grover2024,Hu2023,Marshall2020,Yadav2022},Pedagogical Techniques\cite{Izu2025,Tshukudu2021,Munasinghe2021},Accessibility and Inclusion\cite{Parthasarathy2024},Ethics in Computing\cite{Hu2023}.


\textbf{3.Optimizing Training Delivery and Support Systems}
Resource constraints, scheduling issues, and diverse teaching environments necessitate PD models that are adaptable and well-supported.
For example Flexible and Scalable Delivery\cite{Jetzinger2024,Tsan2022,Perlman2021,Minnes2022}\cite{Zaman2023,Riese2022},Just-in-Time Support that is Brief pedagogical tips offered to TAs before tutoring sessions have proven effective in enhancing teaching strategies \cite{Cheng2024},
Clear Documentation and Resources\cite{McGill2023},Technical Assistance\cite{Jocius2021,Skuratowicz2021},Incentives and Recognition\cite{Everson2022,Flatland2022,Wilde2024},Feedback and Data-Driven Refinement\cite{McGill2024}\cite{Zaman2023,Kussmaul2022}.


\subsection{Remedies for Socio-cultural Challenges}

Socio-cultural challenges in computing education stem from entrenched inequities, systemic biases, and the diverse cultural, linguistic, and socioeconomic backgrounds of learners. Addressing these challenges requires multi-pronged efforts focused on equity, inclusion, and cultural responsiveness across curriculum design, pedagogy, educator training, and student engagement.
Common themes of Socio-cultural Remedies
in our reviewed papers are 
\textbf(1.Promoting Diversity, Equity, and Inclusion (DEI)}
For example Culturally Responsive and Sustaining Education\cite{Hill2021,Venn-Wycherley2020,Hwang2023,Hamouda2025,Wilde2024}\cite{Hamouda2025},Addressing Bias and Stereotypes \cite{Huang2023,Simmonds2021},Broadening Participation\cite{Hill2021,Flatland2022,Nugent2022,Weintrop2022},Integrating Ethics and Societal Impact\cite{Grover2024,Lee2022,Mahon2024,Hu2023,Rosenbloom2023,Yadav2022}.


\textbf{2.Fostering Inclusive Learning Environments}

For example Building Community and Connection\cite{DiPaola2023,Perlman2021,Flatland2022,Malik2024}Promoting Collaboration and Peer Support\cite{Hamouda2025,Sentance2021},Addressing Individual Needs and Power Dynamics\cite{Markel2021},Flexible and Contextualized Learning\cite{Venn-Wycherley2020,Hwang2023,Hamouda2025}.


\textbf{3.Adapting to Cultural and Linguistic Diversity}
For example Culturally Contextualized Materials\cite{Hamouda2025},Training for Cultural Competency\cite{Zaman2023},Bridging Disciplinary Interpretations\cite{Marshall2020},
 Challenging Societal Misconceptions\cite{Repenning2021}.


\subsection{Remedies for Sense of Community/Belonging Challenges}

A strong sense of community and belonging is crucial for both students and educators in computer science (CS), fostering motivation, reducing isolation, and supporting learning. Challenges often arise from the solitary nature of programming, lack of diverse representation, and traditional teaching structures.
Common themes of Sense of Community/Belonging Remedies
in our reviewed papers are 
\textbf{1.Cultivating Supportive Communities for Educators}

Many CS teachers and TAs, especially those in K-12 settings, often work in isolation. Building a strong professional community is vital for their support and growth.
For example Professional Learning Communities (PLCs)
\cite{Flatland2022,Kussmaul2022,Perlman2021,Ni2021,Hill2021,Tsan2022,Lee2022,Nugent2022,Yadav2022,Wilde2024} which includes
Regular Meetings\cite{Flatland2022,Marshall2020,Nugent2022,Wilde2024,Jetzinger2024},Shared Spaces like online platforms like Slack or discussion forums like Canvas\cite{Jocius2021,Nugent2022,Lee2022},Collaborative Activities\cite{DiPaola2023,Lehtimki2022,Musaeus2024},Mentorship and Peer Support\cite{Markel2021,Riese2021,Riese2022,Wilde2024},Structured Training Programs e.g., collaborative lesson planning, peer reflections help foster shared professional identity and belonging \cite{Riese2022,Minnes2022,Akhmetov2024,Haglund2024,Huang2023},Broadening Networks such as Encouraging participation in CS teacher associations (e.g., CSTA) and academic conferences helps educators expand their networks, particularly benefiting those in rural or isolated contexts \cite{Flatland2022,Ni2021},Institutional Recognition such as Institutional efforts to cultivate community (e.g., shared teaching initiatives, interdisciplinary collaborations) enhance faculty cohesion and job satisfaction \cite{Vahid2024}. Open Educational Resources (OER) platforms also facilitate connection and visibility among contributors \cite{Fowler2023}.

\textbf{2.Fostering Belonging for Students}

Students, particularly those from underrepresented backgrounds, may struggle to feel a sense of belonging in CS. Inclusive pedagogical and community-building strategies are vital.
For example Culturally Responsive Pedagogy\cite{Hamouda2025,Hwang2023,Rosenbloom2023},Promoting Collaboration
\cite{Brunelle2022,Vahid2024,Hamouda2025,Luxton-Reilly2023},Inclusive Classroom Climate\cite{Huang2023},Personalized Support and Connection\cite{Malik2024},Destigmatizing Mistakes that is encouraging growth mindset practices—such as viewing errors as opportunities for learning (e.g., through debugging)—reduces anxiety and boosts participation \cite{Macann2023},Connecting with the Broader CS Community\cite{Venn-Wycherley2020,Samarasekara2023,Wilde2024},Transparent and Supportive Instruction\cite{Vahid2024,Zaman2023}.


\subsection{Remedies for Parental and Community Involvement Challenges}

Effective Computer Science (CS) education extends beyond classroom walls and thrives through active engagement with parents, communities, and industry stakeholders. Overcoming barriers such as limited parental awareness, insufficient community buy-in, and weak industry collaboration is essential for building robust and sustainable CS education programs.
Common themes of Parental and Community Involvement Remedies
in our reviewed papers are
\textbf{1.Increasing Awareness and Gaining Buy-in}
For example Public Awareness Campaigns such as designing and executing targeted campaigns via social media and print (e.g., zines, flyers) helps raise awareness of CS and AI literacy, encouraging engagement from policymakers, parents, and the public \cite{DiPaola2023},Educating Parents and Communities\cite{Samarasekara2023,Yadav2022},Early and Widespread Exposure such as making CS compulsory from early secondary levels (e.g., Year 7) increases exposure across gender and socioeconomic lines, enabling broader understanding and acceptance of CS as a viable academic and career path \cite{Williams2020},Promoting Program Outcomes\cite{Hooshangi2025}.

\textbf{2.Fostering Collaboration and Partnerships}
For example Industry Collaboration\cite{Hooshangi2025,Lee2021,Parthasarathy2024}Community Partnerships\cite{Rosenbloom2023,Yadav2022},School–College Partnerships\cite{Flatland2022},Alumni Engagement\cite{VanDeGrift2023},Volunteer Programs\cite{Williams2020}.

\textbf{3.Engaging Parents in Student Learning}
For example Home-Based Resources such as providing materials such as computational thinking (CT) exercise books enables students and parents to collaborate at home, extending learning beyond the classroom \cite{Lehtimki2022},Facilitating Communication via Surveys and formal parent–teacher meetings that can help teachers understand students’ socio-economic and cultural contexts. Inviting family members to share CS-related experiences in class also enhances community connection \cite{Hwang2023},Navigating Cultural Sensitivities \cite{Hamouda2025}Community Events\cite{Hill2021}.

\vspace{0.5em}
By leveraging these multidimensional strategies, CS educators can cultivate a more integrated ecosystem—uniting schools, families, industry, and communities to ensure holistic and equitable computing education.




prefinal remedy section:


\subsection{Remedies Implemented for Pedagogical Challenges}

Computer science (CS) education faces a variety of pedagogical challenges, ranging from effectively training instructors and teaching assistants (TAs) to making CS accessible and engaging for diverse student populations. In response, researchers and educators have proposed and implemented a variety of targeted remedies.
Common themes of Pedagogical Remedies in our reviewed papers
are:
\textbf{1.Pedagogical Training for Instructors and TAs}
A significant focus has been on improving the pedagogical skills of CS instructors and TAs, many of whom lack formal training in teaching methodologies, which can hinder student learning \cite{Cook2022,Riese2021,Zaman2023}. Remedies include explicit pedagogical instruction that trains TAs to provide effective, non-prescriptive feedback, identify gaps in understanding, use complete sentences, and ask guiding questions. Strategic use of code snippets (e.g., examples or test cases) is emphasized over direct solutions \cite{Cook2022,Zaman2023}. 
Small-group practicum sessions enable TAs to practice micro-teaching, grading, and discuss classroom scenarios. Experienced TAs act as mentors while new TAs receive observation-based feedback \cite{Minnes2022,Akhmetov2024}. Just-in-time teaching tips—short, actionable tips provided immediately before tutoring sessions—help TAs guide conversations, ask open-ended questions, and diagnose misconceptions \cite{Cheng2024}.\textbf{2.Inclusive and Supportive Classroom Environments}
To remediate classroom climate and inclusivity issues, TA and teacher training now incorporates inclusive practices, focusing on language use, diverse examples, and accessible course content to foster a welcoming environment \cite{Huang2023}.
\textbf{3.Improving Content and Pedagogical Content Knowledge (PCK)}
Instructor development programs address core CS concepts, abstract reasoning, and the adaptation of existing materials \cite{Yadav2022,McGill2024,Everson2022,Kumar2021}. TA training also integrates general pedagogy, PCK, and TPACK models \cite{Riese2022}. 
The Make-a-Thon (MAT) was specifically designed to empower teachers as AI curriculum designers, enabling them to understand, use, modify, and create AI curricula rather than merely implementing pre-written materials. The core of the MAT involved co-design of AI literacy materials, where teachers played a central role in the design process \cite{DiPaola2023}.As part of a faculty development initiative, a Faculty Development Program (FDP) was conducted to demonstrate improved methods for conducting CS1 programming labs. Instructors were provided with hands-on programming tasks from a student’s perspective \cite{Kumar2021}.A diagnostic tool introduced in 2024 aimed to provide targeted professional development (PD) recommendations. This mixed-methods study involved 66 teachers and used submitted classroom artifacts and justifications, alongside a self-assessment instrument aligned with CSTA Standards. While most teachers found the tool helpful, the self-assessment results were largely uncorrelated with diagnostic findings, highlighting possible Dunning-Kruger effects.
\textbf{4.Curriculum Design and Delivery Innovations}
Innovative curriculum strategies seek to enhance student engagement, understanding, and application for example Contextualized and real-world learning\cite{Venn-Wycherley2020,Samarasekara2023,Hamouda2025},Project-based learning\cite{Lee2021,Hooshangi2025,Repenning2021,Hamouda2025},Scaffolded instruction\cite{Vahid2024,Sauerwein2023},Educational technology tools\cite{Mahoney2023,Wang2021},Interdisciplinary modules\cite{Kalathas2022,Hu2023},Visualizing student thought processes\cite{Shrestha2022}.
\textbf{4.Addressing Specific Student Needs and Challenges}
Tailored strategies help support diverse learners and address individual challenges for example Disability support and UDL\cite{Yadav2022,Huff2021},Bridging knowledge gaps\cite{Luu2023,Krause-Levy2022,Krause-Levy2023,Hooshangi2025},Growth mindset through language\cite{Macann2023},Adapting to Generative AI\cite{Mahon2024,Sheard2024,Lau2023}.


\subsection{Remedies Implemented for Assessment and Evaluation Challenges}
Educators in computer science face numerous assessment and evaluation challenges, ranging from ensuring fairness and consistency to effectively gauging complex learning outcomes. A variety of remedies—spanning technological tools, pedagogical practices, and policy interventions—have been proposed and implemented to address these concerns.
Common themes of Assessment and Evaluation Remedies in our reviewed papers are\textbf{1.Enhancing Feedback and Grading Efficiency}
Providing timely, actionable feedback while managing large classes remains a persistent challenge. To address this, educators are leveraging automation and structured assessment practices for example Automated Assessment Systems (APASs)\textit{ShellOnYou}\textit{TA-Bot}\cite{Berry2022,Forden2023,Sauerwein2023}\cite{Vahid2024},Improved autograder feedback\cite{Shanley2023},Rubrics and exemplars\cite{Esche2024,Kirk2022,Hooshangi2025},Code quality tools\cite{Izu2025},Data-driven instructional insights\textit{UserFlow}\textit{Solvelets} \cite{Singh2020,Kumar2022}.\textbf{2.Ensuring Fairness, Consistency, and Academic Integrity}
Fair assessment practices and the rising challenge of AI-based plagiarism require proactive strategies for example Unique and randomized exams\cite{Rusak2021},Multiple assessment modalities\cite{Mahon2024,Hamouda2025,Lau2023,Sheard2024},Process-based assessment\cite{Mahon2024,Sheard2024,Lau2023},Plagiarism detection tools\cite{Forden2023,Shrestha2022},Clear policies on AI usage \cite{Mahon2024,Sheard2024},TA training on academic integrity\cite{Riese2022},Standardized assessments and data pooling\cite{Krause-Levy2023,Vahid2024}.\textbf{3.Developing Comprehensive Assessment Literacy},Improving educators' understanding of assessment principles and practices is essential for effective evaluation for example Professional development for assessment literacy\cite{Basu2022},Targeted diagnostic tools \cite{McGill2024,Thigpen2024},Integrating assessment in course design\cite{Farghally2024,Huang2023},Calibration sessions for subjective grading\cite{Kao2020,Hooshangi2025},Reframing assessment purpose\cite{Basu2022}.These multi-pronged strategies contribute to a more robust, transparent, and equitable assessment framework in computer science education, equipping educators to better evaluate, support, and guide student learning.

\subsection{Remedies Implemented for Classroom Management Challenges}

Effective classroom management is foundational for maintaining a productive and inclusive learning environment in computer science education, particularly amid growing class sizes, evolving technologies, and diverse learner needs. Educators are adopting a combination of technological, pedagogical, and organizational strategies to address these multifaceted challenges.Common themes of Classroom Management challenges in our
reviewed papers are:\textbf{1.Managing Large Class Sizes and Workload}With surging enrollments in CS courses, managing large student cohorts and the associated instructional workload is a pressing concern. Several scalable and supportive approaches are being implemented for exmaple Leveraging TAs and support teams\cite{Mason2024,Akhmetov2024},Automated tools for efficiency\cite{Sauerwein2023,Wang2021,Forden2023,Vahid2024},Scalable course structures\cite{Brunelle2022},Self-contained learning tools\textit{Solvelets}\cite{Kumar2022}.
\textbf{2.Fostering Engagement and Addressing Behavioral Issues}
Classroom management also entails sustaining attention, minimizing disruptions, and promoting constructive collaboration for example Engaging and flexible curricula \cite{Venn-Wycherley2020},Promoting productive collaboration\cite{Berry2022,Huang2023,Musaeus2024},Addressing distractions and unproductive behaviors\cite{Pieper2020},Clear expectations and classroom policies\cite{Vahid2024,Mahon2024}.
\textbf{3.Supporting Diverse Learning Environments and Student Needs}
Adapting classroom practices to accommodate diverse student backgrounds, technical configurations, and learning preferences is essential for example Consistent development environments\cite{Nitta2022},Support for virtual and remote learning\cite{Flatland2022,Skuratowicz2021},Individualized support for varied skill levels\cite{Lee2021,Huff2021},Culturally responsive practices\cite{Rosenbloom2023,Hamouda2025},Professional development for classroom management\cite{Yadav2022,Williams2020}.
By combining automated tools, strategic TA deployment, inclusive pedagogy, and professional development, educators aim to create CS learning environments that are manageable, equitable, and responsive to diverse student needs.

\subsection{Remedies for Emotional and Psychological Challenges}

Emotional and psychological challenges can significantly impact both educators and students in computing education, affecting motivation, confidence, and overall well-being. Addressing these issues often involves fostering supportive environments, building self-efficacy, and adopting empathetic teaching practices.
Common themes of Emotional and Psychological Remedies in our reviewed papers are: 
\textbf{1.Boosting Confidence and Self-Efficacy}
Many educators, especially those new to teaching CS, grapple with feelings of inadequacy, stress, and isolation. Students, too, can experience frustration and low confidence when facing difficult concepts.For exaple Targeted Professional Development (PD) and Training\cite{Vivian2020}\cite{Zaman2023},Building a Supportive Community\cite{Flatland2022,Kussmaul2022,Perlman2021,Jocius2021,Skuratowicz2021,Tsan2022,Lee2022,Wilde2024,Haglund2024}\cite{Minnes2022,Goletti2021,Farghally2024},Co-creation and Collaborative Learning\cite{DiPaola2023,Musaeus2024,Lehtimki2022}\cite{Hamouda2025},Increased Instructor Support and Feedback\cite{Kirk2022}\cite{Cook2022,Zaman2023}\cite{Wang2021},Reduced Workload and Autonomy\cite{Vahid2024}\cite{Akhmetov2024}.
\textbf{2.Addressing Stress, Anxiety, and Emotional Well-being}
Educators and students can experience stress and anxiety due to heavy workloads, imposter syndrome, and emotionally difficult classroom dynamics.
For example Creating Safe and Inclusive Environments\cite{Huang2023}\cite{Krause-Levy2023},Destigmatizing Mistakes\cite{Macann2023}\cite{Berry2022},Flexible and Adaptable Programs\cite{Tsan2022}\cite{Mahoney2023},Direct Support for Mental Health\cite{Farghally2024,Riese2022,Minnes2022},Confronting Difficult Topics\cite{Hu2023,Parthasarathy2024}.

\subsection{Remedies for Technological Challenges}
Technological challenges in computing education are multifaceted, encompassing limited infrastructure, inconsistent access to tools, and difficulties in keeping pace with rapidly evolving technologies such as AI. In response, educators and institutions have adopted several strategic remedies aimed at improving accessibility, reducing technical barriers, and facilitating the meaningful integration of emerging technologies.Common themes of Technological Remedies in our reviewed papers
are:\textbf{1.Providing Accessible and User-Friendly Tools} for example Web-Based and Containerized Environments\cite{Kumar2022,Nitta2022,Forden2023},Low-Cost Devices and Open-Source Tools\cite{Hamouda2025},User-Friendly Interfaces\cite{Wang2021,Forden2023},Living and Centralized Repositories\cite{Grover2024,Blanchard2022,Fowler2023}.
\textbf{2.Addressing Technical Barriers and Infrastructure Gaps} for example Low-Tech and Offline Alternatives\cite{Lehtimki2022}.Remote and Low-Bandwidth Adaptations\cite{Malik2024,Flatland2022,Hamouda2025},Technical Support and Institutional Roles\cite{Jocius2021,Skuratowicz2021,Flatland2022},Technological Pedagogical Training\cite{Riese2021,Riese2022,Williams2020},Automation of Administrative Workflows\cite{Akhmetov2024}.
\textbf{3.Navigating Emerging Technologies (e.g., AI and GenAI)} for example AI Integration for Feedback and Support\cite{Ishizue2024},Prompt Engineering and AI Guardrails\cite{Ishizue2024,Denny2024},Redesigning IDEs for AI-Aware Pedagogy\cite{Lau2023,Cucuiat2024},Addressing Ethical and Bias Concerns\cite{Mahon2024},Unplugged AI Activities\cite{Macann2023,Grover2024}.

\subsection{Remedies for Administrative and Institutional Challenges}

Administrative and institutional challenges in computing education stem from structural constraints such as faculty shortages, funding limitations, rigid curricula, and inconsistent policy support. Overcoming these barriers requires multi-pronged strategies involving staffing reforms, policy development, and sustained institutional support.
Common themes of Administrative and Institutional Remedies in
our reviewed papers are:
\textbf{1. Addressing Staffing Shortages and Workload} for example Hiring Adjuncts and Alumni\cite{VanDeGrift2023},Tiered TA Structures\cite{Akhmetov2024},Automation Tools\cite{Sauerwein2023,Forden2023,Wang2021,Kumar2022},Centralized Course Materials\cite{Vahid2024},Financial Incentives\cite{Everson2022,Yadav2022,Perlman2021}.
\textbf{2. Enhancing Teacher Preparation and Professional Development} for example Expanding Recruitment Pipelines\cite{Weintrop2022},Formal Certification Pathways\cite{Yadav2022,Flatland2022},Scalable PD Models\cite{Jetzinger2024,Tsan2022},Long-Term Institutional Investment\cite{Yadav2022,Flatland2022,Huff2021,Saraiva2021,Hamouda2025},Strategic Alliances\cite{Simmonds2021,Hamouda2025,Friend2022}.
\textbf{3. Curriculum Alignment, Policy, and Institutional Support}for example Standardizing Curricula and Policies\cite{Upadhyaya2020,Jia2022,Vahid2024},Stakeholder Education\cite{Grover2024,Simmonds2021,Parthasarathy2024},Addressing Time Constraints\cite{Kalathas2022,Anyango2021,Mahoney2023},Flexible Curriculum Design\cite{Jia2022,Hwang2023,Brunelle2022,Skuratowicz2021},Recognition for Faculty Contributions\cite{Fowler2023},Policy Development for AI Integration\cite{Mahon2024,Lau2023}.

\subsection{Remedies for Training and Professional Development Challenges}

The rapid evolution of computer science (CS) and the growing demand for CS education have intensified training and professional development (PD) challenges for educators at all levels. A significant proportion of teachers and teaching assistants (TAs) lack formal backgrounds in CS or discipline-specific pedagogical training, highlighting the critical need for sustained, accessible, and context-relevant professional learning opportunities.
Common themes of Training and Professional Development Remedies
in our reviewed papers are \textbf{1.Comprehensive and Sustained Training Programs}Traditional PD formats are often short, generic, or disconnected from classroom realities. To address this, effective remedies emphasize the design of long-term, iterative, and multifaceted PD programs that support continuous learning and reflection.For example Extended and Iterative PD Models\cite{Tsan2022,Lee2022},\cite{DiPaola2023}\cite{Lee2022},Integrated Content and Pedagogy\cite{Basu2022,Everson2022,Tsan2022,Yadav2022}\cite{Macann2023,Jia2022}\cite{Jetzinger2024},Hands-on and Active Learning\cite{Patel2024,Tsan2022,Skuratowicz2021,Hamouda2025}\cite{DiPaola2023,Musaeus2024,Lehtimki2022,Grover2024},Structured Mentoring and Peer Learning\cite{Kussmaul2022,Minnes2022,Flatland2022,Wilde2024,Haglund2024,Markel2021}\cite{Riese2021}.
\textbf{2.Addressing Specific Knowledge Gaps and Skills}
Educators’ varied backgrounds demand targeted PD interventions that address distinct knowledge and skill deficiencies.
For example Foundational CS Skills\cite{Kumar2021,Everson2022,Flatland2022}\cite{Kumar2021},Emerging Topics such as AI, data science, and cybersecurity\cite{McGill2024,Grover2024,Hu2023,Marshall2020,Yadav2022},Pedagogical Techniques\cite{Izu2025,Tshukudu2021,Munasinghe2021},Accessibility and Inclusion\cite{Parthasarathy2024},Ethics in Computing\cite{Hu2023}.\textbf{3.Optimizing Training Delivery and Support Systems}Resource constraints, scheduling issues, and diverse teaching environments necessitate PD models that are adaptable and well-supported.For example Flexible and Scalable Delivery\cite{Jetzinger2024,Tsan2022,Perlman2021,Minnes2022}\cite{Zaman2023,Riese2022},Just-in-Time Support that is Brief pedagogical tips offered to TAs before tutoring sessions have proven effective in enhancing teaching strategies \cite{Cheng2024},
Clear Documentation and Resources\cite{McGill2023},Technical Assistance\cite{Jocius2021,Skuratowicz2021},Incentives and Recognition\cite{Everson2022,Flatland2022,Wilde2024},Feedback and Data-Driven Refinement\cite{McGill2024}\cite{Zaman2023,Kussmaul2022}.


\subsection{Remedies for Socio-cultural Challenges}

Socio-cultural challenges in computing education stem from entrenched inequities, systemic biases, and the diverse cultural, linguistic, and socioeconomic backgrounds of learners. Addressing these challenges requires multi-pronged efforts focused on equity, inclusion, and cultural responsiveness across curriculum design, pedagogy, educator training, and student engagement.
Common themes of Socio-cultural Remedies
in our reviewed papers are 
\textbf{1.Promoting Diversity, Equity, and Inclusion (DEI)}
For example Culturally Responsive and Sustaining Education\cite{Hill2021,Venn-Wycherley2020,Hwang2023,Hamouda2025,Wilde2024}\cite{Hamouda2025},Addressing Bias and Stereotypes \cite{Huang2023,Simmonds2021},Broadening Participation\cite{Hill2021,Flatland2022,Nugent2022,Weintrop2022},Integrating Ethics and Societal Impact\cite{Grover2024,Lee2022,Mahon2024,Hu2023,Rosenbloom2023,Yadav2022}.\textbf{2.Fostering Inclusive Learning Environments}
For example Building Community and Connection\cite{DiPaola2023,Perlman2021,Flatland2022,Malik2024}Promoting Collaboration and Peer Support\cite{Hamouda2025,Sentance2021},Addressing Individual Needs and Power Dynamics\cite{Markel2021},Flexible and Contextualized Learning\cite{Venn-Wycherley2020,Hwang2023,Hamouda2025}.
\textbf{3.Adapting to Cultural and Linguistic Diversity}
For example Culturally Contextualized Materials\cite{Hamouda2025},Training for Cultural Competency\cite{Zaman2023},Bridging Disciplinary Interpretations\cite{Marshall2020},
 Challenging Societal Misconceptions\cite{Repenning2021}.

\subsection{Remedies for Sense of Community/Belonging Challenges}

A strong sense of community and belonging is crucial for both students and educators in computer science (CS), fostering motivation, reducing isolation, and supporting learning. Challenges often arise from the solitary nature of programming, lack of diverse representation, and traditional teaching structures.
Common themes of Sense of Community/Belonging Remedies
in our reviewed papers are 
\textbf{1.Cultivating Supportive Communities for Educators}
Many CS teachers and TAs, especially those in K-12 settings, often work in isolation. Building a strong professional community is vital for their support and growth.
For example Professional Learning Communities (PLCs)
\cite{Flatland2022,Kussmaul2022,Perlman2021,Ni2021,Hill2021,Tsan2022,Lee2022,Nugent2022,Yadav2022,Wilde2024} which includes
Regular Meetings\cite{Flatland2022,Marshall2020,Nugent2022,Wilde2024,Jetzinger2024},Shared Spaces like online platforms like Slack or discussion forums like Canvas\cite{Jocius2021,Nugent2022,Lee2022},Collaborative Activities\cite{DiPaola2023,Lehtimki2022,Musaeus2024},Mentorship and Peer Support\cite{Markel2021,Riese2021,Riese2022,Wilde2024},Structured Training Programs e.g., collaborative lesson planning, peer reflections help foster shared professional identity and belonging \cite{Riese2022,Minnes2022,Akhmetov2024,Haglund2024,Huang2023},Broadening Networks such as Encouraging participation in CS teacher associations (e.g., CSTA) and academic conferences helps educators expand their networks, particularly benefiting those in rural or isolated contexts \cite{Flatland2022,Ni2021},Institutional Recognition such as Institutional efforts to cultivate community (e.g., shared teaching initiatives, interdisciplinary collaborations) enhance faculty cohesion and job satisfaction \cite{Vahid2024}. Open Educational Resources (OER) platforms also facilitate connection and visibility among contributors \cite{Fowler2023}.\textbf{2.Fostering Belonging for Students}
Students, particularly those from underrepresented backgrounds, may struggle to feel a sense of belonging in CS. Inclusive pedagogical and community-building strategies are vital.
For example Culturally Responsive Pedagogy\cite{Hamouda2025,Hwang2023,Rosenbloom2023},Promoting Collaboration
\cite{Brunelle2022,Vahid2024,Hamouda2025,Luxton-Reilly2023},Inclusive Classroom Climate\cite{Huang2023},Personalized Support and Connection\cite{Malik2024},Destigmatizing Mistakes that is encouraging growth mindset practices—such as viewing errors as opportunities for learning (e.g., through debugging)—reduces anxiety and boosts participation \cite{Macann2023},Connecting with the Broader CS Community\cite{Venn-Wycherley2020,Samarasekara2023,Wilde2024},Transparent and Supportive Instruction\cite{Vahid2024,Zaman2023}.


\subsection{Remedies for Parental and Community Involvement Challenges}

Effective Computer Science (CS) education extends beyond classroom walls and thrives through active engagement with parents, communities, and industry stakeholders. Overcoming barriers such as limited parental awareness, insufficient community buy-in, and weak industry collaboration is essential for building robust and sustainable CS education programs.
Common themes of Parental and Community Involvement Remedies
in our reviewed papers are
\textbf{1.Increasing Awareness and Gaining Buy-in}
For example Public Awareness Campaigns such as designing and executing targeted campaigns via social media and print (e.g., zines, flyers) helps raise awareness of CS and AI literacy, encouraging engagement from policymakers, parents, and the public \cite{DiPaola2023},Educating Parents and Communities\cite{Samarasekara2023,Yadav2022},Early and Widespread Exposure such as making CS compulsory from early secondary levels (e.g., Year 7) increases exposure across gender and socioeconomic lines, enabling broader understanding and acceptance of CS as a viable academic and career path \cite{Williams2020},Promoting Program Outcomes\cite{Hooshangi2025}.\textbf{2.Fostering Collaboration and Partnerships}
For example Industry Collaboration\cite{Hooshangi2025,Lee2021,Parthasarathy2024}Community Partnerships\cite{Rosenbloom2023,Yadav2022},School–College Partnerships\cite{Flatland2022},Alumni Engagement\cite{VanDeGrift2023},Volunteer Programs\cite{Williams2020}.
\textbf{3.Engaging Parents in Student Learning}
For example Home-Based Resources such as providing materials such as computational thinking (CT) exercise books enables students and parents to collaborate at home, extending learning beyond the classroom \cite{Lehtimki2022},Facilitating Communication via Surveys and formal parent–teacher meetings that can help teachers understand students’ socio-economic and cultural contexts. Inviting family members to share CS-related experiences in class also enhances community connection \cite{Hwang2023},Navigating Cultural Sensitivities \cite{Hamouda2025}Community Events\cite{Hill2021}.




% \subsection{Remedies Implemented for Assessment and Evaluation Challenges}
% Educators in computer science face numerous assessment and evaluation challenges, ranging from ensuring fairness and consistency to effectively gauging complex learning outcomes. A variety of remedies—spanning technological tools, pedagogical practices, and policy interventions—have been proposed and implemented to address these concerns.
% Common themes of Assessment and Evaluation Remedies in our reviewed papers are\textbf{1.Enhancing Feedback and Grading Efficiency}
%~\cite{Berry2022,Forden2023,Sauerwein2023}~\cite{Vahid2024}~\cite{Shanley2023}~\cite{Esche2024,Kirk2022,Hooshangi2025}~\cite{Izu2025}~\cite{Singh2020,Kumar2022}.\textbf{2.Ensuring Fairness, Consistency, and Academic Integrity}
%~\cite{Rusak2021}~\cite{Mahon2024,Hamouda2025,Lau2023,Sheard2024}~\cite{Mahon2024,Sheard2024,Lau2023}~\cite{Forden2023,Shrestha2022}~\cite{Mahon2024,Sheard2024}~\cite{Riese2022}~\cite{Krause-Levy2023,Vahid2024}.\textbf{3.Developing Comprehensive Assessment Literacy}~\cite{Basu2022}~\cite{McGill2024,Thigpen2024}~\cite{Farghally2024,Huang2023},~\cite{Kao2020,Hooshangi2025},~\cite{Basu2022}.These multi-pronged strategies contribute to a more robust, transparent, and equitable assessment framework in computer science education, equipping educators to better evaluate, support, and guide student learning.

% \subsection{Remedies Implemented for Classroom Management Challenges}

% Effective classroom management is foundational for maintaining a productive and inclusive learning environment in computer science education, particularly amid growing class sizes, evolving technologies, and diverse learner needs. Educators are adopting a combination of technological, pedagogical, and organizational strategies to address these multifaceted challenges.Common themes of Classroom Management challenges in our
% reviewed papers are:\textbf{1.Managing Large Class Sizes and Workload}~\cite{Mason2024,Akhmetov2024}~\cite{Sauerwein2023,Wang2021,Forden2023,Vahid2024}~\cite{Brunelle2022}~\cite{Kumar2022}.
% \textbf{2.Fostering Engagement and Addressing Behavioral Issues}
%~\cite{Berry2022,Huang2023,Musaeus2024}~\cite{Pieper2020},Clear expectations and classroom policies~\cite{Vahid2024,Mahon2024}.
% \textbf{3.Supporting Diverse Learning Environments and Student Needs}
%~\cite{Nitta2022},~\cite{Flatland2022,Skuratowicz2021}~\cite{Lee2021,Huff2021}~\cite{Rosenbloom2023,Hamouda2025}~\cite{Yadav2022,Williams2020}.
% By combining automated tools, strategic TA deployment, inclusive pedagogy, and professional development, educators aim to create CS learning environments that are manageable, equitable, and responsive to diverse student needs.

% \subsection{Remedies for Emotional and Psychological Challenges}

% Emotional and psychological challenges can significantly impact both educators and students in computing education, affecting motivation, confidence, and overall well-being. Addressing these issues often involves fostering supportive environments, building self-efficacy, and adopting empathetic teaching practices.
% Common themes of Emotional and Psychological Remedies in our reviewed papers are: 
% \textbf{1.Boosting Confidence and Self-Efficacy}
%~\cite{Vivian2020}~\cite{Zaman2023}~\cite{Flatland2022,Kussmaul2022,Perlman2021,Jocius2021,Skuratowicz2021,Tsan2022,Lee2022,Wilde2024,Haglund2024}~\cite{Minnes2022,Goletti2021,Farghally2024}~\cite{DiPaola2023,Musaeus2024,Lehtimki2022}~\cite{Hamouda2025}~\cite{Kirk2022}~\cite{Cook2022,Zaman2023}~\cite{Wang2021}~\cite{Vahid2024}~\cite{Akhmetov2024}.
% \textbf{2.Addressing Stress, Anxiety, and Emotional Well-being}
%~\cite{Huang2023}~\cite{Krause-Levy2023},~\cite{Macann2023}~\cite{Berry2022}~\cite{Tsan2022}~\cite{Mahoney2023}~\cite{Farghally2024,Riese2022,Minnes2022}~\cite{Hu2023,Parthasarathy2024}.

% \subsection{Remedies for Technological Challenges}
% Technological challenges in computing education are multifaceted, encompassing limited infrastructure, inconsistent access to tools, and difficulties in keeping pace with rapidly evolving technologies such as AI. In response, educators and institutions have adopted several strategic remedies aimed at improving accessibility, reducing technical barriers, and facilitating the meaningful integration of emerging technologies.Common themes of Technological Remedies in our reviewed papers
% are:\textbf{1.Providing Accessible and User-Friendly Tools}~\cite{Kumar2022,Nitta2022,Forden2023}~\cite{Hamouda2025},~\cite{Wang2021,Forden2023},~\cite{Grover2024,Blanchard2022,Fowler2023}.
% \textbf{2.Addressing Technical Barriers and Infrastructure Gaps} f~\cite{Lehtimki2022}~\cite{Malik2024,Flatland2022,Hamouda2025}~\cite{Jocius2021,Skuratowicz2021,Flatland2022},Technological Pedagogical Training~\cite{Riese2021,Riese2022,Williams2020}~\cite{Akhmetov2024}.
% \textbf{3.Navigating Emerging Technologies (e.g., AI and GenAI)}~\cite{Ishizue2024},~\cite{Ishizue2024,Denny2024},~\cite{Lau2023,Cucuiat2024},~\cite{Mahon2024},~\cite{Macann2023,Grover2024}.

% \subsection{Remedies for Administrative and Institutional Challenges}

% Administrative and institutional challenges in computing education stem from structural constraints such as faculty shortages, funding limitations, rigid curricula, and inconsistent policy support. Overcoming these barriers requires multi-pronged strategies involving staffing reforms, policy development, and sustained institutional support.
% Common themes of Administrative and Institutional Remedies in
% our reviewed papers are:
% \textbf{1. Addressing Staffing Shortages and Workload}~\cite{VanDeGrift2023}~\cite{Akhmetov2024}~\cite{Sauerwein2023,Forden2023,Wang2021,Kumar2022}Materials~\cite{Vahid2024}~\cite{Everson2022,Yadav2022,Perlman2021}.
% \textbf{2. Enhancing Teacher Preparation and Professional Development}~\cite{Weintrop2022}~\cite{Yadav2022,Flatland2022}~\cite{Jetzinger2024,Tsan2022}~\cite{Yadav2022,Flatland2022,Huff2021,Saraiva2021,Hamouda2025}~\cite{Simmonds2021,Hamouda2025,Friend2022}.
% \textbf{3. Curriculum Alignment, Policy, and Institutional Support}~\cite{Upadhyaya2020,Jia2022,Vahid2024},~\cite{Grover2024,Simmonds2021,Parthasarathy2024}~\cite{Kalathas2022,Anyango2021,Mahoney2023}~\cite{Jia2022,Hwang2023,Brunelle2022,Skuratowicz2021}~\cite{Fowler2023}~\cite{Mahon2024,Lau2023}.

% \subsection{Remedies for Training and Professional Development Challenges}

% The rapid evolution of computer science (CS) and the growing demand for CS education have intensified training and professional development (PD) challenges for educators at all levels. A significant proportion of teachers and teaching assistants (TAs) lack formal backgrounds in CS or discipline-specific pedagogical training, highlighting the critical need for sustained, accessible, and context-relevant professional learning opportunities.
% Common themes of Training and Professional Development Remedies
% in our reviewed papers are \textbf{1.Comprehensive and Sustained Training Programs}~\cite{Tsan2022,Lee2022},~\cite{DiPaola2023}~\cite{Lee2022}~\cite{Basu2022,Everson2022,Tsan2022,Yadav2022}~\cite{Macann2023,Jia2022}~\cite{Jetzinger2024},~\cite{Patel2024,Tsan2022,Skuratowicz2021,Hamouda2025}~\cite{DiPaola2023,Musaeus2024,Lehtimki2022,Grover2024},~\cite{Kussmaul2022,Minnes2022,Flatland2022,Wilde2024,Haglund2024,Markel2021}~\cite{Riese2021}.
% \textbf{2.Addressing Specific Knowledge Gaps and Skills}
%~\cite{Kumar2021,Everson2022,Flatland2022}~\cite{Kumar2021},~\cite{McGill2024,Grover2024,Hu2023,Marshall2020,Yadav2022}~\cite{Izu2025,Tshukudu2021,Munasinghe2021}~\cite{Parthasarathy2024}~\cite{Hu2023}.\textbf{3.Optimizing Training Delivery and Support Systems}~\cite{Jetzinger2024,Tsan2022,Perlman2021,Minnes2022}~\cite{Zaman2023,Riese2022}~\cite{Cheng2024},
%~\cite{McGill2023}~\cite{Jocius2021,Skuratowicz2021}~\cite{Everson2022,Flatland2022,Wilde2024}~\cite{McGill2024}~\cite{Zaman2023,Kussmaul2022}.


% \subsection{Remedies for Socio-cultural Challenges}

% Socio-cultural challenges in computing education stem from entrenched inequities, systemic biases, and the diverse cultural, linguistic, and socioeconomic backgrounds of learners. Addressing these challenges requires multi-pronged efforts focused on equity, inclusion, and cultural responsiveness across curriculum design, pedagogy, educator training, and student engagement.
% Common themes of Socio-cultural Remedies
% in our reviewed papers are 
% \textbf{1.Promoting Diversity, Equity, and Inclusion (DEI)}
%~\cite{Hill2021,Venn-Wycherley2020,Hwang2023,Hamouda2025,Wilde2024}~\cite{Hamouda2025}~\cite{Huang2023,Simmonds2021}~\cite{Hill2021,Flatland2022,Nugent2022,Weintrop2022}~\cite{Grover2024,Lee2022,Mahon2024,Hu2023,Rosenbloom2023,Yadav2022}.\textbf{2.Fostering Inclusive Learning Environments}
%~\cite{DiPaola2023,Perlman2021,Flatland2022,Malik2024}~\cite{Hamouda2025,Sentance2021}~\cite{Markel2021}~\cite{Venn-Wycherley2020,Hwang2023,Hamouda2025}.
% \textbf{3.Adapting to Cultural and Linguistic Diversity}
%~\cite{Hamouda2025}~\cite{Zaman2023}~\cite{Marshall2020},~\cite{Repenning2021}.

% \subsection{Remedies for Sense of Community/Belonging Challenges}

% A strong sense of community and belonging is crucial for both students and educators in computer science (CS), fostering motivation, reducing isolation, and supporting learning. Challenges often arise from the solitary nature of programming, lack of diverse representation, and traditional teaching structures.
% Common themes of Sense of Community/Belonging Remedies
% in our reviewed papers are 
% \textbf{1.Cultivating Supportive Communities for Educators}
%~\cite{Flatland2022,Kussmaul2022,Perlman2021,Ni2021,Hill2021,Tsan2022,Lee2022,Nugent2022,Yadav2022,Wilde2024}~\cite{Flatland2022,Marshall2020,Nugent2022,Wilde2024,Jetzinger2024}~\cite{Jocius2021,Nugent2022,Lee2022}~\cite{DiPaola2023,Lehtimki2022,Musaeus2024}~\cite{Markel2021,Riese2021,Riese2022,Wilde2024}~\cite{Riese2022,Minnes2022,Akhmetov2024,Haglund2024,Huang2023}~\cite{Flatland2022,Ni2021}~\cite{Vahid2024}. ~\cite{Fowler2023}.\textbf{2.Fostering Belonging for Students}
%~\cite{Hamouda2025,Hwang2023,Rosenbloom2023},Promoting Collaboration
%~\cite{Brunelle2022,Vahid2024,Hamouda2025,Luxton-Reilly2023},~\cite{Huang2023},~\cite{Malik2024},~\cite{Macann2023},~\cite{Venn-Wycherley2020,Samarasekara2023,Wilde2024}~\cite{Vahid2024,Zaman2023}.


% \subsection{Remedies for Parental and Community Involvement Challenges}

% Effective Computer Science (CS) education extends beyond classroom walls and thrives through active engagement with parents, communities, and industry stakeholders. Overcoming barriers such as limited parental awareness, insufficient community buy-in, and weak industry collaboration is essential for building robust and sustainable CS education programs.
% Common themes of Parental and Community Involvement Remedies
% in our reviewed papers are
% \textbf{1.Increasing Awareness and Gaining Buy-in}
%~\cite{DiPaola2023},~\cite{Samarasekara2023,Yadav2022},~\cite{Williams2020},~\cite{Hooshangi2025}.\textbf{2.Fostering Collaboration and Partnerships}~\cite{Hooshangi2025,Lee2021,Parthasarathy2024}~\cite{Rosenbloom2023,Yadav2022}~\cite{Flatland2022}~\cite{VanDeGrift2023},~\cite{Williams2020}.\textbf{3.Engaging Parents in Student Learning}
%~\cite{Lehtimki2022},~\cite{Hwang2023},~\cite{Hill2021}.

% By leveraging these multidimensional strategies, CS educators are working to cultivate a more integrated ecosystem—uniting schools, families, industry, and communities to ensure holistic and equitable computing education.


